"It's A Blessing and A Curse": Unpacking Creators' Practices with Non-Fungible Tokens (NFTs) and Their Communities

NFTs (Non-Fungible Tokens) are blockchain-based cryptographic tokens to represent ownership of unique content such as images, videos, or 3D objects. Despite NFTs' increasing popularity and skyrocketing trading prices, little is known about people's perceptions of and experiences with NFTs. In this work, we focus on NFT creators and present results of an exploratory qualitative study in which we interviewed 15 NFT creators from nine different countries. Our participants had nuanced feelings about NFTs and their communities. We found that most of our participants were enthusiastic about the underlying technologies and how they empower individuals to express their creativity and pursue new business models of content creation. Our participants also gave kudos to the NFT communities that have supported them to learn, collaborate, and grow in their NFT endeavors. However, these positivities were juxtaposed by their accounts of the many challenges that they encountered and thorny issues that the NFT ecosystem is grappling with around ownership of digital content, low-quality NFTs, scams, possible money laundering, and regulations. We discuss how the built-in properties (e.g., decentralization) of blockchains and NFTs might have contributed to some of these issues. We present design implications on how to improve the NFT ecosystem (e.g., making NFTs even more accessible to newcomers and the broader population).

==> section/2_Related_Work.tex <==
\section{Related Work}
In this section, we present literature on related innovative marketplaces such as art markets, which have similarities with the NFT marketplace. The interaction between art creators and collectors in traditional art markets is also comparable to that in the NFT marketplace.
% , in terms of individual interactions and community dynamics. 
% We mainly present prior literature on conventional art market on how people perceive the value of art and goods in a commercial environment and 
We also present literature on motivations for engaging in online communities, and typical community interactions and dynamics.
% what are some factors for them to engage in this environment and how the community interact with each other to differentiate characteristic with NFT marketplace.  
% \yang{why art exhibitions/auctions are relevant? make the connection clear} \tanusree{made some connection}. 
Lastly, we include the challenges and disadvantages of blockchain, upon which the NFT marketplace is built. 

\subsection{\textcolor{black}{Similarities and Differences between Traditional Art Market and NFT Marketplace}}

% \yang{this section presents points that are pretty ad-hoc, it'd be better to organize it in a clear structure with major points, which should have clear relevance to NFTs. NFTs are like art pieces, art exhibitions/auctions are like NFT trading. should differentiate these concepts.} \tanusree{edited}

\subsubsection{Market Structure, Stakeholders, and Characteristics}
The NFT marketplace has some similarities with traditional art exhibitions and auctions, as well as online creative communities. They all have two parties: owners/sellers and buyers. In traditional art markets, objects offered for sale are unique pieces, the value of which is determined by their characteristics (e.g., topic, medium, and reputation of artists), subjective non-monetary utility \cite{goetzmann2011art}, and resale value affected by demand factors (e.g., wealth concentration, equity market evolution, changes in art-collecting audience) \cite{lovo2018model}. Similarly, NFT are collections of art, music, games, etc., the trading of which is supported by the underlying distributed ledger, with consistent records of transactions. NFT tokens are unique and can have different value depending on its' rarity, quality, and reputation of creators. 
% Functionalities such as transferring NFT tokens with certain value from one account to another are supported. They can also be resold. 

The main difference between the two marketplaces is that the ownership chain is not well structured in traditional art markets, which may lead to fraudulent events; whereas NFT tokens are created and traded on top of blockchain, the ownership of which can not be easily tampered. From literature, we find that information on provenance, such as details about an art object's pedigree, is important, as it may increase people's confidence in the authenticity of the art object offered for sale in the marketplace \cite{van2002art}. Thus users are in favor of an ownership chain on which art objects can be uninterruptedly traced back to their artists/creators, and associated with photographs, certificates, etc. NFT provides such a feature backed up by the underlying blockchain, bridging the gap of traceability which may improve its trustworthiness. 

\subsubsection{Market Trading Environment}
In the traditional art market, price of goods is established through an interactive and mediated competition between different buyers \cite{auction}. The auction process provides the bidding function in a transparent manner, which enables legitimate and fair valuation and exchange of goods \cite{auction2}. Different social factors, such as social interaction and social structure, can influence buyers' behavior in online auctions. For example, there often exists interactive competition among online actors, which has proven to be one of the most successful and rapidly growing business models for electronic commerce \cite{auction2}. Similarly, NFT marketplaces also allows users to bid for NFT collectibles. Moreover, when an NFT is sold, its metadata and ownership details are added to a new block on the blockchain, thus the ownership history is recorded and preserved. 
% It creates a future block for buyer which is linked to the original data block of sellers as a form of history. 

% In the NFT trading environment,  

\subsubsection{Different Functionalities of NFT and Non-NFT Ecosystems}
\review{While ultimately not the biggest issue, I do believe the lack of engagement with external literature on traditional art markets (ex - Lind, Maria, and Olav Velthuis. "Contemporary art and its commercial markets: a report on current conditions and future scenarios." (2012).), and how issues of forgery are handled in the traditional art world. I would also like to see how the authors situate NFT wrt to copyright infringement issues and piracy more generally including piracy prevention technologies which aren't based on the blockchain. I would also really enjoy seeing more discussion of non-blockchain digital art ecosystems. Concern Level - P2}

\subsubsection{Social Factors in Marketplace}
Due to the lack of literature on social factors in NFT marketplaces, we explore traditional art markets to identify social factors that might lead to success or failure during trading. Researchers have conducted ethnographic studies of the auction market to understand social interaction, visual and material conduct of bidding and buying, operation of markets, and success of auction outcomes \cite{auction}. One of the objectives of this study \cite{auction} is to understand how users interact with the marketplace during trading. In our study, we will conduct an interview study to understand social factors and interactions in the NFT marketplace and community. 

Another topic emerging from the traditional art market is trust. In art auctions, equilibrium prices reflect true value of goods. In this process, trust is established in the community to buy and sell goods. Information on provenance of goods and an open market for bidding create trustworthiness and reliability which reduces the information asymmetry between different trading parties (i.e., buyers and sellers) \cite{auction, bidding}. However, it has been found that information disclosure and pedigree identification are challenging in conventional markets. Given the ownership mechanisms and transparency of the NFT marketplace facilitated by the blockchain, 
% \yang{elaborate this point. what concretely do we know about trust in this context?} \tanusree{elaborated}
it would be interesting to see whether the trust issue is well resolved in NFT trading, and what different user behaviors and community dynamics are there compared to the traditional art market. 

% \yang{Norman Su has written extensively about authenticity in HCI. you should take a look and cite} 
% \tanusree{addressed the comment}
% \textcolor{blue}{They also argued that trust as a factor which is a subjective construct and related to a combination of received referrals and personal experience \cite{virtual} while reputation is another factor that implies quantity derived from the underlying social network \cite{reputation}.}

\subsubsection{Societal Benefits of Art/Creative Markets}
Art exhibitions are common creative commercial market.
% For example, Aesthetica Art Prize Exhibition re-defined the parameters of contemporary art \cite{spence2020bob}. 
They provide a platform for artists from around the world, and support their careers with prize money, exhibition and publication opportunities, and talent development. For the audience, exhibitions are also an environment to efficiently learn about art in an interactive manner, and socialize with other visitors \cite{vosinakis2011virtual}. Moreover, research shows evidence of positive relationship between the engagement in art and physical/psychological well-being of older people \cite{o2012impact}. Arts also provide a paradigm of interaction to enhance children's experience, and support their engagement, learning, and social behavior \cite{rizzo2007fire}. 

There have been attempts for virtual art exhibitions, which allow local and remote visitors to co-exist in the environment, access the interactive content, and communicate with each other \cite{vosinakis2011virtual}. There is a similar trend in the NFT marketplace,
% . There are varied amount of art pieces such as, traditional art, AI based digital art, games, memes, columns, twitter posts, animated crypto characters, top shots from games, etc.
with NFT creators creating different types of NFT, and virtually exhibiting and selling them. 
% to showcase their expertise and create a community with similar interest \footnote{https://www.theverge.com/22310188/nft-explainer-what-is-blockchain-crypto-art-faq}. 
% In this research, we study on NFT users to understand how and what motivate them to be in NFT creative community.
However, there has been a lack of research on the emerging, virtual NFT space. Here we aim to bridge this research gap by understanding the benefits of NFT for people engaging in the NFT marketplace. 

\subsection{Motivations and Dynamics of Community Engagement}
\review{Section 3.2) references are used quite erratically to reference broad concepts. However, more concerningly, the paper fails to engage at all with extensive prior work in HCI and CSCW on blockchain technologies. I've listed a number of relevant works below, but a particular omission is the extensive  ethnographic work by Gao, Lustig, Kow and others around the emergence and values of crypto communities and users. These directly underpin the current NFT hype, and are exemplary works for the analytic depth and rigour in understanding the nature of these communities. Many of the same themes and findings of this paper, are present in this earlier work.
}

People in a group, either in the physical world or social media space, may share similar interests for art, politics, sports, etc. Research shows that socializing, as a vital social activity, is not necessarily task-related. People also socialize with other individuals for emotional reasons \cite{community}, e.g., feeling included in a community. People with similar interests tend to support certain events together, e.g., posting and cheering for certain sports teams using slogans and videos \cite{fandom}. Different ways can facilitate social interaction, such as image sharing, and text-based communication \cite{interaction}. Our everyday objects augmented with technologies can also contribute to disseminating people's lifestyle values \cite{cheon2021jarvis}. The circulation of values may inform us about the alternative roles of technologies in speaking for our norms in a community environment \cite{cheon2019beg}. In a previous study on innovation communities \cite{innovation}, intrinsic motivations prove to be effective for participation and long term engagement in online innovation communities. It is shown that the majority of participants are engaged to the online innovative community for fun and activities that challenge them. In most cases, participants' roles were contributors and collaborators instead of leaders. Extrinsic motivations such as reward also attract people who are interested in objective values \cite{lakhani2003hackers}.

Within a short period of time, we have seen the forming of an active NFT community. There are many online communities and forums for NFT users, such as Discord channels of NFT projects, and discussion forums on NFT trading platforms such as Rarible. Such gathering of individuals with similar interests provide NFT users with an opportunity to share their accomplishments and values in public platforms. In this work, we will look at people's motivations for joining the NFT community, which is intrinsically an innovative community of artists, as well as community dynamics and interactions, toward understanding NFT practices from both individual and community perspectives.  

\subsection{Advantages and Challenges of Blockchain}
The decentralization feature of blockchain enables cryptocurrency built on it to be censorship-resistant. No one has the ability to freely modify transaction data on the ledger. However, some unwanted features also come with decentralization, e.g., lack of scalability, high gas fee, and lack of regulation. Chu et al. propose a quantitative measure of blockchain decentralization, and prove that a fully decentralized blockchain inherently limits scalability, as it incurs a throughput upper bound and prevents scaling smart contract execution \cite{scalability}. Layer-2 \cite{layer2} solutions try to solve the scalability issue by taking some computations off the main chain, and using an extra chain to speed up and scale transactions. One example is OMG Network\footnote{\url{https://omg.network/}}. 

Gas fee on the Ethereum blockchain is especially high recently, given the high volume of on-chain traffic. While miners earn more with increased gas fee, users of DApps built on Ethereum such as Uniswap\footnote{\url{https://uniswap.org/}. Uniswap is a decentralized exchange built on Ethereum.} will have to pay more for their transactions. In Ethereum, users who pay higher fees will have their transactions confirmed faster. To understand the correlation between gas fee and pending time, Sousa et al. collect information about 7.2 million transactions, and conduct a correlation analysis \cite{fee-pending}. Tools have also been developed for lowering gas fees in smart contracts. For example, Albert et al. present Gasol, a gas analysis and optimization tool for Ethereum smart contracts \cite{gas-opt}. Since storage costs a large portion of gas fee, developers use this tool to detect under-optimized storage patterns, and runs an automatic optimization of the selected function.   

Since the blockchain is completely free of regulation, it is also easier for malicious users to commit crimes, e.g., money laundering, and trading illegal items such as drugs \cite{crime}. The blockchain removes the relationship/link between a transaction and the person who conducts it (a.k.a., anonymity), thus it is extremely hard for the police or the government to trace the illegal transactions.

NFT as a new technology built on blockchain may inherit some of the limitations mentioned above. Thus it is important to examine both NFT-specific and blockchain-induced drawbacks, toward creating a better NFT landscape.

==> section/4_Findings-2.tex <==
\section{Findings}
% \review{ How does a persons’ role impact their perceptions of blockchain? Their motivations? The challenges they face?}
% \review{Both in their method, and limitations, but also throughout the findings, I feel the authors could be much more careful and critical in how participants' views are presented and analysed given this investment.
% }
% \review{ In particular, the authors do not ask for any of the participants' experiences with non-NFT markets which I believe limits our ability to interpret the feedback of the participants. Secondly, I think this interview protocol is too focused. NFTs and blockchain technologies have a number of impacts and qualifications to their function such as issues of piracy topics, among other impacts of blockchain, in the interview protocol, as well as the fact that the participants were already participants in NFT communities, makes me somewhat suspect of the picture that these interviews are painting wrt to the general sentiment that these interviews are painting. Maybe it is valid to say that participants just aren't thinking of those issues, but I do think some discussion by the authors of that fact is necessary. Concern level - P1.}
% \review{Overall I found the results section easy to read and well structured; however, it’s a lot of information. If the authors continue to present all the themes in a single paper I would recommend organizing them in a table with short descriptions.}

We now present our participants' \textit{perceptions} of NFTs, including their motivations for creating and engaging with NFTs (RQ1), their  criteria for what makes a good NFTs (RQ2), as well as their \textit{practices}, including their individual and community engagement (RQ3), and challenges that they encounter when engaging with NFT (RQ4).

\subsection{Perceptions of NFTs}

\subsubsection{Motivations for creating NFT (RQ1)}
Our participants indicated different motivations for creating NFT, such as,   expressing personal feelings, emotions, pleasure and a sense of accomplishment in presenting creative artworks, being a part of the innovative movement, and making a profit out of making/selling NFT. Below we will elaborate on different motivations of our participants to create NFTs. 

%\yang{I think we should focus on why they create NFT}
%\zhixuan{now framed from creators' perspectives}

\noindent \textbf{Unique Traits and Ownership.} 
% Unlike, cryptocurrency, NFT cannot be traded for each other as they are unique representations of assets. 
%  (P1, P5, P7, P8) 
Several participants mentioned their motivations for creating NFT as the unique ownership model of digital assets, and its ability to represent real-world items. NFT tokens are non-fungible, and each NFT has its unique traits, while fungible tokens (e.g., Bitcoin, Ether) are all the same. 
% , and its interchangeable in contrast to fungible tokens. 

This motivation was echoed by NFT owners as well. For example, P1 pointed out that every Bitcoin was the same, while NFT were created by different creators, thus had unique value. This participants attributed unique traits of NFT to different intentions of the creators. \yang{quote could be removed} \tanusree{done}

% \begin{quote}
%     \textit{``Every single Bitcoin is exactly the same. When it comes to NFT, they have different creators who made it by intention. It has customized built-into words, and it has digital files attached to it to give it value.''}
% \end{quote}
Uniqueness of NFT gave it more roles than merely speculation, which differentiated it from other fungible tokens, as P7 pointed out:
\begin{quote}
    \textit{``Fungible tokens are more for speculation, and people trade them in the same way as stocks. But non-fungible tokens, most of them are kind of art. [...] They have some special traits, very different from each other. If you own one of them, you have some personal emotion for it, use it as an Avatar. 
    %and sometimes you don't want to resell it.''
    }.
\end{quote}
As he said, many people viewed NFT as collections with unique traits, and would not resell them for speculation purposes. He himself would create NFT avatars of himself that could embed his attributes into unique traits of the NFT. 

% It has been very common among participants that they don't appreciate NFT which were simple copies of successful ones-doesn't present special traits and creativity: P1 said-\textit{``There're thousands of copy cats that are trying to replicate what CryptoKitties have accomplished. And the unfortunate thing is, it's actually working, people are buying the copy cats. When it comes to art, you have to be creative. ''}

\yang{it'd be great to say how many participants said a particular theme}
\noindent \textbf{Expressing Personal Emotions through Creating NFT.}  We observed expressions of personal feelings and emotions as one of the main motivators for NFT creators. 
% P7 thought each NFT had unique characteristics, which explained why creators and owners attached personal emotions to NFT: \yang{kind of repeat about being unique. remove this quote}
% \begin{quote}
% \textit{``Non-fungible tokens, most of which are kind of art, have some special traits. They're very different from each other. If you create one, you have some personal emotions for it''}
% \end{quote}
Some participants mentioned creating NFT, such as NBA Top Shot video clips to support their favored sports teams and players. For example, P10 
% \begin{quote}
%     \textit{``I started to create NBA Top Shot video NFTs to show my feelings.''} 
% \end{quote}
offered emotional support to his favored sport team by creating NFT with the players' finest playing moments. In his case, NFT served to convey his attachment and support to the sports team. 
One of the extraordinary examples is P11, who did not have any technical background, yet wanted to create NFT for his child ready to be born in December 2021, which was seen by him as a way to keep memories for his son. He noted, \yang{best quote so far} 
\begin{quote}
    \textit{``I was thinking of creating NFT because my child will be born in December. I'm thinking of making some connections between the baby and the blockchain, and even create a trend on the market. I think I'm fine with Photoshop and simple art, as well as uploading it to the Ethereum blockchain. I want to do this because I want to keep some memories for him, like funny stories and his dreams.''}
\end{quote}
As we can see, this participant viewed NFT as a sentimental item to keep memories for his son, which revealed the association between NFT creation and people's real lives. The interplay between virtual NFT and personal events in the physical world further attached emotional value to NFT. Some participants also mentioned about sending NFT postcards on special occasions to extend good wishes. 

% P4 explained her stress during pandemic and how she overcome by creating NFT duckies. She explained - \textit{``I have a stressful job during COVID. I needed the thing which is able to create in different ways and the duckies are always in our world everywhere, all over the world.''} 
 
%  It has been very common among participants that they don't appreciate NFT which were simple copies of successful ones-doesn't present special traits and creativity: P1 said-\textit{``There're thousands of copy cats that are trying to replicate what CryptoKitties have accomplished. And the unfortunate thing is, it's actually working, people are buying the copy cats. When it comes to art, you have to be creative.''}

% \review{In effect, the findings primarily recount a small number of experiences, and opinions of those working with NFTs - rather than analysing more deeply the values, implications, and logic of their participants. For example, Pg16 includes a remarkable quote from a participant about creating an NFT aligned with the birth of their son. There is so much more that could potentially drawn out here – that speaks to the role NFTs play in people's lives, the intersection of the 'market' with even the most personal events, the presumed permanence of NFTs etc. As it is, many quotes are left to speak for themselves, and some sections or sub-themes are extremely short.} \tanusree{tried to describe the quote above}

% \zhixuan{10/26: updated till here, split long paragraphs, did some writing and formatting work}

\noindent \textbf{Expression of Creativity.} Expressing creative ideas via NFT was yet another motivator for our participants. Many of whom are artists such as landscape photographers, film maker and tattoo artists create NFTs to demonstrate their creativity in subsequent domain. 

Creating NFT swas seen by them as a way to express themselves, according to P4 and P5. Artists could create/mint NFTs out of their own ideas, without having to follow clients' requirements. In P4's previous business, she had to design tattoos for clients' ideas and requirements while now she could create NFTs out of her own ideas and interest:
\begin{quote}
    \textit{``This was a way to step out of my comfort zone of normal art a little bit, start something new, learn something new, and create something new. In my previous [tattoo] business, I created tattoo designs for my clients' ideas. But NFT are just my own ideas, and that's pretty cool to make something new.''}
\end{quote}

Similarly, P5 combined his multiple personal interests, such as writing, blogging, and video editing into NFT creation which were ways of expressing and content creation for him. \tanusree{less interesting}
\begin{quote}
    \textit{``I've experienced a lot of different forms of content creation on the Internet. I've been a writer. I've been a Blogger. I've worked for the University of [redacted], sort of doing academic stuffs. I've been a video editor. I'm an artist as well, so sort of all these different things. Interests of mine sort of came together for this [NFT] project.''} 
\end{quote}

% Since he ran an NFT company, building a brand that people love was also an important motivation in his NFT creation and promotion:\begin{quote} \textit{``I think the most important thing to me is sort of building a brand and building a company that people love, and creating content that people love. Like that's my motivator, like I entertain people you know. Like I've put out videos on Decentraland, the game I was talking about earlier, they had like tens of thousands of views, or hundreds of retweets, or whatever, because people like it.''}\end{quote}P2's motivation for creating NFTs is also ``trying to make everyone happy'', which was seen by him as a kind of professionalism for artists. 



\noindent \textbf{Transparent Business Model.} In the traditional art market, artists often relied on event organizers and sponsors to exhibit their work \cite{spence2020bob}.
% Similarly, many participants indicated the decentralization in ethereum blockchain as a self-governance mechanism where individuals don't require to trust or grant custodianship to a third party imposing rules. 
The decentralized, self-governing Ethereum blockchain, freed the NFT marketplace from gatekeepers. P13 indicated the NFT platform as an autonomous platform which empowered artists, who could exhibit, sell and promote their work out of their own will and they can regulate their goods with underlying smart contract: 
\begin{quote}
    \textit{``One of the benefits [of the NFT marketplace] is that there are no gatekeepers like in the traditional art market. In the NFT world, you're a self promoter. You just need to come on the platform and do your promotion, and sell NFT.''}
\end{quote} 

In addition to removing gatekeepers from the the art market, NFT also empowered artists by providing them with a low entry level. P9 and P11 mentioned the low barriers to entry for NFT artists to present their digital work. Even unknown artists could grow their career in the NFT marketplace. 
% NFT marketplace gives an opportunity to numerous digital artists to pounce upon and use their skills to earn living.
P11 described how the inclusive, supportive NFT marketplace enabled unknown artist to thrive:
\begin{quote}
    \textit{``Some artists are unknown, and it's hard for them to make money. I know some artists in Taiwan who are not that famous. They make extra money by creating NFT of their artwork. So I have friends who are painters, I recommend them to create NFT on the platforms.''} 
\end{quote}

Some participants created NFT due to its convenient business model. P3, who owned an NFT company, highlighted convenience of the business model to create NFT due the underlying Blockchain. He thought NFT allowed freelancers to automate their workflow, with all transactions recorded by the blockchain and easily exportable, which made people's work more efficient: \tanusree{good quote}
\begin{quote}
    \textit{``It empowers individuals to create their own business model. Your business transactions would always be recorded. I think it's something that will benefit freelancers to automate their workflow. You don't have to worry about tracking receipts. They're all stored on the blockchain.''}.
\end{quote}
% He also added the advantage of cryptographic ownership model that allow them to get the interest of their content every time it changes hand to different buyers/collectors. The basic conceptions and key characteristics of NFT are its authenticity and cryptographic ownership, 

In the conventional art market, the process of verifying copyright of intangible commodities is cumbersome. Often times, there is not a way to validate their provenance \cite{van2002art}. On the contrary, NFT collectibles including art/design and game items are valued for their authenticity, rarity and cryptographic ownership. Each minted\footnote{``Minting" refers to the process of tokenizing an item, and uploading it to an NFT platform such as Foundation.} item is encoded into the underlying blockchain \cite{wang2021non}, which can be traced back to its owner. The transparency and traceability of the NFT business model could be attributed to the underlying cryptographic mechanisms, which allowed buyers to check authenticity of NFT art. P7 contrasted the pre-NFT and post-NFT era regarding authenticity confirmation, demonstrating the level of transparency, NFT brought to the art market:
\begin{quote}
    \textit{``Before NFT was a thing, I would post paintings on Instagram, and offer them for sale. 99.9\% of people would just say, why should I buy it? I can just copy the image and download it for myself. There's no real way to prove that you created it or that you've bought it. Now every time it is sold, I get the percetage''}
\end{quote}
The concept of ``percentage'' mentioned by P7 showcased the long-lasting traceability of NFT. People could trace their NFT even after it has been resold several times.

\noindent \textbf{Being a Part of an Innovative Movement.}
Some participants created NFT out of the purpose of being a part of the blockchain innovation and NFT art revolution. P13 started his NFT career during pandemic to make a living, but he kept creating NFTs even after pandemic to stay in the NFT marketplace, which he thought was an ongoing art revolution:
\begin{quote}
    \textit{``It's the new art revolution[...] I'm better in online marketing than in the real world. I guess it's a cool new thing because I have pretty much followers on Instagram and Facebook. On Instagram I have around 180,000, and on Facebook I have 110,000. So I know I'm better in online stuff, and it's excited to be part of this revolution.''}
\end{quote} 
Some created NFTs due to their interest and passion in blockchain technologies. P5 said: 
\begin{quote}
    \textit{``It's like a new frontier right on the Internet, you know, we're sort of on that cutting edge of all the cool new stuff that's coming out. And a lot of that, has to do with blockchain.''} 
\end{quote}
P11 was yet another case. He thought creating NFTs ``made him feel that he was keeping up with the times.'' Many members of the NFT community shared the excitement about the advancement and value of NFTs, and wanted to do more to develop this space. They called NFT the new Renaissance for artists. P3 noticed:
\begin{quote}
    \textit{``Almost everyone that I've interacted with believes this [NFT] to be one of the most important technologies and advancements in our lifetime. A lot of people are calling it the new Renaissance for artists[...]. A lot of new inspiration and new art is coming out, and people are very willing to collaborate in network, across countries, across the world. So, overall perception I've received is, people are very excited and very optimistic, and they want to do more with this space and develop it.''}
\end{quote} 

Many participants indicated how they used NFTs as a self identity in digital space. P7 thought NFTs could be used as personal identities when making friends online, especially in the Metaverse \footnote{https://studio.gometa.io/landing}, which was a virtual shared space:
\begin{quote}
    
\textit{''I believe in the future, people will spend more time on the Internet, in the virtual world, in the Metaverse. And in that world, people don't meet each other physically. People use their digital identities to make friends with each other.''} 
\end{quote}

Similarly, Bored ape was a popular NFT project. P7 told that NFT-related Clubhouse room used bored apes as their Avatars, which showed their membership. This participants also explained an idea discussed in their NFT group of creating a ape NFT themed attack for a non NFT group. The main idea is to let the non NFT people to know about NFTs. P11 thought one day, a bored ape may be used as the digital identity to attend parties held by the community. Similarly, P3 indicated the about this growing community with diverse people. He added that how he made friends within this short period and gained a large network. He felt that this community provided him the ability to reach out many people.

\noindent \textbf{Supporting Art Business during Pandemic.}
\yang{maybe combine this subsection with the earlier subsection on transparent business model into a subsection on creating NFTs for art business}
%\yang{making money is less interesting. i think we can focus on supporting art business during pandemic and a new mode of art} \zhixuan{framed in this way}
Given the high monetary return of NFT selling, many people were devoted to NFT creation and trading nowadays, as reported by our participants. Our participants who were NFT creators would sell their NFTs for monetary value. This was especially true during the pandemic, when offline art trading was impossible, and they would rely on the virtual NFT market for a living.

Some traditional artists tried to keep their business up through the new occupation of NFT during the pandemic, when offline business was made impossible by lock-down policy of many cities. For example, P13 was the inventor of the famous hyper-real landscape photography, and used to earn money through workshops, tutorials and speeches in pre-Covid times. The pandemic hurdled his offline work, and he had to turn to the NFT market for a living: \tanusree{good quote}
\begin{quote}
    \textit{``The events I used to attend for a living were almost not possible during the pandemic. So I lost almost 80\% of my income because of that. [...] Then I built a team with 2 guys. Now I try to sell as much NFT as possible in my spare time to earn enough money to pay my bills.''}
\end{quote}

Similarly, P4, who was a tattoo artist, also started her NFT career out of the purpose of keeping her business up in a virtual/online manner during the pandemic, when Berlin was in locked down:
\begin{quote}
    \textit{``I started creating NFT during the pandemic. Lockdown was just the reason for that, I came to know and research about it.''} 
\end{quote}

The pandemic doesn't seem to end in a short period, thus the NFT martketplace will keep playing a role in supporting traditional artists who want to take a transition to digital art.

%Some participants mentioned to trade NFT and speculation for future gain in profit. P3 would buy NFT with the specific intention of re-selling them for a higher price: \textit{``I bought one piece (of NFT), specifically with the intention of reselling it. So I saw that it was pretty undervalued, or I knew that it was going to go up in price. So I bought it, and I'm currently holding it up, basically with the intention of selling it eventually.''}

%\textbf{Fear of Missing Out (FOMO)}. One of the emotion, Fear of Missing Out (FOMO), noticed among people who create and speculate on NFT. When the price of a cryptocurrency went up, or when a new cryptocurrency was listed, they would purchase it out of the fear that the price would go up sharply one day. If she did not buy it, she would miss the huge opportunity while other people grabbed it. It was also a major motivation for P11 when he bought NFT: \textit{``I was controlled by the FOMO emotion. I told myself not to buy more NFT, but when I saw many people talking about it in Discord, I started buying again. I thought the price would go up.''} However, the price of several NFT he bought due to the FOMO emotion dropped by a large percent.  Some traders merely cared about financial returns, without considering the real value of NFT. P1 expressed his disapproval of this phenomenon:  \textit{``Some people are just arrogant. They're rich, and they just like to waste their money. So they buy whatever is popular. Some people convinced themselves that something would gain value, even though it's not that great of an investment.''}

% P7 also observed that most members in an NFT-centered Clubhouse room cared more about speculation than the real value of NFT:% \begin{quote}
%     \textit{``And I think most of them in our room, just like me, are quite new to the market. And most of them want to make some profits, which means even if they buy an ape NFT they like, when the price goes down, they will be frustrated. And some of them will panic sell. Because the NFT tokens are not a small amount of money. They're spending like tens of thousands of RMB for an image, and if they cannot sell the image later, they're losing a lot of money. So, for them, they have some expectation to sell them in the future for a higher price. So, I think most of them were up there for speculation.''}
% \end{quote}
% P15 did not like it when people created and bought NFT only for money:
% \begin{quote}
%     \textit{``People think differently about NFT. Some of them think it's a good marketplace to get money. Some of them think that it's a good place where you can get inspiration. And some of them want to share their artworks with people. I don't like people who think it's only for money. Because it's not for money. It's our industry. It's good to create good art in the industry right now.''}
% \end{quote}

% \zhixuan{since we're discussing the community aspect later, maybe we can remove the motivation of community engagement here} 
\noindent \textbf{Staying in The Supportive Community.} \tanusree{they also mention---will describe in later section}
Some mentioned the supportive community as a motivation of being in the NFT space. For example, P4's motivation for staying in the NFT marketplace after the pandemic had much to do with community ties, such as mutual support and understanding among the artist community: 
\begin{quote}
    \textit{``The first thing I think is the community of artists. I didn't know that such a kind and supportive community would even exist (before I started my NFT career).[...] Artists understand other artists, so it's pretty good to ask them for advice and opinions. I think being in this NFT community is the most important thing.''} 
\end{quote}
In later section \ref{5.2}, we will elaborate more on community aspects of the NFT marketplace. 

% Among our participants, we didn't observe much collaboration in NFT creation. In most cases, NFT creation was a reflection of artists' own unique emotions and skills.
Collaboration was found common in the NFT community. For example, P6 mentioned how the artist community collaboratively proposed new forms of NFT art: 
\begin{quote}
    \textit{``We're really collaborative and always trying to make valuable pieces of art, not trying to make products just for sale. We're always thinking about proposing something new in the art market.''}
\end{quote}
As the founder of an NFT platform, P10 would attend online meetings organized by other platform founders and developers, and discuss product functions, as well as how to create a better NFT ecosystem for artists.

% There is a drift of willingness to collaborate. For example, P3 expressed his optimism and will for collaboration in the NFT community: 
% \begin{quote}
%     \textit{``A lot of new inspiration and work are coming out, and people are very willing to collaborate, in network, across countries, across the world.''}
    % So the overall perception I've received is, people are very excited and optimistic about collaboration. and they are wanting to do more and more with this space and develop it.
% \end{quote}

% \noindent \textbf{Building Own Business Models.}
% Another motivation for NFT users is owning a unique business model without central regulation. The decentralization of NFT supported by the underlying blockchain empowered individuals to create their own business models within smart contracts, as P3 said,
% \begin{quote}
%     \textit{``I think the first benefit for an NFT marketplace is that, it empowers individuals to create their own business model and smart contracts. So in theory, if you use the right, if you trust the platform you work with, you would have unlimited control.''}
% \end{quote}
% \subsubsection{Observed Motivations in the Community.}
% P9 enjoyed the atmosphere of NFT-game-related communities, since the members cared more about the long-term value of NFT instead of short-term speculation, and they only talked about NFT games rather than investment and prices. She thought many people bought game-related NFT out of curiosity and for collection purposes:
% \begin{quote}
%     \textit{``They don't know whether it will have value in the future. They're just curious. They just want to participate and own it. If it has value in the future, then they can have financial rewards. Even if it doesn't, they still have some fun. It's a game after all.''}
% \end{quote}

\subsubsection{Criteria for High-quality NFT (RQ2)} \tanusree{remove and add some content in challenges sections}
% \textbf{Consideration of NFT as Aesthetic VS Utility} 
A large number of new NFTs are created like bamboo shoots after the rain. People in the NFT community are overwhelmed with the ``NFT overload.'' Our participants share various criteria they used to identify good NFTs,  such as, aesthetics, creators' reputation, effort behind the NFT, vision and/or meaning behind the NFT \yang{currently no examples of this below}, and practical utility.
% \review{Aesthetic (should look nice), Reputation of creators?, visions/meanings behind the NFT (specific context behind creation), Utility (i.e. postcard for occasions, badges for social media interaction, tickets for attending conference)}
% \vspace{3pt}
%\tanusree{how about doing an analysis of their actual NFT content. They shared their NFT profile during interview. By doing so, we can address Professor Yun's comment "what’s the ethnicity background of the participants? what’s the ethnicity or political flavors of the created content?". We can have different empression and background directly from art they create. Similar to real world "Abstract Expressionism"} 

\noindent \textbf{Aesthetic.} When the participants showed the authors their collections of NFTs, either created or collected by them, nearly all of them expressed how beautiful the NFTs were. Beauty was seen as a simple and direct standard of a good NFT for P1: \yang{quote not too useful. look nice sounds too abstract. did the participant mention what the NFT s/he was referring to? might need another quote} 
\begin{quote}
    \textit{``It just looks nice. Sometimes, even if the art does not have any meaning, you personally just think it looks nice and present a good taste of NFT.''}
\end{quote} 
% By saying that, this participant further discussed how it is important it is to have creativity element in NFT. However, he added that aesthetic value of NFT has the capacity of eliciting pleasure with positive taste.

\noindent \textbf{Reputation of Creators.} When assessing the value/quality of a certain NFT, people may fall back to simple heuristics, since NFT is a relatively new field, and there is a lack of established assessment measures. For example, P3 estimated the future value of a certain NFT based on its creator's reputation and popularity. He believed NFT created by established artists would be worth more in the future:
\begin{quote}
    \textit{``It was a piece of music that I bought, and it was created by a well known musician group. My thinking is that, they're already an established group. They have a large following in social media. So there's a demand for this item. I see he's very engaged in this space.''}
\end{quote}
% This participants was both a creator and collector. In case of buying NFTs, he considered the reputation of an artists to speculate the price in future. He also added that the legitimacy of an art depends on the reputation of the artist while there are many copycat exist in the marketplace.
\update{According to this participant, NFT created by reputable artists could better serve speculation purposes, due to popularity of the artists, and people's high demand for their work. In many cases, including this participant, social media (especially Twitter) followers are one of the main indications for our participants to assess the reputation of an artist.} 

People would buy NFT created by well-known artists they perceived as talented, even without giving much thought to the real quality of the NFT. P5 mentioned a reputed figure in the NFT marketplace, who was known as Beeple and sold NFT in record-breaking amount of $63$ million dollars. \update{According to this participant, Beeple was talented and successful in delivering trending content in 3D art, and people would buy his work no matter how good it is. In addition to it, he has already a numbers of followers in twitter which is a way to discover his artwork and even gain more popularity}: 
\begin{quote}
    \textit{``His name is spelled BEEPLE. He's the biggest artist in 3D art. It's 3D animation, the most popular form of content. And people see value in it. [...] So I think people tend to like/buy things [...] created by someone talented, regardless of whether it's good or not.''}
\end{quote}

\update{Another participant, P4, who is a tattoo artist, shared her experienced how her NFTs got popularity within a very short period of time. She never had a real life art presentation in gallery. Within three months of joining NFT marketplace, she started to connect with the community and got 3k followers in her twitter account. Before that, she even never had a twitter. As the followers increase, her art piece in NFT got more popularity. \yang{do we have more info about how she got popular or how she got 3k followers? the current quote is still pretty abstract. in general, more specific quotes are better}
\begin{quote}
    \textit{``I'm not an artist itself with, I didn’t draw a picture to sell it in the Gallery in real life. I entered this space three months ago and no one ever know me or saw me. I didn't have a Twitter profile before that. Now I have 3k followers. If you're open to be a part of the community and grow with the others, and you get a lot of followers in twitter and your NFTs get noticed.''}
\end{quote}
}


\noindent \textbf{Efforts behind NFT.} The amount of time and effort devoted to making an NFT was yet another simple heuristic in addition to reputation of creators: the more effort, the more value. P5 used the example of 3D animation, a time-consuming form of NFT art, to illustrate his opinions: 
\begin{quote}
    \textit{``3D animation basically is kind of the most popular form of content. People see value in it, probably because it takes a lot of time and effort to model things. So I think people tend to [buy/like it] when they see something that has taken a lot of time.''}
\end{quote}
% According to this participant, good NFT should represent the effort f

% In this similar context, P1 preferred a NFT to present a certain meaning that creator want to convey and creativeity as two main criteria of good NFT. \textit{``So I'd say the main criteria when I look at NFT arts [...] whether it's a good piece of art is originality, creativity and peacefulness. Sometimes a piece of art can be extremely abstract. But if it's done in a tasteful way and have meaning even though it doesn't contain that much imagery.''}. 

% This participant's preference of good NFT has a similarity with the conventional abstract painting which is a opposition to Renaissance model and figurative art \cite{leder2006entitling}. It contains the valuation of shapes, colors and textures which is subjective to and tangled with artists' emotion that prob audience to understand the meaning behind the work. 

% \noindent \textbf{Practical Utility or Not?}
% \yang{Having actual utility (e.g., NFT as tickets) was considered another criterion, find anther quote}. 

\noindent \textbf{Practical Utility} \yang{separate utility and meaning/vision.} Having actual utility (e.g., NFT as tickets, postcard) was considered another criterion for a good quality NFT among our participants. 

A heated debate about whether NFT should have utility or practical value behind it was noticed by P12. He personally liked the idea of having utility behind NFT, which gave NFT more possibilities:
\begin{quote}
    \textit{``Does NFT need to have utility behind it? Or can it just be digital art? Some people say an NFT is worth more if it has utility behind it. I know there's NFT like, if you buy it, you're able to get into a conference with it. There's a lot of debate happening there, but I personally like the idea of having utility behind NFT, cause there's a lot of exploration you can do there that hasn't been done yet.''}
\end{quote}

Many participants indicated how they used NFT as a self identity in the digital space. P7 thought NFT could be used as personal identities when making friends online, especially in the Metaverse \footnote{https://studio.gometa.io/landing}, which was a virtual shared space:
\begin{quote}
    \textit{''I believe in the future, people will spend more time on the Internet, in the virtual world, in the Metaverse. And in that world, people don't meet each other physically. People use their digital identities to make friends with each other.''}
\end{quote}

\noindent \textbf{Meaning/vision}. 

% Similarly, Bored Apes, which werev popular NFT avatars, were used as personal identities by members of some Clubhouse rooms. P7 told us that members of a Chinese-speaking NFT-related Clubhouse room used Bored Apes as their Avatars, which was seen by them as a sign of membership. This participant also mentioned an NFT-themed ``attack,'' in which they randomly entered other non-NFT rooms, and shouted like apes. The main motivation behind this ``attack'' was to ``let the non-NFT people know about NFT.'' P11 thought one day, a Bored Ape may be used as the digital identity to attend parties held by the community. 

% Similarly, P3 indicated the about this growing community with diverse people. He added that how he made friends within this short period and gained a large network. He felt that this community provided him the ability to reach out many people.

\subsection{Practices of NFT Users and Communities}
\label{5.2}
In our study, we have seen participants comparing NFT with 1995 internet revolution. P1 compared the NFT innovation to the 1995's in which Google and Amazon survived out of many other companies and proved to be successful. 
\begin{quote}
    \textit{``I think NFT is an extreme bubble right now. It's going to burst within this year. But I think every bubble has meaningful innovations. So just like the 1999 dot com [.com] bubble, we got Google and Amazon and other huge corporations right now which rose from the ash of that 1999 bubble.''}
\end{quote} 
Despite the huge bubble in the NFT marketplace, he thought good NFT projects would eventually survive.
\update{NFT has became popular only recently, and majority of our participants (10 out of 15) had less than 1 year of experience with NFT at the time of our study.
We observed positive attitudes in our participants towards NFT. They expected it to be the next art revolution and creative form of blockchain. Some emphasized on the implication of NFT to the future prospect of internet where people's interaction will be shaped by the idea of Metaverse. Our study also indicate inequity in social, community and market dynamics in NFT that could potentially have long-term harms to creators and overall community.
In this section, we will report both individual and community level practices around NFT and discuss possible implication to creators and this new marketplace.}

%\subsubsection{Individual and Community Engagement with NFT (RQ3)}
\subsubsection{Individual Engagement/practice of NFT creators (RQ3)}
\yang{it's hard to differentiate individual vs. community practices. many individual practices involve social media and online communities. shall we consider restructuring this section by focusing on how they use social media/online groups? are there cases where they get offline help/support/interactions?}

Our study presents different stories behind NFT creation to discover the engagement of NFT creators with their peers, buyers and NFT platform admin. \update{We also highlight specific creation workflow of different NFT creators as well as the openness and closeness of collaboration (i.e., drawing insights from others' art pieces, working with peers in a same art piece, etc.) in their ``Creation process.'' Further, we present creators' distinct in demand art media to create NFT, including, physical / digital media, AI, Data media, 3D, etc.}


% \tanusree{`\textbf{Process of NFT creation practice}'' can be divided into 2 types: a) once they initially joined, b) after a while when they are pretty regular in creating and selling --- maybe creating graph of these two types of practice in creation process.}

% \tanusree{`\textbf{use of media (3D, data, digital, physical), type of NFT creation practice}''}

% \tanusree{\textbf{NFT creation in terms of collaboration}. Looking at our sample participants, there are 3 types. One can be in more than 1 category. a) who creates independently, b) who draws insights and motivation from popular artist and make their own art, c) who creates with peers in same piece.}


%\noindent \textbf{Individual: NFT Discovery and Initial Engagement.} 
%\noindent \textbf{Practice: Process of NFT creation} 

\noindent \textbf{Process/Practice of NFT creation} \update{Our participants had mainly two different types of workflow in their NFT creation process: a) Process of NFT creation while they initially joined in this new marketplace, b) Process of NFT creation when they are become more experienced. Figure~\ref{process} present the NFT creation process for our participants throughout their early stage to date.} 


\begin{figure}[b!]
\caption{Process of NFT creation with resources for participants throughout their experience from early stage to comparatively experienced\tanusree{not final yet} \yang{for the more experienced stage, why do they still need to learn NFT terminology and blockchain concepts?} \yang{what do dotted boxes mean?}}  
\centering
\includegraphics[width=1.0\textwidth]{NFT-2.png}
\label{process}
\end{figure}


\update{\textit{During early-stage}, participants explained their creation process by their experience of discovering and joining NFT from a diverse range of information sources.} Some (P1 and P5) learned about NFT from online resources, such as YouTube videos, and some (P9, P14, P15) learned about NFT from news of record-breaking bids. P9 acknowledged learning more about NFT only after he saw its record-breaking bids and wide applications:
\begin{quote}
    \textit{``NFT became hot, and there were always record-breaking bids. [...] Then I noticed many applications of NFT in different areas, which motivated me to learn more about it in depth.''}
\end{quote}  
Some participants learned about NFT from their friends and family members. For example, P4's brother introduced NFT to her as a way to sell her tattoo designs online during the pandemic, when her shop was closed per the lockdown policy.
% :  \textit{``Actually, I'm a tattoo artist based in Berlin. During lockdown and pandemic we had to close our shops. My brother told me about NFT as a new way to share, and sell the pictures. That was my entry in NFT.''} 
% P11 started to engage with NFT with NBA-related airdrops to support his sport team. This initial experience also opened a door for him, and got him to start learning about NFT. Later, he became more interested in NFT when he noticed some NFTs are sold in millions of dollars. His interest in NFT was further enhanced after extensively reading articles about NFT:\textit{``I spend quite some time on cryptocurrency every day besides my work and study. Instead of focusing on the price, I pay more attention to some in-depth articles about cryptocurrency, which make me believe that NFT will have some real value in the future.''}

Participants also mentioned difficulties when they were initially creating NFT due to the lack of understanding of underlying blockchain concepts, especially for those who did not have a computer science background. For example, P12 thought NFT to be tech-heavy, and it took him  a while to understand the new terminologies. P6 explained that the crypto world was changing fast, and there was a lot to learn about NFT and general cryptocurrency when he first stepped into this field:
\begin{quote}
    \textit{``When I started working with this community of artists, I didn't understand anything about NFT and the crypto world. It's moving really fast, so I've been studying a lot since last year.''}
\end{quote} 
In their early stage, participants seemed to first learn about new terminologies (i.e. minting, wallet setup, gas fee, etc), underlying blockchain concepts. This scenario has a similarity with traditional software development where new developers face challenges in engaging due to new terminology and concepts \cite{aagerfalk2008benefits}. During their early stage, NFT creators tend to look for resources in youtube, twitter posts to learn by themselves. In many cases, as new creators, some participants were not aware of ethereum gas fees' irreversibility once minted and thus, lost their money by uploading incorrect NFTs in marketplace. P4 said-
\begin{quote}
    \textit{``From Discord server I got to know there are people who lost money in minting. It hurts the gas prices are the main issue on Ethereum. they didn't know that they can't get the fee back once minted with wrong art piece. I heard about the Ethereum new version is coming anf a lot of people are hopeful now.''}
\end{quote}



\noindent \textit{During comparatively experienced stage, \yang{more clearly define this stage}} \update{we also noticed similar types of difficulties when they becomes more experienced in this NFT marketplace. However, we noticed changes in their method of learning about NFT creation materials and media for seeking help. These practices becomes more organized as they did during their early stage. When encountered with bugs during their NFT minting process, queries on art media, they tend to ask to NFT community through discord, twitter or NFT platform admin for help.} 

When confronted with difficulties, it was common for our participants to seek external support from representatives of NFT platform. For instance, P3 had difficulty setting up a wallet and depositing cryptocurrency into it to mint his NFT. He asked the question on Twitter, and was directly replied to and helped by a platform representative, who helped him successfully mint his first NFT:
\begin{quote}
    \textit{``It was actually kind of difficult to set up a wallet on that blockchain, and to deposit the cryptocurrency. I asked around and tweeted about my challenge. And then one of their representatives directly replied to me, and was able to help me.''}
\end{quote}

\update{Here, the admin of NFT platforms directly help NFT artists. Participants referenced discord, Telegram online forum as their most frequently places for seek for help. Majority of participants seemed to be a part of a small local or global NFT community within a few months of their experience in this community. Rather than learning NFT creation resources and trend by themselves, they tend to rely on and discuss with NFT community for suitable resources. P3 said-
\begin{quote}
    \textit{``After few month of joining, I am on many different discord groups. So I think the overall. Norm is supporting each other and pointing out potential problems and sharing resources to help in creating. I have never met such a community who's willing to grow each other with each other and not.''}
\end{quote}}

We found NFT creators to follow different approaches while creating NFT. There are some participants who creates NFT independently, one who draws insights and motivation from popular artist and combine into their own art, c) one who creates with peers in a same piece of art. A participant can be in more than one category. 

\noindent \textbf{Differences of types/media in individuals' NFT Creation.} 
\update{Different forms of NFT were created by our participants. NFT creators have their distinct in demand art media to create NFT, including, physical / digital media, AI, Data media, 3D, etc. Further, some participants preferred to mix traditional art with digital media.} For instances, P1 liked to combine NFT with traditional paintings, with the help of AI tools (he chose not to share the specific information which he thought was ``private''), and expressed his dislike of purely digital art:
\begin{quote}
    \textit{`` I've always been a fan of fine art that was made in the 1600s, 1700s, 1800s. I'm not a huge fan of the overly digital art that's very popular now. It looks a little bit childish.''}
\end{quote}
On the contrary, some participants preferred purely digital NFT. P4 created 3D digital duckies with different colors, textures and costumes using Blender, a 3D computer graphics software. 
Some preferred NFT with practical value. For instance, P10's team combined NFT with VR:
\begin{quote}
    \textit{``We created immersive VR scenarios such as an office, a cinema, or a pub. They're especially useful during the pandemic when you stay home every day. It's different from just sitting in front of your computer, because it requires you to interact.''}
\end{quote} 
He thought such NFT had more practical value in life than other popular ones such as NBA player cards which were ``merely for collection purposes." 

While the participants mentioned above made NFT from scratch, others may recreate NFT out of their earlier artworks. For example, P13, a landscape photographer, created NFT based on his own pictures by adding animation and other digital effects. Similarly, P14 minted NFT out of his design works which he created before. 


% \tanusree{one paragraph to explain the 2 points below}

% \tanusree{how they choose different types/content for creating NFT. what influence their decision. Their can be some personal, ethnicity background or political flavors that influence their art contents. need to analyze that.}

% \tanusree{how they make the balance in their created content. A balance between the topic they are interested in creating (capable of creating) and the topic that can be rewarding financially. Some criteria they followed in the creation process.}


% \noindent \textbf{Practice in collaboration for NFT creation.} 
% \update{In terms of collaboration, our participants had mainly three types of practices while creating NFTs, a) one who creates NFT independently, b) one who draws insights and motivation from popular artist and combine into their own art, c) one who creates with peers in a same piece of art. A participant can be in more than one category. \tanusree{will add 3 quotes for these 3 types}}

% Participants are found to create some NFT to give way in social media just to promote their overall collection. P3 created an interactive digital model of an abstract sculpture as a giveaway on his Twitter page for promotion purposes. 

% NFT creators from our study don't usually disclose information regarding and considered their art media to be very private unlike traditional art market where the media such as, acrylic, oil, water color are clearly defined. During our interview when P2 was asked about the media they used for NFT, he stated that. \textit{``I sold my NFT for 0.777 ETH within 26 minutes, It's called mountain elephant- AI generated piece of art. But, I I can't share that information on tools and studio. It's private.''} Though this community seemed to be supportive to each other, it appears to be a competition in this market to sell NFT. In regards of NFT creation, we observed collaboration between NFT platform designer and NFT creators. 

% P9 was an NFT platform designer/developer. Through the platform she built, she collaborated with known artists, and created and sold high-quality NFT paintings: \textit{``Our platform takes the role of ensuring quality of NFT. We collaborate with known artists who have reputation and popularity. We mass produce, say 100 NFTs mimicking the style of their paintings with machine learning techniques. All the 100 NFTs have the gene of the original painter, but the production rate can be much higher.''} This present the engagement among people in different hierarchy in NFT platform to ensure the quality of NFT. 

%\noindent \textbf{Community: Mutual Support in the Reciprocal Community}

\subsubsection{Community Engagement/practice of NFT Creators (RQ3)}
\update{NFTs represent an unprecedented opportunity for independent creators to promote their projects, a space for NFT creators to support each other and provide alerts on potential scams, with the collective goal of forming a sustainable marketplace. Meaningful community engagement is something that large corporations spend substantial amounts of money chasing, and often without success \cite{}. In this section, we discuss NFT community practice/engagement for communally greater financial independence. We also highlight community practices and pitfalls that can lead to the distortion of art creation and harms other industries.}

\noindent \textbf{NFT Promotion and Community Building Practice.} Our participants mentioned discord channels of mainstream NFT projects as their main media to promote their NFT. Many participants mentioned promoting their work within the community. P1 said:
\begin{quote}
    \textit{``If you're the owner of a personal [NFT] project, you can talk to your community via discord, engage with them, and answer any questions of potential buyers.''}
\end{quote} 
\update{In addition to Discord channels, NFTs are promoted from NFT creators Twitter account as well his as well as other community members' (creators'). P2 also used discord channels as a place to connect with buyers, and understand their preferences for NFT. Later, he used those insights into NFTs to capture the market trend and better met the taste of the market.} 
\begin{quote}
    \textit{``I'm in 15 Discord channels. There are members who are buyers. It’s great to connect with people, knowing what type of work they like, so I can import those in my NFT.''}
\end{quote} 

Reputed NFT projects owner, such as MeetBit, Crypto Punk and NBA TopShot, also promoted their projects by actively organizing events and attracting people into their community. P5, who was the owner of an NFT company, was organizing an online event at the time of the interview to promote the NFT game they created. 
\begin{quote}
    \textit{``We're throwing an event to open our gallery in Decentraland. Our main focus right now is sort of building the community and developing our brand.''}
\end{quote} 
\update{In addition to promote NFTs, many NFTs creators hold meeting to help other creators to learn new NFT contents, such as, gaming, 3D arts.} P5 mentioned that he enjoyed creating ties with the community by streaming on Twitch\footnote{\url{https://www.twitch.tv/}. Twitch is a live streaming platform.}: 
\begin{quote}
    \textit{``Now we stream on Twitch almost every day, spending hours in the game (Decentraland), meeting people, and then helping them learn how to play NFT games and create content. Creating relationships with the community and then building things together is a lot of fun.''}
\end{quote} 
Such community building and promotion efforts were shown helpful for the development of NFT projects, according to our participants. 

\update{Besides these community ties and support, majority of participants mentioned that NFT creators come to this NFT marketplace for different intention. Some comes with malicious agenda to trick the system with solely business purpose (i.e. poor quality NFT), not thinking of the well-being of community. P1 said-
\begin{quote}
    \textit{``Some people don't care about quality, just posts anything on Twitter, spam link to promote and extremely desperate for people to see that piece of work. Their art, I wouldn't even call it art. It's like something that you'd make within 20 minutes on Photoshop. However, in the long run, they will not sustain in this marketplace because they are shaddy.''}
\end{quote}
He mentioned about some creators to be shaddy in their communication with peers and providing wrong information on their NFT contents. On that note, P8 added that NFT place is growing and thus, it will make those shaddy characters to be outlier in the long run. As a reason, he explained that NFT community/circle prefer to grow with people with similar intention, who will be in this community for a long time and being their authentic self.
Participants suggested to new comers' to be their authentic self while creating NFT and having long term goal rather than impatience in quickly making money.}


\noindent\textbf{Chained Support among Artists} In the NFT community, there existed a ``chained'' support system where artists helped each other to grow. P12 identified himself as a ``community-based person'', and liked engagement through resource sharing. He mentioned how community members including creators and admins helped each other to succeed in this field:
\begin{quote}
    \textit{``Everybody gives me a sense that they really want to help you succeed. They're very open. If you're a newbie and you have a very simple question that you just don't know, they never try to put you down. It's a very giving community.''}
\end{quote} 

Some participants mentioned showing support to new creators by buying their NFT. P4 mentioned buying a NFT of a new artist. He added that other community members did the same thing:
\begin{quote}
    \textit{``There's part of the community that will buy your first NFT. They just want to get you started. Some think that you might become something really big, so they buy your first NFT. And others are doing it like `hey, let's just get you started. Let's get you moving, get you excited, give you a little push.''}
\end{quote} 
% Some of the responses also showed that NFT artists/creators tended to give back to the community by buying other artists', specially new artists' NFT to encourage them. 
P1 also did such a thing to show support/encouragement to new artist, to give back to the community, as well as to help grow the NFT marketplace: \yang{sounds like reciprocity}
\begin{quote}
    \textit{``I set up a goal in my mind: when I reach a milestone, I'll give back to the community by buying an NFT. And after I sold my first NFT, I bought one back.''}
\end{quote} 
P4 enjoyed collecting different types of NFT and supporting other artists at the same time: 
\begin{quote}
    \textit{``I think a big part of my incentive to buy an NFT is knowing that money go directly into the wallet of someone who I think does cool work and who I want to support.''}
\end{quote} 

P2, who just bought a GIF work from a less known artist to show support, mentioned another reciprocity behavior, i.e., follow-back, among artists on Rarible:
\begin{quote}
    \textit{``When you follow an artist on Rarible, often he would just follow back. I also do this on Twitter, by actively commenting and reacting.''}
\end{quote} 
Such reciprocity and mutual support could benefit the growth of each individual artist, as P4 said,
\begin{quote}
    \textit{``I entered this space three months ago. I didn't have a Twitter profile before that. If you're open to just being a part of the community and growing with others, then you get a lot of followers and friends there to support you.''}
\end{quote}

\update{Despite the chain support among NFT creators, a group participants mentioned lack of trust towards some peers due to the anonymous nature of their account. Underlying blockchain provide NFT creators to preserve their personal information and be anonymous. P8 thinks that many new NFT creators use alias name to add a safety layer and hide behind. As a reason, he mentioned lack of confidence of new artist. He encountered discomfort of communicating with peers who once asked him for help. There is a phenomenon to use avator as NFT profile and P8 was not very comfortable in sharing his NFT art experience without knowing who he was talking to. 
\begin{quote}
\textit{``Some new people use pen name for safety. It might be okay because the NFT platform allowing it. But the phenomenon of avator and not knowing who is behind it makes me trust less. once a guy asked for help to create a piece, but I was not comfortable, you don't know who is behind. He had lack of confidence as new artist. maybe thats why he was using pen name.''}    
\end{quote}
}



\noindent \textbf{Alerting the Community about Scams.}
In addition to promoting NFT and showing support, community members also proactively discussed and alerted about recent NFT scams to prevent potential victims from falling to them. Our participants mentioned that NFT traders/collectors would share their recent experiences of NFT purchasing in great detail, including those of scams (P11). P3 provided such an example:
\begin{quote}
    \textit{``It's a community [..] pointing out potential problems in addition to supporting. For example, recently, someone was going around scamming a lot of people and taking their money. Almost everyone in the community was talking about it and saying, `Be careful. They're stealing money.' I think overall it's the norm.''}
\end{quote}
Sometimes platform admins and moderators also remind community members of potential risks reported by other members.

\noindent\textbf{Getting Technical Help from the Community.} 
There are different challenges and drawbacks for our participants, especially when they were experiencing newly launched NFT projects and marketplaces. Server and site crash, minting issues and technical ignorance were just some of the challenges. They explained how platform admins and community members helped them to overcome those difficulties. P15 mentioned how he got help from the community to learn the process of minting NFT, and connecting to his crypto wallet while he faced difficulties due to his language boundary.
\begin{quote}
    \textit{``I'm not a native English speaker. But when I try to connect with other people, they usually helped me to understand how to post, how to release artworks, transaction fees, and how to minting NFT. And it's amazing to get help from a lot of people from all over the world.''} 
\end{quote}
When P11 encountered technical issues, he got direct help from a project owner in Discord: 
\begin{quote}
    \textit{``I had some issues in minting an NFT. So I asked questions in the Discord channel. Then a founder of the project directly sent me some ETH, and asked me to use it as the gas fee to finish my transaction. The project became a success later, and I realized the founder was such a famous person. He solved my issue himself! I didn't believe it until now''}
\end{quote}

% P7 thought community building was a key to the success of NFT projects, and mentioned the friendly atmosphere in the community:
% \begin{quote}%     \textit{``I believe the success of some NFT projects like CryptoPunk or bored apes is because they create a big community with friendly atmospheres. Some of them are in Twitter and some of them in Clubhouse... In a Clubhouse room, many of us have the ape avatar, and we're like a family. We spend a lot of time talking about our apes. I really like that atmosphere. 
%     % And even in the recent days when the crypto market is bearish, we still have some topics about apes, and the atmosphere in our room is positive. So I think that's the power of NFT projects. That's the power of an active community. The community people are doing some efforts about the apes and  these NFT projects.
%     ''}

%\tanusree{need to decide if we want to keep this theme since we planned to only focus on NFT creators} \zhixuan{I commented this part out for now. also not that exciting}

% \noindent \textbf{Practices of Buying/Collecting/Trading NFT.}
% We observed participants to different types of NFT. P11 bought NFT of virtual land and other relevant elements in a decentralized sandbox game\footnote{A sandbox game is a video game which gives players a great degree of creativity to complete tasks towards a goal within the game.}, which made him a ``landlord'' and allowed him to rent land to other players: \textit{``I can create new things on my land like a manor owner. You can rent your land to others. I rent a piece of land to another player, and he uses the land to run his own business.''} He once researched on a horse racing game, in which one could buy his own NFT horse, or bet on the outcome of blockchain-supported races. He later decided not to play the game, because he thought it was too centralized: the rules could be easily changed by the developers. We found several holders (known as ``holders'' in the crypto community) in our participants. P3 had not resold any of his NFT collections, just holding and appreciating them: \textit{`` I would say I'm more of a holder right now. I haven't really resold any of them, like putting them in the secondary market. So for me it's more about collecting work from friends and things that I like. I just hold and appreciate them.''} Similarly, P11 had not sold any of his collections, even for the ones whose price had dropped by 95\%. We also found NFT buyer and traders to collect NFTs and speculate that the price will go up. P8 regarded himself as an NFT trader, and decided to hold his NFT collections and sell them in the future when the price went up: \textit{``I've not sell any token, so because I actually want to see how it grew better in future. I'm actually trying to wait for a few more years from now to start selling.''}

% P4 said he was also a business person/marketer in addition to a creator:\textit{``I definitely see myself as a creator. I've collected a couple of NFTs, but I'm more of a creator. I mean, I'm an artist, but I don't really think like an artist. I think more like a business person or like a marketer.  And that's what I mean. One interesting thing is a lot of artists don't necessarily think that way.''}He was honest about his will to make money, and thought of his self-identification of a trader as an advantage compared to other artists:\textit{``So that's I think that's one advantage that I have. A lot of artists hear about the NFT thing and they want to capitalize on it, and they want to make some money. So you have a lot of people coming into the NFT space. They don't know much about crypto at all. The only thing they know is how to list their artwork on Opensea or Rarible or these different NFT platforms.''} % P11 collected several types of such as a 3D NFT of a singer playing the guitar, which he thought could potentially be used to connect the virtual world with the real world, e.g., as an access to enter his concerts in the future. % We also found NFT collectors, P3 who collected a diverse set of NFT genres, including 2D and 3D collage, computer- and code- generated work by generative artists.  % As a musician, P15 was planning to release his album as an NFT, since crypto music was a new thing to him.


\subsection{Challenges in the NFT Marketplace (RQ4)}
NFT was a relatively new phenomenon, and the marketplace was far from mature. 
% We had a diverse set of participant from different countries, educational background and age range. 
% It appeared that there was a lack of support and open information for newbies. There is a fear of loosing money on NFT which arises from lack of information and comprehension of NFT concepts among non-English speakers and people in different age range-\textit{``in fear of losing a lot of money and a lot of time for NFT,''}- as P15 commented.
According to the participants, they were confronted with many challenges including (a) assessing good artist and artworks, b)lack of regulatory and moderation mechanisms c) challenges in using existing system consisting of tech-heavy blockcahin concepts and new terminologies.

%\noindent \textbf{Tensions between Decentralization and Quality} 
\noindent\textbf{Lack of Assessment metric for good artist and artworks}. 

\yang{this is very relevant to the earlier section on criteria for good NFTs. somehow we should combine them}

\update{While the underlying blockchain is supporting NFT creators to create their own business model to ccreate and sell NFTs without an intermediaries, it also greatly lowered the barriers for artists to entered this marketplace. Creators are now empowered to create and promote their NFT freely without gatekeepers as such traditional art markets. This phenomena, on the other hand, gives rise to low quality NFT. Besides, the blockchain layer to authenticate artworks, there lacks regulatory standards to authorize and assess artist throughout their activities in the marketplace, which in turns, leading to the prevalence of scams and low-quality NFT. Participants in our study indicated that low-quality NFT could be attributed to the lower barriers to entry of the NFT marketplace compared to traditional art markets, as P1 said--
\begin{quote}
    \textit{``They just spam their link. They're extremely desperate for people to see that piece of work, and most of those people, actually, their art isn't actually that great. It's something that you'd make within 20 minutes on Photoshop. Unfortunately, that's because the gates are open and they are not accountable for anything.''}
\end{quote}
Participants mentioned that Low-quality NFT became a demotivating factor for legitimate creators. For example, P13 was demotivated and upset by the fact that artists who created lower-quality NFT than him sold better. He also added that there is no mechanisms in NFT marketplace to assess good artist and artwork: 
\begin{quote}
    \textit{``So most of the best-selling artists are not really good photographers. And I sold, since last month, nothing. That's a little bit demotivated if I see other guys are selling, even if they are worse than me.''}
\end{quote} 
This is also similar for P5 who was also demotivated by seeing people sell low-quality work, since he put a lot of work into his own NFT. He also added that many malicious NFT creators copy others' work and create NFT. Since buyers are not aware of this fact, so, they tend to buy NFTs from them.

P8 mentioned a metric to discover and assess good artist or artwork which is reputation. According to him, NFT created by reputable artists could better serve speculation purposes, due to popularity of the artists. He added that people would buy NFT created by well-known artists as they perceived them as talented, even without giving much thought to the actual quality of the recent NFT. According to this participant, Beeple was talented and successful in delivering trending content in 3D art, and people would buy his work no matter how good it is. : 

\begin{quote}
    \textit{``His name is spelled BEEPLE. He's the biggest artist in 3D art. It's 3D animation, the most popular form of content. And people see value in it. [...] So I think people tend to like/buy things [...] created by someone talented, regardless of whether it's good or not.''}
\end{quote}

In many cases, including this participant, social media (especially Twitter) followers are one of the main indications for our participants to assess the reputation of an artist. So, either being already well-known or having twitter followers are some of the metrics to assess artwork. P4, who is a tattoo artist, shared her experienced how her NFTs got popularity within a very short period of time in her twitter account. As the followers increase, her art piece in NFT got more popularity.
\begin{quote}
    \textit{``I never draw a picture to sell it in the Gallery in real life. I entered this space three months ago and no one ever know me or saw me.[...] Now I have 3k followers in Twitter and my NFTs get noticed.''}
\end{quote}
}
However, there is no defined metrics of how to discover and assess good quality artwork and artist in this NFT marketplace. 


\noindent\textbf{Blurred moderation mechanisms in NFT}.
\yun{Instead of regulation, you could mention something like "Blur Moderation of NFTs." Basically, content moderation needs human-AI collaboration, there has been works defin- ing the stages of training human moderators, e.g., Seering 2019 paper on moderator engagement, and there are many moderation rules (e.g., Casey’s paper on Reddit Rules!), but I wonder if it is clear for NFT communities? you may look at the blocks for general online communities’ moderation, then point out that new building blocks may need to
be added.}
\update{Our Participants mentioned that malicious users frequently posted scam NFT (which were not NFT at all, or copies of famous and expensive NFT) in Discord channels of mainstream NFT projects, and on Twitter. From their experience, scams cost huge losses. P2 knew one person who fell for a scam NFT, which cost him 11 ETH (worth of tens of thousands of dollars). P7 explained how a scam NFT was made, the process of which was as easy as copying existing images, adding a few new features, and minting it on NFT platforms:
\begin{quote}
    \textit{``People can copy an image, photoshop it to add some new traits, and mint it on Opensea. It can scam people by showing that this is the original one, but actually it's altered by some random people.''}
\end{quote}
Unfortunately, mainstream NFT marketplace doesn't have moderation mechanisms to handle NFT scam that violate copyright, such as malicious actors to use exiting NFT, add adding some feature and claim those to be their creation.} P7 and P11 mentioned a special type of scam on Opensea, which arose from design issues of the platform: since the icons for different cryptocurrency were not distinguishable from each other in the bidding process, some malicious buyers claimed to bid in Ethereum (worth of thousands of USDC), but eventually paid in USDC (worth of approximately 1 dollar), which led to a huge loss to sellers. They thought such scams could be avoided if platforms improved their moderation designs and provided some forms of alert to users.

P4 thought of the high gas fee on Ethereum as a moderation measure for the market: \textit{``If the gas fee keeps this high, it may stop some trash (low-quality) NFT from being posted.''} However, such a  measure was against the inclusiveness of NFT, showcasing the tension between inclusiveness and quality. P2, P10, P15 all mentioned that high gas fee and minting cost put a heavy burden on NFT artists. 

NFT platforms propose ways to moderate scams and low-quality NFT. For instance, Rarible asked new users to verify their Twitter accounts in the onboarding process (P2), which was mostly a KYC process in centralized platforms. However, this was not mandatory rather for those who would like to enjoy more visibility on the platform. P11 mentioned that Foundation adopted another mechanism, i.e., invite-only, to restrict low-quality NFT in its marketplace. P11 felt more confident about the quality of NFT on Foundation compared to other platforms:
\begin{quote}
    \textit{``If you want to join, you've got to have someone invite you.[...] When the platform just started, there were only several known artists. Only those invited by them could join, and could further invite 2 or 3 other artist, like a snowball. So I feel assured about the quality of NFT on Foundation.''}
\end{quote} 
However, again, the invite-only mechanism may hurdle the inclusiveness of NFT. For example, P5 perceived this as a barrier for many artist to enter the NFT space. He also mentioned that the invitation process could be biased, and may include not-so-good artists as well. 

Manual checking was another human-intensive manner of coping with low-quality NFT by the platforms. P4 mentioned a scenario where he reached out to the admins of the platform to report a copyright violation incident: \begin{quote}
    \textit{``[If the copyright is violated] I will either message staff members about this, and they may take down the work after investigation. Or I would tweet it, so that more people get to know.''}
\end{quote} 
P6 also mentioned an artist being banned for selling copies on Rarible, which were taken down by Rarible's manual inspection efforts. P8 noted that Theta moderators would check each transaction, including the buyer and the seller, to mitigate the process of any act of scams. However, this process of manual moderation seems to be labor intensive given that this marketplace is growing. Some private NFT project, i.e., P10's team would automatically filter out NFT irrelevant to VR, using off-the-shelf AI technologies developed by Baidu and Google. 

\noindent \textbf{Complexity in using Existing system}.
\update{Our participants repeatedly reported challenges regarding the sophisticated concepts of blockchain technology and new terminologies in NFT. Newbies found it especially challenging in initial engagement. 
% Some participants mentioned that different age groups (older) in the community face difficulty to grasp the concept of NFT and how it works. 
Such features of the NFT marketplace made the engagement with NFT intimidating for many. For example, P12 had many ideas in art and design, and wanted to play with the NFT marketplace. However, the minting process of NFT seemed too hard for him. He watched YouTube videos to grasp the concept, however, those contained too many technical details  and far from instructional for lay people. 
% He was hoping those to be breaking down in common language, step by step for general users. 
He elaborated,
\begin{quote}
        \textit{``In my opinion, NFT is still pretty tech heavy. [..]They're almost speaking another language and system is complicated, doesn't have guidelines. So,I've watched YouTube videos and they don't make sense, not instructional at all [..] Without knowing the details, it gets a little hazy when I'm going to put some money in in crypto.''}
\end{quote}
On that note, P4 suggested making NFT less intimidating and more newbie-friendly, especially for older adults and even new NFT creators who were not familiar with virtual assets. The current NFT platform design is challenging for participant to mint (upload in blockchain) their NFTs. The platform doesn't include any instructional guidelines for creating and promoting NFT. Some get demotivated when they couldn't sell their NFTs in their first few months due to lack of resources. He added that the NFT marketplace should have a directory for new creators to learn about different tools to improve artwork rather than wondering around different online group. As the implication, this will help new artist to learn about tools to create and promote NFTs since the early stage is the most challenging time when one can feel demotivated due to lack of strategies to promote, sell and create NFTs.

P2 explained difficulty in communicating business idea around NFT with other people (in different age groups), i.e., some of his business partners don't comprehend the concept of NFT well to invest. This suggests to improve design and implication of NFT space for broader audience. 
\begin{quote}
    \textit{``You're in university, and you must be in your early 20s. The idea of owning a digital good in a video game is a natural thing for you. But for my generation, and especially the generation above me, it's like a foreign language. The number one thing that comes to my mind is making it less intimidating.''}
\end{quote} 

Since NFT was built on top of blockchain especially Ethereum, several drawbacks/challenges of it were related to the nature of the blockchain technology. Though irreversibility of blockchain/NFT prevented malicious users from tampering the data and controlling the market, this feature could also lead to some inconvenience for artists. For instance, P1 noted that if mistakes were made during minting an NFT, there was no way to restore it:
\begin{quote}
    \textit{``Let's say, you're preparing for an NFT, and you mint it out. And then two hours later, you realize you've made a typo, or you've uploaded the wrong file, or the cover isn't the exact cover you wanted. It's set in a stone, so you can't edit it. You can't change it. Let's say you accidentally burned an NFT, then there's no way could it be restored. It's gone forever. So it's both a blessing and a curse.''}
\end{quote} 
Participants also mentioned their issues around trust in fellow NFT creators/ community when anonymity is a built in feature of blockchain technology. According to P8's experience, he was uncomfortable with fellow NFT creators who acted suspicious behind avator. He said- \textit{``Its not always comfortable to help fellow NFT creators with resources when they always hide behind the avator and their interaction in the community group is not satisfactory.''}
}
%\zhixuan{the platform bug thing seems not that exciting, commented out for now}
% Participants also mentioned some security risks and bugs from NFT platforms. Since many NFT platforms and projects were new, even in their infant stage, thus there were constantly bugs and technical issues. For some participants, it was understandable for a new platform to have bugs, given that NFT was a new realm. For example, P5 mentioned about bugs due to huge traffic. He explained it as a issue of scalability than security:\textit{``They're kind of buggy, but that's only because they've experienced a huge amount of traffic and users coming onto their platform in the last two months. they've had to scale their platforms considerably up.''} However, P3 was concerned about trustworthiness of new NFT projects, which were lacking in consistency and stability:  \textit{``I think a lot of the platforms are still very new, and so there's constantly changes happening,a lot of bugs, and some sites get crashed and go down. Then along with that, there's a lot of new projects that pop up, and it's hard to gauge how trustworthy a new project is, and whether to actually invest in it or not. So in that way, I'm a little bit concerned.''}. Platform instability made this participant to question the trustworthiness while he spent money on it. According to him, when crash happens and sites goes down, there remains always concerns since NFT is based on decentralized governance and if they loss money, there is no specific ways to recover that.

% \review{it could be something design aspect}% P3 pointed out the lack of full control and features in different NFT marketplaces. As a result, he had to shift between different platforms. He thus called for a comprehensive platform with smart contracts which could support more functions:% \begin{quote}
%     \textit{``I think I have yet to see a marketplace that is 100\% control, like able to be controlled by the user, like you can adjust every single parameter. There's no platform with all features [...] so you have to split between different platforms. I would love to see one NFT space with unlimited capabilities, so you can use it very simply and straightforward.''}
% \end{quote} 

%\review{\textbf{need to present/ reflect the significance of this finding}-- result Similarly - varied views between participants is rarely expressed or teased out. For example, there is a clear tension between the desire for open access to NFT markets, the desire for high-quality works, and some form of regulation. But this is not reflected in the findings particularly.}\zhixuan{framed a section into tensions between decentralization and quality}


\begin{comment}
\noindent \textbf{Other Blockchain-Induced Challenges.}
Since NFT was built on top of blockchain especially Ethereum, several drawbacks/challenges of it were related to the nature of the blockchain technology.
% P3 thought of extensive energy consumption and negative environment impact as frustrations induced by the Ethereum blockchain:
% \begin{quote}
%     \textit{``I do have concerns with the environmental impact of the Ethereum blockchain. The first thing they say (about Ethereum) is that, `oh, it's bad for the environment.' That was one frustration. I wish there was a better understanding of how exactly it impacts the environment, and whether there're alternatives that don't have the same energy usage as Ethereum.''}
% \end{quote}
% P6 also mentioned the negative effect of Ethereum blockchain on global warming. He tried to improve the quality of his NFT, to make up for his addition to global warming:
% \begin{quote}
%     \textit{``Instead of focusing on my profit, I'm more on the quality of my work. 
%     % Because I believe that in the long term, that's gonna make some profit. I tried to balance that, you know. 
%     If I'm gonna contribute to global warming, then I'm gonna try to make something that's not so harmful.''}
% \end{quote}
Though irreversibility of blockchain/NFT prevented malicious users from tampering the data and controlling the market, this feature could also lead to some inconvenience for artists. For instance, P1 noted that if mistakes were made during minting an NFT, there was no way to restore it:
\begin{quote}
    \textit{``Let's say, you're preparing for an NFT, and you mint it out. And then two hours later, you realize you've made a typo, or you've uploaded the wrong file, or the cover isn't the exact cover you wanted. It's set in a stone, so you can't edit it. You can't change it. Let's say you accidentally burned an NFT, then there's no way could it be restored. It's gone forever. So it's both a blessing and a curse.''}
\end{quote} 

Another major challenge for NFT creators and traders was the high gas fee on Ethereum, which made minting and transacting expensive. For example, P2 sold his NFT for \$1800 CAD, but only earned \$700 CAD after paying the gas fee. P4 regarded the high gas fee as a major issue of Ethereum: 
\begin{quote}
    \textit{``I think the gas price is the most important thing for artists, because it's a lot. OpenSea, for example, you can mint for free there, but you still have to pay gas prices. I think the gas prices are the main issue of Ethereum.''}
\end{quote} 
According to her, artists had to sell NFT for a higher price, in order to compensate for the fee during minting and transacting.
% :
% \begin{quote}
%     \textit{``And the gas is really high, so yeah, you have to sell it for a higher bit. It makes sense for you that you don't pay for selling the NFT. And that's a little bit complicated. Yeah, gas price is too much nowadays and it's like increasing everyday now.''}
% \end{quote}
% \begin{comment}
%  He thought the high gas fee may scare some new artists and traders away:
% \begin{quote}
%     \textit{``Now I can't say everything is amazing, because I'm not like the other artists who're not speaking the truth. No one likes to speak about gas prices and how much people are really making. In total I've sold around \$1800 CAD but only got \$700 CAD because of gas prices. Pretty insane number that most people don't talk about, because it scares people away. Not saying that everything is bad, because jeez I'm saving for college, and \$700 bucks is \$700 bucks.''}
% \end{quote}
The high gas fee on Ethereum affected P3's opinion for NFT. He did not like the facts that some people did not have enough money to participate, and that artists were not gaining proper monetary return: 
\begin{quote}
    \textit{``I think the price right now on the Ethereum blockchain is very high. It turns me away from NFT a little bit, because it looks kind of exclusionary. Some people who don't have money can't participate, so I don't like that... I think one thing that initially discouraged me was creating a lot of work and putting them up for sell, and then not having any actual monetary return.''}
\end{quote}
% The gas fee varied in different places and times. It could be extremely high in peak hours and in countries where NFT was popular. For P1 who lived in UAE, gas fee was less of an issue:
% \begin{quote}
%     \textit{``It depends on the time we're looking at. So fortunately, for me, I live in the opposite side of the world where NFT are most popular. So when I mint out my NFT, most of the Western world are asleep. So the gas fees are extremely low compared to the peak hours when gas fees are almost \$180. I average around \$70 in gas fees.''}
% \end{quote}

% \end{comment}
\end{comment}

==> section/4_Findings.tex <==
\section{Findings}

\review{Both in their method, and limitations, but also throughout the findings, I feel the authors could be much more careful and critical in how participants' views are presented and analysed given this investment.
}


\review{ In particular, the authors do not ask for any of the participants' experiences with non-NFT markets which I believe limits our ability to interpret the feedback of the participants. Secondly, I think this interview protocol is too focused. NFTs and blockchain technologies have a number of impacts and qualifications to their function such as issues of piracy topics, among other impacts of blockchain, in the interview protocol, as well as the fact that the participants were already participants in NFT communities, makes me somewhat suspect of the picture that these interviews are painting wrt to the general sentiment that these interviews are painting. Maybe it is valid to say that participants just aren't thinking of those issues, but I do think some discussion by the authors of that fact is necessary. Concern level - P1.}

\review{Overall I found the results section easy to read and well structured; however, it’s a lot of information. If the authors continue to present all the themes in a single paper I would recommend organizing them in a table with short descriptions.}


We now present 1) our participants' perceptions of NFT, %including their understanding of the NFT concept, perceived characteristics of NFT, their standard for good NFT, as well as perceived challenges and drawbacks facing the NFT marketplace, 
2) their motivations for creating, trading or interacting with NFT, and 3) their individual and community-based NFT practices.
% \yang{too many findings. what are the 2-3 most important/interesting findings?}

%\yang{we might need to differentiate different types of users first: creators, traders, etc.}

\subsection{Perceptions of NFT (RQ1)}
Here we will present our participants' understanding of NFT, their criteria for good NFT, and their perceived limitations of NFT.

\subsubsection{Users' Understanding of NFT}

Our participants saw NFT as something unique, and as a way of verifying ownership of items, empowering artists, collaboration, and representing digital identity. 
% refers to the expertise of explaining the underlying concepts of NFT. In this study, it refers to how the participant understand the process and can make a person (who don't know about NFT) to understand the purpose of it in a given context. The norms refer to something that represent the standard for individual's pattern of social behavior, preference when included in a community. Such knowledge and norms are deeply rooted into specific contexts. From our interview, we divided this into three facets: 

% \textbf{Explaining Concept and Characteristics of NFT.} %When we asked the participants to explain NFT to a lay person, they revealed their personalized understanding of the NFT concept. 

%While NFT is a recent phenomenon, our participants had a fair amount of knowledge of it. Their explanation represent different perceptual model around NFT, including, ownership, unique trait of artist, empowerment for artist, place of collaboration and scope for self created business model.  

%\yang{I'd suggest highlighting and distinguishing what's correct understanding and what's misunderstanding.} \tanusree{From my understanding, none can be identified as they are misunderstanding NFT, but we can say how many are explaining it comprehensively}
%\yang{report how many participants had reasonable understanding of NFT} 

\vspace{3pt}
\noindent \textbf{NFT is Unique.} 
NFT tokens are non-fungible, which means each NFT has some special trait, while fungible tokens (e.g., Bitcoin) are the same, and can be divided. Four participants (P1, P5, P7, P8) mentioned the non-fungible and unique properties of NFT in contrast to fungible tokens. 
%were able to distinguish different features between NFT and Bitcoin. 
% 
%For example, P1 pointed out that every Bitcoin was the same, while NFTs were created by different creators: 
%\begin{quote}
 %   \textit{``Well Bitcoin, every single Bitcoin is exactly the same. The only thing that's different is the code. But when it comes to an NFT, first of all, it has different creators. So basically, Bitcoin comes out of nothing, basically, but when it comes to NFT, someone made or at least something has made it and it's intentional. It has customization built-into words, and as I said, it has digital files attached to it to give it value.''}
%\end{quote} 
%P2 complemented another difference. According to him, Bitcoin had a fixed supply, but there was not a supply limit for NFT: 
%\begin{quote}
 %   \textit{``I'm familiar with Bitcoin, and have basic knowledge of smaller tokens. Bitcoin is like digital gold. The supply remains the same. Ethereum (where NFTs are created) does not seem to have a supply limit. Unlimited number of NFTs can be created.''}
%\end{quote}
P7 saw fungible tokens as a way for speculation, and NFT as art with special traits, for which people may have emotions associated to it:
\begin{quote}
    \textit{``Fungible tokens are more for speculation, and people trade them like stocks. They have very good liquidity. But non-fungible tokens, most of them are kind of art. When people buy one of the tokens, people will see that this token has some special traits. Each one of the tokens is very different. If you own one of them, you have some personal emotion for it. Maybe you use it as an Avatar and use it for a long time. You don't want to sell it.''}
\end{quote}

%\textbf{Characteristics of NFT.}
%Typical features of NFT include uniqueness, provable scarcity, inter-operability, and indivisibility. The participants were able to identify some of the features.

%\textit{Irreversibility} of NFT ownership was mentioned by some participants. For instance,  P2 said, 
%\begin{quote}
%    \textit{``It's stored on the blockchain, which is secure. You can't copy or remove it. You can only add, no taking away.''} 
%\end{quote}
%Irreversibility of NFT was supported by the underlying blockchain, which prevented third parties from maliciously tampering ownership of digital collectibles. P11 also mentioned the irreversible and transparent feature of NFT, which made it hard to copy original, valuable items, such as a postcard from a famous person. 

% NFT is also free of physical damage, according to him:
% \begin{quote}
%     \textit{``If I receive a physical postcard, I have to make an effort to protect it from water or fire. There's some risk in storage.''}
% \end{quote}

From an artist's perspective, P1 did not like NFT which were simple copies of successful ones, without presenting special traits and creativity:
\begin{quote}
    \textit{``There're literally thousands of copy cats that are trying to replicate what CryptoKitties have accomplished. And the unfortunate thing is, it's actually working, like people are buying the copy cats. I'm not shaming them. I'm just saying when it comes to art, you have to be creative. Just copying someone else's work can harm creativity, even if you're making money out of it.''}
\end{quote}

\noindent \textbf{NFT Means Ownership.}
In conventional art markets, the process of verifying copyright for intangible goods was cumbersome. Often times, there was not a way to validate the authenticity \cite{van2002art}. P1 illustrated a scenario where it was difficult to verify the authenticity and ownership of art:
\begin{quote}
    \textit{Before NFT was a thing, I would post the painting on Instagram, and then offer it for sale. Everyone, 99.9\% of people would just say, why should I buy it? I can just copy the image and download it to myself. There's no real way to prove that you created it or that you've bought it. 
    % And NFT was just a perfect solution for that, verifying authenticity. Awesome!
    ''}
\end{quote} 

On the contrary, NFT is a cryptographic ownership of a unique item which is encoded into the underlying blockchain \cite{wang2021non}. Each NFT can be traced back to its owner. p1, P3 and P14 talked about the ownership aspect of NFT. For instance, P1 considered NFT as a way to verify ownership of digital files:  %, which was difficult to do otherwise in the physical world:
\begin{quote}
    \textit{``So basically, an NFT is buying the coin of someone, and that coin has its value because a digital file is attached to it, whether that be a video, a song, a painting, or just a picture. It's very much just a way to verify ownership of digital files, which previously was very difficult to do.''}
\end{quote}


%\yang{does anyone comment on they caring more about ownership than using the files?}
%\tanusree{not explicitly, frequently mentioned about ownership. 7 participants mentioned about the ownership}
%P2 explained NFT as something unchangeable and secure on the blockchain:
%\begin{quote}
%   \textit{``It’s hard to explain. Like, it’s stored on the blockchain, which is secure. You can't copy or remove it. You can only add, no taking away.''}
%\end{quote}

%\yang{this seems to be more about crypto in general than NFT}
%However, P11 found it hard to explain the NFT concept to a lay person, since he seldom did this before, due to negative stereotypes against NFT in Taiwan:
%\begin{quote}
 %   \textit{``Cryptocurrency is kind of a negative thing especially in Asia, or Taiwan. It's often related to scams. The concept of decentralization is hard to understand for most people.''}
%\end{quote}

% Some participants were knowledgeable about blockchain. P10 knew well the concept of ERC-721 standard on which NFT was built. 

\noindent \textbf{NFT Empowers Users}. 
As a business person owning an NFT company, P3 highlighted convenience of the business model of NFT. He thought NFT allowed freelancers to automate their workflow, with all transactions recorded by the blockchain and easily exportable, which made people's work more convenient and efficient: 
\begin{quote}
    \textit{`` It empowers individuals to create their own business model and smart contracts. Your business transactions would all be recorded, so you could export that data. So from a business model perspective, I think it's something that will benefit freelancers, and allow people to automate their workflow more easily. You don't have to worry about tracking receipts and things like that anymore, because it's all stored on the blockchain. 
    % So everything that you see in this environment exists on the chain.
    ''}
\end{quote}

% \textit{Decentralization} was also an advantage of NFT. P5 mentioned the decentralization feature of Decentraland, an NFT game allowing users to own and trade virtual land, which was supported by the underlying Ethereum blockchain:
% \begin{quote}
%     \textit{``The coolest part is, this whole game is built on top of Ethereum. So you know Ethereum obviously is this decentralized blockchain.''}
% \end{quote}

In the traditional art market, artists often relied on event organizer and sponsors to exhibit their work. The decentralization feature of NFT given by the underlying blockchain freed the NFT marketplace from those gatekeepers. Such an autonomous platform empowered artists, who could exhibit, sell and promote their work freely now, according to P13:
\begin{quote}
    \textit{``One of the benefits (of the NFT marketplace) is there are no gatekeepers like in the traditional art market. In the NFT world, you're a self promoter. You just need to come on the platform and do your promotion and sell it without the gatekeepers. So that I guess is one of the biggest benefits.''}
\end{quote}
%\yang{what exactly did P13 mean by gatekeepers? art market organizers or government regulators? so is it lack of regulation or lack of gatekeeping?} \tanusree{yes,he meant govt. and organiizer}
% By stating that the participant indicated that this market doesn't have regulatory barrier for them to restrict promoting or selling their work. 
% They have their own account to reach audience which doesn't need any organizer/ sponsors.
% \textit{Being friendly and supportive to unknown artists or freelancers}. 
Similarly, P9 thought NFT provided low barriers to entry for artists to present their digital work, with the help of painting tools and software.
% \begin{quote}
%     \textit{``It's not hard to create digital paintings. We have a lot of painting tools and software.''}
% \end{quote}
Even unknown artists could grow their career in the NFT marketplace. P11 liked to collect NFT created by unknown artists, and would recommend his friends who were artists to create NFT: 
% \yang{this example is more about empowering artists}\zhixuan{placed in the right place}
\begin{quote}
    \textit{``Some artists are unknown, and it's hard for them to make money. But their art may sell well if a market is built to support their career. I know some artists in Taiwan who are of some renown but not that famous. They make extra money by creating NFT of their artwork. So if I have friends who are painters, I would recommend them to create NFT on the platforms.''}
\end{quote}

\noindent \textbf{NFT is a Place for Collaboration.} P3 expressed the optimism and will to collaborate in the NFT community: 
% \yang{this quote is pretty general. add another more specific quote that talks about a specific collaboration or how they collaborate.}\zhixuan{added another one}
\begin{quote}
\textit{``A lot of new inspiration and new work is coming out and people are very willing to collaborate. In network, across countries across the world. So I think the overall perception I've received is, people are very excited and very optimistic and they are wanting to do more and more with this space and develop it.''}
\end{quote}

On a practical level, P6 told us how the artist community collaboratively tried to propose new forms of NFT art:
\begin{quote}
    \textit{``We're really collaborative. And we're always trying to make valuable pieces of art, you know, not trying to make products just for sale. We're always thinking about proposing something new in the art market.''}
\end{quote}
As the founder of an NFT platform, P10 would attend online meetings organized by other platform founders and developers, and discuss product functions, as well as how to create a better NFT ecosystem for artists.

\noindent \textbf{NFT Represents Digital Identity}. P7 thought NFT could be used as personal identities when making friends online, especially in the Metaverse, which was a virtual shared space:
%\yang{cite Metaverse}
\begin{quote}
    \textit{''I believe in the future, people will spend more time on the Internet, in the virtual world, in the Metaverse. And in that world, people don't meet each other physically. People use their digital identities to make friends with each other.''}
\end{quote}
% \yang{elaborate the identity representation and communicative utility of NFT.}

Bored ape was a popular NFT project recently. P7 told us that members of a Chinese-speaking NFT-related Clubhouse room used bored apes as their Avatars, which showed their membership. 
% They joined another English-speaking bored ape room, and later, the two rooms joined together, and planned ``ape attacks'' by entering other non-crypto rooms. They believed by doing so, they could ``let non-crypto people get to know about NFT.'' 
% P11 also observed that several influencers and artists in Taiwan bought bored apes, and exhibited them on Twitter and Facebook to promote them. 
P11 thought one day, a bored ape may be used as the digital identity to attend parties held by the community.  
% P3 also indicated the same about this growing community with diverse people. He added that how he made friends within this short period and gained a large network. He felt that this community provided him the ability to reach out many people.

\subsubsection{Criteria for Good NFT}
Our participants shared their different criteria for good NFT when buying/collecting NFT.
% \textbf{Users' Standard/Criteria for Good NFT.} 
%During our interview, we received different level of judgement about the quality of good/poor NFT. 
%They shared their views in the context of collecting NFTs, seeing people to buy NFTs within community, their individual preference in specific types of NFT. There are 2 types of responses on good NFT artwork. 
% Originality and creativity were the two main criteria. %factors to consider NFT as good quality regardless the media such as, 2D, 3D, AI tools usage, traditional art media. 
%Some participants mentioned about utility of NFT and future prospect/popularity of an NFT artist as their decision mechanisms for buying NFT. 
%
%\yang{this section seems to be more about how people make NFT purchase decisions} \tanusree{Not all the quotes.they mentioned those characteristics in different context- mentioned above} The participants had their personalized standards for good NFT. 
% For example, P1 explained his criteria for assessing NFT art: 
% \begin{quote}
%     \textit{``So I'd say the three main criteria when I look at the arts are originality, creativity and peacefulness. Sometimes a piece of art can be extremely abstract. But if it's done in a tasteful way, then it could possibly look nice. It could have meaning even though it doesn't contain that much imagery.''}
% \end{quote}
%\yang{this is more about art than NFT. not the best quote} \tanusree{its the answer for NFT/crypto art. question was about crypto art}
% \yang{elaborate on peacefulness}

\vspace{3pt}
\noindent \textbf{Aesthetic Consideration.}
When our participants talked about their collections, nearly all of them expressed how beautiful the NFTs were. For example, beauty was seen as a direct attractiveness for P1:
\begin{quote}
    \textit{``It just looks nice. I mean sometimes art has meaning behind it. Sometimes it doesn't. Sometimes, even if the art does not have meaning, but you personally just think it looks nice, then, by all means, it just looks nice.''}
\end{quote}

\noindent \textbf{Inferring Value by Heuristics.}
When assessing the value/quality of a certain NFT, people may fall back to simple heuristics, since NFT is a new field, and there is a lack of established assessment measures. 

For example, P3 estimated the future value of a certain NFT based on its creator's reputation and popularity. He believed NFT created by established artists would be worth more in the future: %\yang{this is more about why he purchased NFT} \tanusree{purchase decision based on artist's prospect/popularity}
\begin{quote}
    \textit{``It was a piece of music that I bought, and it was created by a well known musician group. My thinking is that, they're already an established group. They have a large following. So there's a demand for this item.
    % (I prefer a certain NFT) If I personally believe that the artist has a lot of potential. And I see he's very engaged in this space. I will keep it for 10 years if that person is still making work, no matter whether the value of his work will go up.
    ''}
\end{quote}

The amount of time and effort devoted to making an NFT was yet another criterion: the more effort, the more value. 
%standard \yang{this again seems to be more about what criteria people use to make purchase decision} \tanusree{in majority cases, when participants mentioned about the good/bad quality of NFT, the context was purchasing}, 
P5 explained: 
% \yang{you need to explain the quote not just present the quote}
\begin{quote}
    \textit{``3D animation basically is kind of the most popular form of content. People see value in it, probably because it takes a lot of time and effort to model something. So I think people tend to (want to buy it) when they see something that has taken a lot of time, regardless of whether it's good or not. 
    % They tend to want to buy it if that makes sense.
    ''} 
\end{quote}

\noindent \textbf{Practical Utility or Not?}
% \yang{Having actual utility (e.g., NFT as tickets) was considered another criterion, find anther quote}. 
P12 noticed a heated debate about whether NFT should have utility or practical value behind it. He liked the idea of having utility behind NFT, which gave NFT more possibilities:
\begin{quote}
    \textit{``If NFT need to have utility behind it? Or can it just be digital art? Some are saying that you know an NFT is worth more if it has better utility behind it. I know there's NFT like, if you buy it, you're going to be able to get into a conference with it.
    % and you can't buy physical tickets. You have to be an owner of the NFT to be able to enter the conference. And that NFT itself is a collectible, is an art piece. 
    So there's a lot of debate happening there. I personally like the idea of having utility behind NFT, cause there's a lot of exploration you can do there that hasn't been done yet.''}
\end{quote}

\subsubsection{Challenges Facing NFT}
%Since NFT was a relatively new phenomenon, there was a lack of support and open information for newbies, especially those who were non-English speakers, and who were ``in fear of losing a lot of money and a lot of time for NFT,'' as P15 commented. P7 thought the high price fluctuation, low liquidity of NFT (i.e., difficulty of reselling NFT), and low success rate of new NFT projects made the NFT market more risky than stock markets. %P10 also mentioned the high price fluctuation of NFT, and pointed out the difficulty of reselling NFT as a major challenge facing buyers and collectors.
% since ``many NFT lost their selling value immediately after they were bought.''

According to the participants, there were many challenges facing NFT, i.e., (1) technical issues, (2) security risks, (3) lack of effective regulation, and (4) challenges introduced by the underlying blockchain technologies. %of newly emerging NFT platforms and projects, which were still on their early stage. The second barrier was lack of regulation from NFT platforms and communities, which led to the prevalence of scams and low-quality NFT. The third barrier was inherited from the underlying Ethereum blockchain, including environmental impact, irreversibility of on-chain transactions, and high gas fee.
%\yang{this section can be significantly shortened.} \tanusree{updated}

\noindent \textbf{Technical Issues}. 
Since NFT has existed only for a short time, many NFT platforms and projects were new, even in their infant stage. Thus there were constantly bugs and technical issues. Some people thought it understandable for the platforms to have bugs, given that NFT was a new realm. For example, P5 did not feel demotivated by platform bugs which were caused by the huge traffic:
\begin{quote}
    \textit{``I think the platforms are fine. They're kind of buggy, but that's only because they've experienced a huge amount of traffic and users coming onto their platform in the last two months, right? So they've had to scale their platforms considerably up. I don't think I've ever felt demotivated.''}
\end{quote}

However, P3 was concerned about trustworthiness of new NFT projects, which were lacking in consistency and stability: 
% \yang{move this to the 2nd quote, so naturally leads to the security risk.}
\begin{quote}
    \textit{``I think a lot of the platforms are still very new, and so there's constantly changes happening, and there's a lot of bugs, and some sites get crashed and go down. Then along with that, there's a lot of new projects that pop up, and it's hard to gauge how trustworthy a new project is, and whether to actually invest in it or not. So in that way, I'm a little bit concerned.
    % with how new it is, because I think it's still in a baby stage, and I think it's still developing a lot, so it's just something to deal with.
    ''}
\end{quote}

% P3 pointed out the lack of full control and features in different NFT marketplaces. As a result, he had to shift between different platforms. He thus called for a comprehensive platform with smart contracts which could support more functions:
% \begin{quote}
%     \textit{``I think I have yet to see a marketplace that is 100\% control, like able to be controlled by the user, like you can adjust every single parameter. There's no platform with all features [...] so you have to split between different platforms. I would love to see one NFT space with unlimited capabilities, so you can use it very simply and straightforward.''}
% \end{quote} 

\noindent \textbf{Security Risks (Scams).} Malicious users frequently posted scam NFT, which were not NFT at all, or copies of famous and expensive NFT, in Discord channels and on Twitter, asking for more money than their real value. P7 described how a scam NFT was made, the process of which was simply copying existing images, adding new traits, and minting it:
\begin{quote}
\textit{``People can copy an image, photoshop it to add some new traits, and mint it on Opensea. He can scam people that this is the original one, but actually it's altered by some random people.''}
\end{quote} 

Scams could cost huge losses to buyers/collectors. P2 knew one person who fell for a scam NFT, which cost him 11 ETH (worth of tens of thousands of dollars).'' Due to the prevalence of scams, it was a hot topic on many online forums, as P3 noticed:
\begin{quote}
    \textit{``Recently someone was going around scamming a lot of people and taking their money, within not even one day, I would say, like 30 minutes. Almost everyone in the community was talking about it right away and was saying, `be careful of this person. They're stealing money.'''}
\end{quote}
Fortunately, reminders from other community members often time helped prevent people from falling for scams, as in the case of P4.
% \begin{quote}
%     \textit{``I was lucky until now, because I got the information about the different scamming ways. That's a good thing with the Discord server to connect with other artists, because I got to know there are some people who lost money.''}
% \end{quote} 

P7 and P11 mentioned a special type of scam on Opensea, which arose from design issues of the platform: since the icons for different cryptocurrency were not distinguishable from each other in the bid process, some malicious buyers claimed to bid in Ethereum (worth of thousands of USDC), but eventually paid in USDC, which led to a huge loss to sellers. They thought such scams could be avoided, as long as users paid more attention, and platforms provided some forms of alert to users.

\vspace{3pt}
\review{\textbf{need to present/ reflect the significance of this finding}-- result Similarly - varied views between participants is rarely expressed or teased out. For example, there is a clear tension between the desire for open access to NFT markets, the desire for high-quality works, and some form of regulation. But this is not reflected in the findings particularly.}

\noindent \textbf{Lack of Effective Regulations (Low-Quality NFT).} P4 thought the high gas fee on Ethereum more or less regulated the market, since ``not everybody was able to mint.'' From P2's perspective, despite the regulatory effect of the high gas fee, it also put a heavy burden on NFT artists: 
\begin{quote}
    \textit{``If the gas fee keeps this high, it may stop some trash (low-quality NFT) from being posted. But it's really expensive for creators.''}
\end{quote}

There have also been regulatory efforts by NFT trading platforms. However, such regulations were not consistent across different platforms.

For example, P2 noticed that Rarible encouraged new users to verify their Twitter accounts in the onboarding process. This was not mandatory, however, those who did so would enjoy more visibility on the platform, which meant more people could see their posted NFT. The platform also helped deal with copyright violations, as mentioned by him:
\begin{quote}
    \textit{``(If the copyright is violated) I will either message staff members about this, and they may take down the work after investigation. Or I would tweet it, so that more people get to know.''} 
% From the response, it seems that solving copyright violation issues are ad-hoc where users post any incident on external social media account to convey the news to community to give alert.
\end{quote}
P6 also told us that an artist was banned for selling copies on Rarible, showing effectiveness of Rarible's manual regulatory efforts.
% \begin{quote}
%     \textit{``The other day, I saw that a renowned Japanese artist was selling copies, and then a few days later, the artist was banned.''}
% \end{quote}

Foundation was an invite-only NFT trading platform, which ensured the quality of NFT to some extent. P11 felt more confident about the quality of NFT on Foundation compared to other platforms:
\begin{quote}
    \textit{``It was pretty like Clubhouse. If you want to join, you've got to have someone invite you. So not everyone could be an creator. When the platform just started, there were only several known artists. Only those invited by them could join, and could further invite 2 or 3 other artist, like a snowball. So I feel assured about the quality of NFT on Foundation.''}
\end{quote}

Other NFT trading platforms also practiced their unique regulatory measures. Opensea moderators would put a blue mark on authenticated NFT, in order to avoid copies of famous projects. P8 noted that Theta moderators would check each transaction, including the buyer and the seller, to mitigate the process of any act of scams. However, he mentioned that if the buyer and seller knew each other and decided to make private transactions outside of the platform, their transactions would not be protected. 
% P9 noticed Xianyu, a Chinese platform for trading secondhand goods, removed some NFT of sky-high price posted by users.
The NFT platform developed by P10's team would automatically filter out NFT irrelevant to VR, using off-the-shelf AI technologies developed by Baidu and Google. However, they did not pay attention to other quality issues for budget considerations. 

Despite all the regulatory efforts mentioned above, such as optional social media verification (Rarible), invite-only mechanism (Foundation), authentication (Opensea), manual check of transactions (Theta), and AI-powered filtering of NFT themes (P10), there was not a single platform which practiced all these measures. As a result, aforementioned scams and low-quality NFT was prevalent in the NFT marketplace.  

% On that end, P3 regarded lack of regulation and changing policies of platforms as unacceptable features, which made them weak in accountability, and called for more strict regulation:
% \begin{quote}
%     \textit{``I think for the most part, the regulation on the majority of marketplaces is very unknown, like there's not a lot of information, especially for the smaller and the newer sites. There's very little documentation [...] They're always changing their policies. For example, initially any user was able to verify their account on Opensea. And then at some point, I think the platform decided to change the policy and take away people's verification [...] I think it's discouraging to know that the platforms themselves have very little effort holding them accountable.''
%     % .. Then the competitiveness of this space. So if a marketplace has bad regulations and not great features, people just leave, they'll go to another marketplace.
% }
% \end{quote}

Low-quality NFT could be partly attributed to the lower barriers to entry of the NFT marketplace compared to traditional art markets, as P1 said,
\begin{quote}
    \textit{``They just spam their link. They're extremely desperate for people to see that piece of work, and most of those people, actually, their art isn't actually that great. It's like something that you'd make within 20 minutes on Photoshop. Unfortunately, that's because the gates are open, and the price barrier is relatively low.
    % It's still high, let's say you want to mint like \$150, that's \$150. You have to be upfront without knowing whether NFT is going to be sold or not. But it's a lot, a lot, a lot less than, let's say, if we go to an art gallery or a museum and you want to sell there. But I think as soon as the NFT bubble bursts, it will get a lot better, because money isn't going to be as much of an incentive as it is right now.
    ''}
\end{quote}
As a creator, P13 was demotivated and upset by the fact that artists who created lower-quality NFT than him sold better:
\begin{quote}
    \textit{``So most of the best-selling artists are not really good photographers. And I sold, since last month, nothing. That's a little bit demotivated if I see other guys are selling, even if they are worse than me.''}
\end{quote}
P5 was also demotivated by seeing people sell low-quality work, since he put a lot of work into his own NFT. 
% He avoided such demotivation by seeing his NFT career as a marathon instead of a sprint.
% \begin{quote}
%     \textit{``I mean sometimes seeing other people sell NFTS that aren't that good can be kind of demotivating, because you, you know, put a lot of work into it. But I see this happen all the time. You do see on Twitter a lot of people get demotivated, but I think it's a marathon. It's not a sprint. So my vision for my NFT company is like four or five years down the road. It's not about cashing in today or tomorrow or next week, you know. That's how I avoid demotivation. I just kind of try to stay steady and work every day.  I have a schedule. I post 20 videos every week of my decentralized content.''}
% \end{quote}
P15 expressed a similar opinion:
\begin{quote}
    \textit{``I don't understand artists who release low-quality NFT. It's not good for other artists, because some artists spend a lot of time to create some artwork and can't sell it. But some people can create low-quality NFT and sell it for big money. It's not cool for me.''}
\end{quote}

% While the NFT marketplace was saturated with low-quality and scam NFT, and money laundering, participants tend to prefer less regulation with a benefit of decentralization.  P1 stated-
% \begin{quote}
%     \textit{``I personally think that decentralized projects should remain that way. Just like the dark web. Good is going to exist and also bad. [...] for example, your government (China) banned the internet, but you're still using it. So if governments around the world are banning such projects, it would decrease the amount of people engaging into it.''}
% \end{quote}
% From his opinion, increased regulation and barriers to entry of NFT platforms would be a hurdle to artists' growth. P11 mentioned similar aspects and indicated that self awareness of users was more important to avoid scam and poor NFTs. 
% \begin{quote}
%     \textit{``I see increased regulation and barriers to entry, and it decreases the chances of upcoming artists to share and make a living off the arts they're making. So for example, if the barriers to entry were a lot higher on Rarible, I wouldn't be able to share my art because I don't have that much of a social media presence yet. 
%     ''}
% \end{quote}
% P11 also felt fine with the current level of regulation, and thought self awareness of users was more important than regulatory efforts of platforms:  
% \begin{quote}
%     \textit{``I think users, rather than project owners or platforms, should take the responsibility. They should do their research, and learn how to avoid scams.  Regulation can hurt the free space of art creation. 
%     % I've indeed bought NFT without blue marks which were created by unknown artists. They were not checked by the platform, but still good
%     ''}
% \end{quote}

\noindent \textbf{Blockchain-Induced Challenges.}
Since NFT was built on top of blockchain especially Ethereum, several drawbacks/challenges of it were related to the nature of the blockchain technology.
% P3 thought of extensive energy consumption and negative environment impact as frustrations induced by the Ethereum blockchain:
% \begin{quote}
%     \textit{``I do have concerns with the environmental impact of the Ethereum blockchain. The first thing they say (about Ethereum) is that, `oh, it's bad for the environment.' That was one frustration. I wish there was a better understanding of how exactly it impacts the environment, and whether there're alternatives that don't have the same energy usage as Ethereum.''}
% \end{quote}
% P6 also mentioned the negative effect of Ethereum blockchain on global warming. He tried to improve the quality of his NFT, to make up for his addition to global warming:
% \begin{quote}
%     \textit{``Instead of focusing on my profit, I'm more on the quality of my work. 
%     % Because I believe that in the long term, that's gonna make some profit. I tried to balance that, you know. 
%     If I'm gonna contribute to global warming, then I'm gonna try to make something that's not so harmful.''}
% \end{quote}

Though irreversibility of blockchain/NFT prevented malicious users from tampering the data and controlling the market, this feature could also lead to some convenience for artists. For instance, P1 noted that if mistakes were made during minting an NFT, there was no way to restore it:
\begin{quote}
    \textit{``Let's say, you're preparing for an NFT, and you mint it out. And then two hours later, you realize you've made a typo, or you've uploaded the wrong file, or the cover isn't the exact cover you wanted.
    % That's the blessing and the curse when it comes to decentralized tokens. 
    It's set in a stone, so you can't edit it. You can't change it. Let's say you accidentally burned an NFT, then there's no way could it be restored. It's gone forever. So it's both a blessing and a curse.''}
\end{quote}

Another major challenge for NFT creators and traders was the high gas fee on Ethereum, which made minting and transacting expensive. For example, P2 sold his NFT for \$1800 CAD, but only earned \$700 CAD after paying the gas fee. P4 regarded the high gas fee as a major issue of Ethereum:
\begin{quote}
    \textit{``I think the gas price is the most important thing for artists, because it's a lot. OpenSea, for example, you can mint for free there, but you still have to pay gas prices. I think the gas prices are the main issue of Ethereum.''}
\end{quote}
According to her, artists had to sell NFT for a higher price, in order to compensate for the fee during minting and transacting.
% :
% \begin{quote}
%     \textit{``And the gas is really high, so yeah, you have to sell it for a higher bit. It makes sense for you that you don't pay for selling the NFT. And that's a little bit complicated. Yeah, gas price is too much nowadays and it's like increasing everyday now.''}
% \end{quote}
% \begin{comment}
%  He thought the high gas fee may scare some new artists and traders away:
% \begin{quote}
%     \textit{``Now I can't say everything is amazing, because I'm not like the other artists who're not speaking the truth. No one likes to speak about gas prices and how much people are really making. In total I've sold around \$1800 CAD but only got \$700 CAD because of gas prices. Pretty insane number that most people don't talk about, because it scares people away. Not saying that everything is bad, because jeez I'm saving for college, and \$700 bucks is \$700 bucks.''}
% \end{quote}
The high gas fee on Ethereum affected P3's opinion for NFT. He did not like the facts that some people did not have enough money to participate, and that artists were not gaining proper monetary return: 
\begin{quote}
    \textit{``I think the price right now on the Ethereum blockchain is very high. It turns me away from NFT a little bit, because it looks kind of exclusionary. Some people who don't have money can't participate, so I don't like that... I think one thing that initially discouraged me was creating a lot of work and putting them up for sell, and then not having any actual monetary return.''}
\end{quote}
% The gas fee varied in different places and times. It could be extremely high in peak hours and in countries where NFT was popular. For P1 who lived in UAE, gas fee was less of an issue:
% \begin{quote}
%     \textit{``It depends on the time we're looking at. So fortunately, for me, I live in the opposite side of the world where NFT are most popular. So when I mint out my NFT, most of the Western world are asleep. So the gas fees are extremely low compared to the peak hours when gas fees are almost \$180. I average around \$70 in gas fees.''}
% \end{quote}

% \end{comment}

\subsection{Motivations for Participating in the NFT Marketplace (RQ2)}

% \yang{i don't think you need to differentiate individual vs. community-level motivations. it's often blurred.}

% \yang{the main motivations seem to be: monetary gain (nft/art creation, nft trading/speculation), be part of a movement, express oneself}

People had very different motivations for participating in the NFT marketplace, as observed by our participants. For example, P2 noticed that some people owned NFT just for profit, while others owned NFT for real value of it.
% \begin{quote}
%     \textit{``Some of them are not trying to sell. They just hold, not for profit. But some people just own a ton of NFT for profit. I mean, it’s a 50 to 50 case.''}
% \end{quote}

Simple motivations could be pleasure and a sense of accomplishment for creators, as in the case of P3,
\begin{quote}
    \textit{``And another concrete benefit I would say is, it's just fun. It's a lot of fun! There's a sense of accomplishment. When you saw something (you create), there's a sense of accomplishment.''}
\end{quote}

Here we report on different motivations of our participants as well as their observed motivations among community members, such as monetary gain for both creators and traders, expressing oneself via creating NFT, being a part of the innovative movement, and staying in the supportive community.

% Motivations for participating in NFT creation, collection, and trading includes, make a living during the pandemic, being a part of the art revolution, staying in the supportive community, building own business model, combining NFT with personal interest, expecting monetary return. \zhixuan{re-write} 

% Other motivations in our interview participants included virtualizing offline art business during pandemic, enjoying community support from other NFT artists, combining one's personal interests, making people happy with NFT art, monetary return, and chasing the frontier of blockchain technology.
\subsubsection{Monetary Gain}

Given the high monetary return of NFT selling, many people were devoted to NFT creation and trading nowadays, as reported by our participants. 

\noindent \textbf{Creating NFT for a Living.}
Our participants who were NFT creators/artists would sell their NFT after creating/minting them. For example, P2 was a high school student, and saved for college by creating and selling NFT:
\begin{quote}
    \textit{``I would say I'm a 12th year high school student, and I need to save for college. If I earn 1 ETH from my NFT sell, and one day the price (of ETH) blows up and gets me a crazy sell, that would be really great.''}
\end{quote}

Some traditional artists tried to keep their business up in the NFT marketplace during the pandemic, when offline business was made impossible. For example, P13 was the inventor of hyper-real landscape photography, and used to earn money through workshops, tutorials and speeches. The pandemic hurdled his offline work, and he turned to the NFT market for a living:
\begin{quote}
    \textit{``(The events were) Almost not possible during the pandemic. So I lost almost 80\% of my income because of that. And then I guess two or three months ago, two guys reached out to me, and asked me if I knew anything about NFT. Then they built a team with me. Now I try to sell as much NFT as possible in my spare time to earn enough money to pay my bills.''}
\end{quote}
Similarly, P4, who was a tattoo artist, also started her NFT career out of the purpose of keeping her business up in a virtual/online manner during the pandemic, when Berlin was locked down: 
\begin{quote}
    \textit{``I started trading in the NFT marketplace during the pandemic. Lockdown was just the reason for that, and I had time at that moment too. I came to research about it.''}
\end{quote}

\noindent \textbf{Trading NFT for Speculation.} P3 would buy NFT with the specific intention of re-selling them for a higher price:
\begin{quote}
    \textit{``I bought one piece (of NFT), specifically with the intention of reselling it. So I saw that it was pretty undervalued, or I knew that it was going to go up in price. So I bought it, and I'm currently holding it up, basically with the intention of selling it eventually.''}
\end{quote} 

Fear of Missing Out (FOMO) was a common emotion among  cryptocurrency traders, per our observation in online groups. When the price of a cryptocurrency went up, or when a new cryptocurrency was listed, they would purchase it out of the fear that the price would go up sharply one day. If she did not buy it, she would miss the huge opportunity while other people grabbed it. It was also a major motivation for P11 when he bought NFT:
\begin{quote}
    \textit{``I was controlled by the FOMO emotion. I told myself not to buy more NFT, but when I saw many people talking about it in Discord, I started buying again. I thought the price would go up.''} 
\end{quote}
% He was further encouraged to collect and invest in NFT after he knew two famous blockchain investors were also collecting NFT. 
However, the price of several NFT he bought due to the FOMO emotion dropped by a large percent. 

Some traders merely cared about financial returns, without considering the real value of NFT. P1 expressed his disapproval of this phenomenon: 
\begin{quote}
    \textit{``Some people are just arrogant. They're rich, and they just like to waste their money. So they buy whatever is popular. Some people convinced themselves that something would gain value, even though it's not that great of an investment.''}
\end{quote}
% P7 also observed that most members in an NFT-centered Clubhouse room cared more about speculation than the real value of NFT:
% \begin{quote}
%     \textit{``And I think most of them in our room, just like me, are quite new to the market. And most of them want to make some profits, which means even if they buy an ape NFT they like, when the price goes down, they will be frustrated. And some of them will panic sell. Because the NFT tokens are not a small amount of money. They're spending like tens of thousands of RMB for an image, and if they cannot sell the image later, they're losing a lot of money. So, for them, they have some expectation to sell them in the future for a higher price. So, I think most of them were up there for speculation.''}
% \end{quote}
% P15 did not like it when people created and bought NFT only for money:
% \begin{quote}
%     \textit{``People think differently about NFT. Some of them think it's a good marketplace to get money. Some of them think that it's a good place where you can get inspiration. And some of them want to share their artworks with people. I don't like people who think it's only for money. Because it's not for money. It's our industry. It's good to create good art in the industry right now.''}
% \end{quote}

\subsubsection{Freely Expressing Oneself}

Creating NFT was seen as a way to freely express themselves, according to P4 and P5. Artists could create/mint NFT out of their own will and ideas, without having to follow client requirements. 

In P4's previous business, she had to design for clients' ideas. Now she could freely create NFT out of her own ideas and interest:
\begin{quote}
    \textit{``This was a way to step out of my normal art comfort zone a little bit, start something new, learn something new, and create something new. In my business, my job, I created designs for my clients, for the ideas of them. And NFT are just my ideas, and that's pretty cool to make something new.''}
\end{quote}

For P5, NFT creation combined his multiple personal interests, such as writing, blogging, and video editing:
\begin{quote}
    \textit{``I've experienced a lot of different forms of content creation on the Internet. I've been a writer. I've been a Blogger. I've worked for the University of California, sort of doing academic stuffs. I've been a video editor. I'm an artist as well, so sort of all these different things. Interests of mine sort of came together for this (NFT) project and it's been going on really well, so I've been having a lot of fun with it. 
    % And in about 2 months we have almost 3,000 followers on Twitter, which is like a lot in my experience.
    ''}
\end{quote}
% Since he ran an NFT company, building a brand that people love was also an important motivation in his NFT creation and promotion:
% \begin{quote}
%     \textit{``I think the most important thing to me is sort of building a brand and building a company that people love, and creating content that people love. Like that's my motivator, like I entertain people you know. Like I've put out videos on Decentraland, the game I was talking about earlier, they had like tens of thousands of views, or hundreds of retweets, or whatever, because people like it.''}
% \end{quote}
% P2's motivation for creating NFTs is also ``trying to make everyone happy'', which was seen by him as a kind of professionalism for artists. 

Even people without a technical or art background could express themselves with NFT. P11 was planning to create NFT for his child ready to be born in December, which was seen as a way to keep memories for his son:
\review{In effect, the findings primarily recount a small number of experiences, and opinions of those working with NFTs - rather than analysing more deeply the values, implications, and logic of their participants. For example, Pg16 includes a remarkable quote from a participant about creating an NFT aligned with the birth of their son. There is so much more that could potentially drawn out here – that speaks to the role NFTs play in people's lives, the intersection of the 'market' with even the most personal events, the presumed permanence of NFTs etc. As it is, many quotes are left to speak for themselves, and some sections or sub-themes are extremely short.}

\begin{quote}
    \textit{``I was thinking of creating NFT because my child will be born in December. I'm thinking whether I can make some connections between the baby and the blockchain, and even create a trend on the market. I think I'm fine with Photoshop and simple art, as well as uploading it to the Ethereum blockchain. I want to do this because I want to keep some memories for him, like funny stories and his dreams.''}
\end{quote}

\subsubsection{Being Part of an Innovative Movement}
Some participants expressed their motivation of being a part of the progress and frontiers of blockchain innovation and NFT art revolution. 

P13 started his NFT career during pandemic to make a living, but he kept creating NFT even after pandemic. His current motivation to stay in the NFT marketplace was to be a part of the ongoing art revolution:
\begin{quote}
    \textit{``It's a new way to sell art. I guess it's the new art revolution... I'm better in online marketing than in the real world. I guess it's a cool new thing because you know, I have pretty much followers on Instagram and Facebook. On Instagram I have around 180,000, and on Facebook I have 110,000. So I know I'm better in online stuff, and it's excited to be part of this revolution. 
    % Now the whole feeling is like that because the photographer NFT space is really new, so I'm like part of our revolution. That's an exciting thing.
    ''}
\end{quote}
P5 also created and traded NFT due to his interest and passion in blockchain technologies:
\begin{quote}
    \textit{``It's like a new frontier right on the Internet, you know, we're sort of on that cutting edge of all the cool new stuff that's coming out. And a lot of that, you know, has to do with blockchain. So that's kind of my thoughts on this.''}
\end{quote}
P11 was another case. He thought collecting NFT ``made him feel that he was keeping up with the times.'' 

P3 noticed that many members in the NFT community were excited about the advancement and value of NFT, and wanted to do more to develop this space:
\begin{quote}
    \textit{``I think almost everyone that I've interacted with believes this (NFT) to be one of the most important technologies and advancements in our lifetime. I think a lot of people are calling it the new Renaissance for artists, and most people are very excited and very energized. A lot of new inspiration and new work is coming out, and people are very willing to collaborate in network, across countries, across the world. So I think the overall perception I've received is, people are very excited and very optimistic, and they're wanting to do more and more with this space and develop it.''}
\end{quote} 

\subsubsection{Staying in The Supportive Community.} P4's motivation for staying in the NFT marketplace after the pandemic was more about community ties, such as mutual support and understanding among the artist community:
\begin{quote}
    \textit{``The first thing I think is the community of artists. I didn't know that such a kind and supportive community would even exist (before I started my NFT career). I met a lot of nice people. Artists understand other artists, so it's pretty good to talk with them, or ask them for advice and opinions. I think being in this NFT community is the most important thing.''}
\end{quote}

Later, we will elaborate more on community aspects of NFT.

% \noindent \textbf{Building Own Business Models.}
% Another motivation for NFT users is owning a unique business model without central regulation. The decentralization of NFT supported by the underlying blockchain empowered individuals to create their own business models within smart contracts, as P3 said,
% \begin{quote}
%     \textit{``I think the first benefit for an NFT marketplace is that, it empowers individuals to create their own business model and smart contracts. So in theory, if you use the right, if you trust the platform you work with, you would have unlimited control.''}
% \end{quote}

% \subsubsection{Observed Motivations in the Community.}

% P9 enjoyed the atmosphere of NFT-game-related communities, since the members cared more about the long-term value of NFT instead of short-term speculation, and they only talked about NFT games rather than investment and prices. She thought many people bought game-related NFT out of curiosity and for collection purposes:
% \begin{quote}
%     \textit{``They don't know whether it will have value in the future. They're just curious. They just want to participate and own it. If it has value in the future, then they can have financial rewards. Even if it doesn't, they still have some fun. It's a game after all.''}
% \end{quote}

\subsection{Individual- and Community- Level NFT Practices (RQ3)}

% \yang{practices: how they discover NFT, create/mint  NFT, buy/sell NFT, use NFT, interact with others in the NFT community}

NFT has became popular only recently, and many of our participants (10/15) had less than 1 year of experience with NFT. Generally, they had positive experiences in and attitudes towards NFT, seeing it as a creative form of blockchain art. P1 compared the NFT innovation to the 1995 Internet revolution, in which Google and Amazon survived and proved to be successful companies, while many other companies went broke: 
\begin{quote}
    \textit{``I think NFT are in an extreme bubble right now. It's going to burst within this year. But I think every bubble has meaningful innovation. So just like the 1999 .com bubble, most of the companies failed. But we got Google and Amazon, and other huge corporations right now which rose from the ash of that 1999 bubble.''}
\end{quote}
Despite the huge bubble in the NFT marketplace, he thought good NFT projects would eventually survive. 

He we will report both individual- and community- level practices around NFT.

\subsubsection{How People Discover NFT}

Our participants got to know about NFT from a diverse range of information sources. P1 and P5 learned about NFT from online resources, such as YouTube videos explaining NFT concepts. P9 first knew NFT as a phenomenal thing with record-breaking bids. After he saw the wide application of NFT, he was motivated to learn more about it: 
\begin{quote}
    \textit{``NFT became hot and there were always record-breaking bids. It's a virtual thing, yet has such a high value, which is worth my attention. Then I noticed many applications of NFT in different areas, which motivated me to learn more about it in depth.''}
\end{quote}

% P1 mentioned about youtube from where he learned the basics and then started to research by his own. 
% \begin{quote}
%     \textit{``I learned NFT from the internet. One of the YouTubers I watched mentioned NFT back in December, but I didn't give it much thought. But then a couple of months later, the video explained what NFT was and laid out the basics. After watching that video, I continued doing my own research. And then I'd say a week ago, I started minting by myself."} 
% \end{quote}
% P5 also learned NFT from a YouTuber, who talked about NFT as well as Pokémon cards in a video,
% \begin{quote}
%     \textit{``The first time I learned about NFT was from a Youtuber, a pretty famous character on YouTube. He was talking about NFT [...] he was unboxing old Pokémon cards, like the original Pokémon cards from the 90s. And through that he was also talking about NFT.''}
% \end{quote}
% P14 learned about NFT from a Clubhouse room specific established to discuss NFT-related topics. P12 learned about NFT from a content provider he followed on multiple social media platforms and then did his own research to follow a similar path in the crypto world. 

% He was able to combine his entrepreneurial spirit with NFT during creation and promotion.
% \begin{quote}
%      \textit{``He has an entrepreneurial-like personality. He's also like a motivational speaker, but he runs a bunch of big businesses. And He produces like Internet content, I don't know, like 10 times a day for each platform from LinkedIn to Tiktok to YouTube, from Instagram to Twitter to podcasts. So I usually like a lot of his insights and a lot of his thoughts. I discovered NFT through him and I started doing my own research... Then I also happen to have a friend who I really trust and I like the way he thinks. He's very deep in the space despite the space is really still fairly new, but he's writing articles about various cryptos. He has a couple of mentors in the crypto world, so he started investing in crypto, and I'm preparing myself to follow a very similar path... And I see the NFT space. I see the ability to create. And I really want to go in as a creator with an entrepreneurial spirit and business mindset. I'm going to be mixing the two. That's really amazing.''}
% \end{quote}

Some participants learned about NFT from their friends and family members. For example, P4's brother introduced NFT to her as a way to sell tattoo art online during the pandemic, when her shop was closed under the lockdown policy: 
\begin{quote}
    \textit{``To be honest, I don't have much experience with cryptocurrency before I started with NFT. My brother invested in it for a longer time... Actually, I'm a tattoo artist based in Berlin. During lockdown and pandemic we had to close our shops... He told me about NFT as a new way to share, and maybe also sell the pictures... That was my entry in cryptocurrency, blockchain and NFT.''}
\end{quote}

P11 started his collection of NFT from claiming free airdrops of NBA-related NFT. He felt happy for getting free things. This initial experience also opened a door for him, and got him to start learning about NFT. Later, he became more interested in NFT when he noticed some NFT which ``did not exist in the real world at all'' sold millions of dollars. His belief in NFT was further enhanced after extensively reading articles about NFT:
\begin{quote}
    \textit{``I spend quite some time on cryptocurrency every day besides my work and study. Instead of focusing on the price, I pay more attention to some in-depth articles about cryptocurrency, which make me believe that NFT will have some real value in the future.''}
\end{quote}

\subsubsection{How People Initiate NFT Engagement}
When first engaging with NFT, there may be difficulty understanding the underlying concepts, especially for those who did not have a computer science background. When talking about his initial experience with NFT, P6 mentioned that the crypto world was changing fast, and there was a lot to learn about NFT and general cryptocurrency when he first stepped into this field:
\begin{quote}
    \textit{``When I started working with this community of artists, I didn't understand anything about NFT and the crypto world. It's moving really fast, so I've been studying a lot since last year. 
    % And when I first started to understand how the market works, I tried to propose something from my perspective, such as animation, and drawing, and maybe something from the conceptual part of my production. But it's always changing.
    ''}
\end{quote}
P12 thought NFT to be tech-heavy, and he could not understand many concepts related to blockchain:
% \begin{quote}
%     \textit{``In my opinion, like it's still pretty tech heavy, and like not a lot of people really understand it. I was struggling in that situation at times. They're almost speaking another language if you don't have the background.''}
% \end{quote} 
He further suggested making NFT less intimidating and more newbie-friendly, especially for age groups who were not familiar with the mode of virtual assets:
\begin{quote}
     \textit{``I think the number one thing that comes to my mind is making it less intimidating. 
    %  I think there's a perception that it's fairly intimidating. I heard this great analogy: I'm in my mid-40s, right? Sp the cell phone actually came pretty natural to me as they came out, but my parent, my mom still has an issue with her iPhone. So it's the same thing with digital technology, like 
     You're in university, and you must be in your early 20s. The idea of owning a digital good in a video game is a natural thing for you. But for my generation, and especially the generation above me, it's like a foreign language... 
    %  It's like, why do people do that? Am I OK with it?
     In five years, everything is gonna be drag and drop. NFT will be more in use than it is now. It'll just be a part of our lives, like the iPhone or smartphone. 
    %  I see the value in it, but I know there's lots of other people of my age, some of my business partners, are like, I don't get it. Why would you want to do that?
     ''}
\end{quote}

% P7 bought his first NFT 3 months after he first learned about NFT, due to the difficulty of buying NFT:
% \begin{quote}
%     \textit{``
%     % I think the time is like this February, when the Bitcoin is going up very fast and all the crypto world is attractive to many new people. That's when I get connected to DeFi and NFT. But 
%     NFT isn't easy to buy for new people. The process to buy some NFT is very hard for them. I heard about it, but I didn't find some direct ways to buy it. So I just ignored it. But later when I heard the word more and more often, I started to search it and learn. 
%     % So I first learned about the crypto punk, the most famous NFT project. That time, I have some idea to get my own NFT but you know crypto punk is very expensive and I cannot afford one. But in last month, when this project (bored ape) was released, I finally find an NFT project that I can afford and I liked. That's why I learned it in February but finally got my own NFT three months later.
%     ''}    
% \end{quote}

% Some participants seems to research the future prospect of NFT before jumping into it. P8 also learned NFT for some time and then dived into the marketplace as a trader:
% \begin{quote}
%     \textit{``A friend of mine told me about NFT. I didn't actually jump into it first. I, first tried to, you know, get to know more about crypto and try to see how it might grow. What's the future of NFT trading? So I get to read and see what's the demand of NFT currently. Well, based on my research, I begin to find more interest to work with it.''}
% \end{quote}

% P12 was a filmmaker in Hollywood, who thought himself to have entrepreneurial instincts, and ``was always the kid who sold baseball cards to his friends in the 90s.'' He was the one ``who drew out the map for Super Mario Brothers 2 before it even existed.''

When coming across difficulties in initial engagement with NFT, it was common for our participants to seek external support from platform representatives to solve them. When P3 first interacted with an NFT platform, he had difficulty setting up a wallet and depositing cryptocurrency into it. He asked the question on Twitter, and was directly replied to and helped by a platform representative. He successfully minted his first NFT in the end:
\begin{quote}
    \textit{``It was actually kind of difficult to set up a wallet on that blockchain, and to deposit the cryptocurrency. I asked around and tweeted. And then one of their representatives directly replied to me, and was able to help me. 
    % They sent me some free cryptocurrency, and after that, I just minted my first NFT. I selected an artwork that I had already created in the past, and I minted it on their platform. That was very straightforward.
    ''}
\end{quote}
P4 sought help from his brother instead.
% \begin{quote}
%     \textit{``The first experience was not easy to be honest, because of the wallet and account stuff, all the things. My brother helped me with that, and he did a lot of stuff with me. To be honest, if I didn't have him at my side, it would be a lot to learn and figure out, because it's really complicated when you don't have any skills before, and when you were not really into that cryptocurrency thing... Then I learned about that, and he showed me everything. Now I'm minting by myself.''}
% \end{quote}
% P15 came across multiple issues with different marketplaces such as Rarible and Foundation, including high fee and low visibility for unknown artists. Opensea, on the other hand, made an effort to promote his work:
% \begin{quote}
%     \textit{``I have a lot of problems with Rarible, because I never know a lot of about cryptocurrency and these marketplaces. First of all, for example, in Belarus, we have some problems to work with this platform. My big problem was the big fees to the platforms or to the Ethereum... After that I found the Foundation marketplace. I spent maybe two months to get this invite to Foundation. And I was so sad because in Rarible I spend, maybe \$50, for publication of my NFT. But on Foundation, I should spend maybe \$200 for publication. And for me as a younger artist, it's so much. And after that I am so sad because Foundation never get promotion for your artworks. You should do it only by yourself. If you are famous artists, like Lady Gaga, these platforms can support you. But if you are not famous, not popular artists, like me, for example, small artists, this platform is not interested in promoting you... But when I create my collection on Opensea, it starts promoting my artworks. It's really so great. It's so amazing. After Opensea supports me, a famous singer followed me on Instagram, like, `oh, I love your works.' It was so amazing for me. And I was so happy.''}
% \end{quote}

\subsubsection{How People Create NFT}
Different forms of NFT were being created by our participants.
% Some leaned towards traditional art, while some preferred to create AI-generated digital arts. 
Some participants preferred to mix traditional art with digital media. For example, P1 liked to combine NFT with traditional paintings, with the help of AI tools (he chose not to share the specific information which he thought was ``private''), and expressed his dislike of purely digital art. 
\begin{quote}
    \textit{`` I've always been a fan of fine art, high class art, you know, things that were made in the 1600s, 1700s, 1800s. I'm not a huge fan of the overly digital art that's very popular now with NFT, you know crypto themes. In my personal opinion, it looks a little bit childish. It doesn't feel tasteful.''}
\end{quote} 
Similarly, as a landscape photographer, P13 created NFT based on his own pictures, which were animated with digital effects. Similarly, P14 minted NFT on multiple NFT platforms out of his design works which he created before.

On the contrary, some participants preferred purely digital NFT. P4 created 3D digital duckies with different colors, textures and costumes using Blender, a 3D computer graphics software. 
% We also found NFT collectors, P3 who collected a diverse set of NFT genres, including 2D and 3D collage, computer- and code- generated work by generative artists. 
% As a musician, P15 was planning to release his album as an NFT, since crypto music was a new thing to him.
P10's team combined NFT with VR. Specifically, they created NFT of VR scenarios and elements: 
\begin{quote}
    \textit{``We created immersive VR scenarios, products and materials with interactive functions, like an office, a cinema, or a pub. I can directly participate in some pop bar activities in VR.They're especially useful during the pandemic when you stay home every day. It's different from just sitting in front of your computer, because it requires you to interact. It is really not just a visual nature, it is more based on the experience of the entire environment ad interaction''}
\end{quote}
He thought such NFT had more practical value in life than other popular ones such as NBA player cards which were merely for collection purposes. 
% He commented that the circulation of NBA Top Shots dropped by 80\% in May. 
% P3 created an interactive digital model of an abstract sculpture, which he created as a giveaway on his Twitter page for promotion purposes.
% P11 collected several types of such as a 3D NFT of a singer playing the guitar, which he thought could potentially be used to connect the virtual world with the real world, e.g., as an access to enter his concerts in the future. 

\subsubsection{How People Buy/Collect/Trade NFT}
P11 bought NFT of virtual land and other relevant elements in a decentralized sandbox game\footnote{A sandbox game is a video game which gives players a great degree of creativity to complete tasks towards a goal within the game.}, which made him a ``landlord'' and allowed him to rent land to other players:
\begin{quote}
    \textit{``I can create new things on my land like a manor owner. You can rent your land to others. I rent a piece of land to another player, and he uses the land to run his own business.''}
\end{quote}
He once researched on a horse racing game, in which one could buy his own NFT horse, or bet on the outcome of blockchain-supported races. He later decided not to play the game, because he thought it was too centralized: the rules could be easily changed by the developers.
% \begin{quote}
%     \textit{``I'm concerned that rules of the races and capabilities of the horses may be changed by the developers. This will make the game less fair. People who buy horses earlier will suffer a loss.''}
% \end{quote}

% \textbf{Privacy in Individual's NFT creation media}
% Unlike traditional art market where the media is clearly defined, such as, acrylic, oil, water color, sketch, wood, etc, NFT creators seemed very private in this regards. During our interview when P2 was asked about the media they used for NFT, he stated that.

% \begin{quote}
% \textit{``Within 26 hours of the initial mint, I sold my NFT for 0.777 ETH, It's called mountain elephant. This is actually an AI generated piece of art. But, I can't I can't share that information on tools and studio. It's private.''}
% \end{quote}

% P7 thought himself as a collector. He would sell his bored ape collections only if he could make a large profit out of them, but he would keep at least one ape that he favored. He thought NFT creation as artists' job, which he did not qualify for:
% \begin{quote}
%     \textit{``I think NFT creation is the artists' job. I don't know how to use Photoshop or something. So I'm not capable to create my own.''}
% \end{quote}

We found several holders (known as ``holders'' in the crypto community) in our participants.
P3 had not resold any of his NFT collections, just holding and appreciating them:
\begin{quote}
    \textit{``
    % I would say I identify myself in this space as an artist and as a creator, but I also have a collection. 
    I would say I'm more of a holder right now. I haven't really resold any of them, like putting them in the secondary market. So for me it's more about collecting work from friends and things that I like. I just hold and appreciate them.''}
\end{quote} 
Similarly, P11 had not sold any of his collections, even for the ones whose price had dropped by 95\%. 

% P4 said he was also a business person/marketer in addition to a creator:
% \begin{quote}
%     \textit{``I definitely see myself as a creator. I've collected a couple of NFTs, but I'm more of a creator. I mean, I'm an artist, but I don't really think like an artist. I think more like a business person or like a marketer.  And that's what I mean. One interesting thing is a lot of artists don't necessarily think that way.''}
% \end{quote}
% He was honest about his will to make money, and thought of his self-identification of a trader as an advantage compared to other artists:
% \begin{quote}
%     \textit{``So that's I think that's one advantage that I have. A lot of artists hear about the NFT thing and they want to capitalize on it, and they want to make some money. So you have a lot of people coming into the NFT space. They don't know much about crypto at all. The only thing they know is how to list their artwork on Opensea or Rarible or these different NFT platforms.''} 
% \end{quote}

% Although P6 identified himself as a creator and trading is not of his interest, he had to make a prolific career to attract collectors:
% \begin{quote}
%     \textit{``There is a lot of people who are entering this space for economical purpose... I don't think trading is really interesting for me. But I also believe that if you are not making a prolific career, then the collectors didn't notice you. It's like a real war. We have art galleries, and you like contacts start to grow on that direction.''}
% \end{quote}

% P8 regarded himself as an NFT trader, and decided to hold his NFT collections and sell them in the future when the price went up:
% \begin{quote}
%      \textit{``I've not sell any token, so because I actually want to, you know, see how it grew better in future. I'm actually trying to wait for a few more years from now to start selling.''}
% \end{quote}

\subsubsection{How People Build the NFT Infrastructure}

P9 was an NFT platform designer/developer. Through the platform she built, she collaborated with known artists, and created and sold high-quality NFT paintings:
\begin{quote}
    \textit{``
    % We're not building a UGC (user-generated content) platform. You can't ensure the quality and value of NFT if users are the ones who upload them. 
    Our platform takes the role of ensuring quality of NFT. We collaborate with known artists who have reputation and popularity. We mass produce, say 100 NFTs mimicking the style of their paintings with machine learning techniques. All the 100 NFTs have the gene of the original painter, but the production rate can be much higher.''}
\end{quote}
% However, compared to UGC platforms, such a business mode would potentially cost more human resources.

Similarly, P10 built an NFT platform to work with traditional artists who had no knowledge in NFT. They gained the right to use their paintings, and created and sold NFT.

% NFT has become popular only recently, thus all of our participants had less than 1 year of experience with NFT creation and trading. Generally, they had very positive attitudes toward NFT, and consider it as a creative form of blockchain art. P1 thought despite the huge bubble in the NFT marketplace, good projects would eventually survive:
% \begin{quote}
%     ``I think NFTs are in an extreme bubble right now. It’s going to burst within this year. But I think every bubble has meaningful innovation, something meaningful with common. So just like the 1999 .com bubble, most of
%     the companies failed. But we got Google and Amazon, and these huge corporations right now that were from the ash of that 1999 bubble.''
% \end{quote}

% All of the participants were both creators and collectors, actively creating and collecting various forms of NFT using different technologies: 2D and 3D paintings, AI-generated art, VR works, breathable NFTs, virtual augmented games, memes, etc. They also have different initial experiences in creating and collecting NFT. Some learned NFT from well-known figures on YouTube (P1, P5), some started NFT careers during pandemic (P4), some were enthusiast about blockchain and cryptocurrency for a long time (P3), and some got to know NFT from their friends and family (P4). When they ran into difficulties in creating their first NFT, they would seek for external supports from friends or platforms. We summarize some of the participants' interaction with different types of NFT, their self-identified role(s) in this marketplace, and initial experiences with NFT in Appendix~\ref{tab:overview}.

% \tanusree{created a table and summarize section 4.1 to the table. I am moving section{overview to appendix and summarized in a table}}. 

\subsubsection{An Open and Reciprocal NFT Community}
The NFT community is an open platform for creators to promote their NFT and projects, as well as a reciprocal space for its members, both creators and other users, to support each other, which makes the NFT landscape more supportive and sustainable.

\vspace{3pt}
\noindent \textbf{NFT Promotions.}
NFT communities such as Discord channels provided artists/creators with a platform to promote their NFT, which was seen as a valuable feature of the NFT community by P1:
\begin{quote}
    \textit{``You can promote your own NFT, as I said, if it's an appropriate channel (in Discord). Especially if you're the owner of a personal project, you can talk to your community, you can engage with them, and answer any questions of a potential buyer.''}
\end{quote}
In addition to Discord channels, P1 also promoted his own and hunted for other artists' NFT on Twitter.
% \begin{quote}
%     \textit{``So I was browsing Twitter. That's my main social channel to promote my own stuff. And I also view other people's stuff. I came across it. I liked the picture, but it wasn't listed as an NFT at the time, so I contacted the creator himself. He said, Yes, it's going to be minted later on tonight. And I just bought, as soon as it was minted.''}
% \end{quote}

Similarly, P2 used Discord channels as a place to connect with buyers, and understand their preferences for NFT. In this way, he was able to create NFT that better met the taste of the market:
\begin{quote}
    \textit{``I'm in 15 Discord channels. Most of the members are buyers. It’s great to connect with people, knowing what type of work they like, so that I can replicate this in my NFT.''}
\end{quote}

Owners of NFT projects would also promote their projects by actively organizing events and attracting people into their community. P5, who was the owner of an NFT company, was organizing an online event at the time of the interview: 
\begin{quote}
    \textit{``We're throwing an event on Thursday to open our gallery in Decentraland. Our main focus right now is sort of building the community and developing the brand.''}
\end{quote}
He also enjoyed creating ties with the community by streaming on Twitch\footnote{\url{https://www.twitch.tv/}. Twitch is a live streaming platform.}:
\begin{quote}
    \textit{``Now we stream on Twitch almost every day. So we're spending hours in the game (Decentraland), just streaming, and meeting people, and then helping them learn how to play the NFT game and create content. Creating relationships with the community and then building things together is a lot of fun.''}
\end{quote}

Such community building and promotion efforts were shown helpful for the development of NFT projects, according to our participants. For example, P11 told us the excitement felt when he was replied directly by a project owner in Discord:
\begin{quote}
    \textit{``I had some issues when playing with an NFT project. So I asked questions in the Discord channel. Then a founder of the project directly sent me some ETH, and asked me to use it as the gas fee to finish my transaction. The project became a success later, then I knew the founder was such a famous person. He solved my issue himself! I didn't believe it until now''}
\end{quote}
% P7 thought community building was a key to the success of NFT projects, and mentioned the friendly atmosphere in the community:
% \begin{quote}
%     \textit{``I believe the success of some NFT projects like CryptoPunk or bored apes is because they create a big community with friendly atmospheres. Some of them are in Twitter and some of them in Clubhouse... In a Clubhouse room, many of us have the ape avatar, and we're like a family. We spend a lot of time talking about our apes. I really like that atmosphere. 
%     % And even in the recent days when the crypto market is bearish, we still have some topics about apes, and the atmosphere in our room is positive. So I think that's the power of NFT projects. That's the power of an active community. The community people are doing some efforts about the apes and  these NFT projects.
%     ''}
% \end{quote}

% P10 observed that the attention paid to new NFT projects by the community would only last for a short time:
% \begin{quote}
%     \textit{``Members of the Telegram group show great interest in new NFT projects. They would try them after seeing the campaigns or ads of the projects, especially those about Metaverse. There're heated discussions about these. But the topic won't last a long time.''}
% \end{quote}

\noindent \textbf{Reciprocity and Mutual Support in the Community.} In the NFT community, there existed a ``chained'' support system where artists helped each other to grow. P12 identified himself as a ``community-based person'', and liked the giving NFT community whose members were sharing, and wanted to help others succeed in this field:
\begin{quote}
    \textit{``Everybody is so sharing and they give me a sense that they really want to help you succeed. They're very open. If you're a newbie and you have a very simple question that you just don't know the answer to, they never try to put you down for not knowing. They're more like, here is the information, here's a place you could go, or here's what I would do with that. It's a very giving community. 
    % You know there's part of the community that will buy your first NFT that you release, because it's your first NFT. They want to get you started. You know they have wealth and so they're like, `hey, you might become something really big in the future, so let me buy your first NFT.' But others are doing it like `hey, let's just get you started. Let's get you moving, get you excited, give you a little push.'
    ''}
\end{quote}

% Some participants mentioned showing support to new creators by buying their NFT. 
NFT artists/creators in our participants tended to give back to the community by buying other artists', specially new artists' NFT to encourage them. P1 did such a thing to show support to new artist, as well as to help grow the NFT community:
\begin{quote}
    \textit{``I set up a goal in my mind: when I reach a milestone, I'll give back to the community by buying an NFT that I actually like. And after I sold my first NFT, I bought one back.''}
\end{quote}
P4 enjoyed collecting different types of NFT and supporting other artists at the same time:
\begin{quote}
    \textit{``I think a big part of my incentive to buy an NFT is knowing that money go directly into the wallet of someone who I think does cool work and who I want to support.''}
\end{quote}
Similarly, P2 bought 
% Justin's Tron Reactor, 
a GIF work, from a less known artist to show support, since ``it was his first sell.'' He also mentioned another reciprocity behavior, i.e., follow-back, among artists on Rarible.
\begin{quote}
    \textit{``When you follow an artist on Rarible, often he would just follow back. I also do this on Twitter, by actively commenting and reacting.''}
\end{quote}

Such reciprocity and mutual support could benefit the growth of each individual artist, as P4 said,
\begin{quote}
    \textit{``I entered this space three months ago, and no one ever knew me or saw me. I didn't have a Twitter profile before that. If you're open to just being a part of the community and growing with others, then you get a lot of followers and friends there to support you. I have never met such a community whose members are willing to grow with each other.''}
\end{quote}

% Good collaboration could also be established in the reciprocal community, as in her case:
% \begin{quote}
%   \textit{``I started as a creator. Now I think I'm a collector too, because I'm connected with a lot of artists and other people through Twitter or Discord. And then I got to know some other artists and made some collaborations. And through this I saw a lot of other art pieces, and wanted to support other artists too. And so, I started to collect also.''}
% \end{quote}

% P3 suggested making use of community support to obtain useful information and help:
% \begin{quote}
%     \textit{``I've gained a very large network of very diverse people. Some of them have actually already become, I would consider friends. You know we talk every single day and we talk on the phone. So yeah, the networking, the community itself around NFT is like, the ability to network and to see who traded what, where they're collecting it, who's supporting who, how much someone is selling, and how much you know the ability to reach out to anyone at any time within this community. I think the networking capabilities are very broad.''}
% \end{quote}

% He also pointed one thing he did not like about the community/social aspect of NFT:
% \begin{quote}
%     \textit{`This is the part I don't like honestly, but owning a specific NFT is giving you a certain level of social status.''}
% \end{quote}
% After he understood the NFT space, he planned to start his own group or become an important voice of another group.

In trader/collector communities, members would share NFT recently bought by them or in a trend with other people, as noticed by P11. They would also kindly remind others of potential risks in the NFT marketplace such as scams. P3 explained,
\begin{quote}
    \textit{``
    % I'm in many different Discord channels. So I think the overall vibe or norm is like, people are very supportive and it's very community-based.
    It's a community that is supporting each other and also pointing out potential problems. For example, recently someone was going around scamming a lot of people and taking their money. Almost everyone in the community was talking about it and saying, `Be careful. They're stealing money.' I think overall it's the norm. It's a very collaborative and supportive environment.''}
\end{quote}
% p13 also told us about the supportive community:
% \begin{quote}
%     \textit{``I guess they think the same (about the value of NFT) because you know they are all new. Everyone is new. It is a great community because they all support each other. It's a cool community. They all work together, they all think it is a great thing.''}
% \end{quote}
% P15 also talked about the supportive, global NFT community:
% \begin{quote}
%     \textit{``When I started posting NFTs for promotion on my Instagram pages or on Twitter, I found a lot of big communities. And I am so excited because you get connections with a lot of good amazing people who can support you and tell you more about this. I am not a native English speaking man. But when I try to connect with other people, they usually helped me to understand how to post, how to release these artworks, about fees, about platforms. And it's amazing to get help from a lot of people from all over the world.''}
% \end{quote}

% \subsection{Summary}
% Our participants created different forms of NFT art, such as 3D paintings and digital Duckies. They heard of NFT either from online resources, or people in real life. Difficulties and challenges were common in their initial experience of minting/creating NFT, but they managed to overcome them with external support. They more or less understood the concepts and characteristics of NFT, and were able to explain it to lay persons who have no prior experience with NFT. Interestingly, they had different motivations for creating NFT, such as brand developing, earning money, interest in blockchain technology, empowerment of users, pleasure and a sense of accomplishment, etc. In NFT communities such as Discord channels of NFT projects, people exchanged ideas and promoted their NFT selling. They also talked about recent NFT scams to remind other potential victims. Reciprocity and mutual support were found common among NFT artists, which were beneficial for both individual development and effective collaboration. Challenges and drawbacks experienced by the NFT landscape included technical issues of newly launched NFT projects and marketplaces, lack of regulation which led to the prevalence of low-quality NFT and scams, as well as Ethereum-introduced flaws such as high gas fee and environmental impact. \zhixuan{need rewriting

==> section/5_Discussion.tex <==
\section{Discussion} 


\yun{if the interview findings shed any light on what to regulate, who regulate, how to regulate… that could be a strong discussion point.}

\yun{From some other social media moderation paper, we got to see some consideration of values, where there is an absence of value "inspiration/creativity". However, students in class, they want to receive inspirations from social media or online communities, especially design students. But I don’t see a lot of related topics discussed in typical moderation papers.} 

Our study aims to understand users' perceptions of and engagement in the NFT marketplace and community. We look at NFT practices from different angles, i.e., both individual-level motivations and behaviors, and community-level interactions. We also reveal drawbacks and limitations of the NFT marketplace. After recapping our main findings, we will propose design implications on existing issues in the NFT marketplace, such as high gas fee and the tension between providing a lower barrier and ensuring NFT quality, and how different stakeholders can collectively build a more supportive and sustainable NFT community. 

\subsection{Recap of Main Findings}
Since there is not much prior work focusing on NFT, we present an exploratory study to understand users' motivations for creating NFT, criteria for good NFT, user interactions and community dynamics in the NFT marketplace, and user's perceived drawbacks and limitations of the NFT marketplace. 

\subsubsection{Perceived Advantages and Limitations of  NFT}
% Creative commercial community is designed to collaborate and compete with an aim to influence the success of objects or goods. Members participate in a range of ways to construct the trading environment as we explained in section 3.1. We found studies of such commercial creative community where research has been conducted to understand social interaction, and material conduct of trading operation to indicate the factors of the community success \cite{auction}. 
Understanding how 
% these platforms operates within different stakeholders, how
different stakeholders such as NFT creators/artists and collectors/traders perceive the pros and cons of the marketplace might help create a more sustainable and  creative NFT community. 
% In our study, we have found mainly three types of stakeholders in NFT community which includes, creator, collector and trader. 
% Unlike existing literature of creative community, we noticed a NFT user to be potentially active in one/more roles at the same time while interacting with this marketplace.

Our participants expressed their positive perceptions of NFT. In addition to features inherited from the underlying blockchain such as provable ownership and uniqueness of NFT items, our participants also valued NFT as a way of collaboration (7/15), empowering artists (6/15) and proving digital identities (9/15). The NFT community was also described by them to be optimistic about the future of NFT and blockchain. Many see NFT as an ongoing art revolution, and want to be a part of it. 
% In aspect of collaboration, participants shares a range of approaches, they participate in community, working on similar ideas for projects,  providing constructive criticism for each other's work, voicing support for other NFT creators. This indicates that collaboration in NFT market can be improved for sustainability. Previous research indicates that collaboration can be a significant a factors for mutual profits from the sale of the product in commercial creative market \cite{paulini2014motivating}. Furthermore, digital identity and art empowerment seem unique perceptions in case of NFT marketplace. NFT artists feel empowered by the functionality of blockchain (smart contract) which automates their business workflow and remove the barriers from intermediaries (govt. sponsors). Additionally, they are now able to hold an unique digital identity as a artist.

% In NFT community, we notice quantifying the quality of art differently. This includes the judgements of aesthetic quality, utility and heuristics (i.e., artists' reputation). Previous literature examined some similar meaning of good quality traditional art where aesthetic quality has been frequently indicated as a measure for good quality \cite{cupchik1988search}. Studies considered representation and visual effects as a metrics for aesthetic quality of art \cite{cupchik1988search}. We found our participants to explain the representation of NFT and use of media as aesthetic meaning of art. Utility of NFT art seems to be considered as a topic of debate among NFT community. Participants tend to follow some heuristics, such as, artist' reputation as a measurement for good quality NFT. This aligns with similar trend of the traditional art where artist's reputation significantly influence the price of art.

However, our participants also mentioned challenges facing the NFT marketplace, including technical issues of NFT platforms, security risks (scams), lack of effective regulation which leads to the prevalence of low-quality NFT, and blockchain-induced challenges such as energy consumption and high gas fee. 
% the main issues are security risks and lack of regulation. While NFT users seem to be developing external online support groups as their communities of practice, it is raising issues with NFT scam. 
% Participants mentioned that malicious users frequently post scam NFT or copy of famous NFT in different community groups in Discord, Twitter which lead to financial loss for community. Furthermore, participants indicated lack of regulation imposed. 
Some NFT platforms include features to solve some of these issues, e.g., hiring moderators to filter low-quality NFT, use an ``invite-only'' mechanism, etc., but they are not effective enough to solve the issues. Also, the regulatory efforts are not consistent across different platforms: not a single platform practices all the measures.  
% copyright issues - but majority of platforms are not secure at this point. 

% while the success of sale depends on the visibility of NFT, our participants mentioned that well-known artists with a better social media following (i.e., more followers) enjoyed better visibility, whose NFT was recommended to more platform users, while less-known artists got much less attention.

% Our participants also pointed out unfavorable features of NFT trading platforms, which made the NFT marketplace less of a fair and inclusive space. For example, Rarible and Opensea were reported by our participants to charge high minting fee and gas fee during creation and transaction, 
% Though participants endorsed self regulated media in NFT marketplace for selling art, 
% which demotivates many from participating and creating NFT art. 
% Additionally, 
% since the NFT marketplace is a creator-centric model,
% We thus call for more decentralization in the recommendation system of NFT trading platforms, which gives artists, either well-known or less-known ones, an equal chance to be seen. 

In section~\ref{design}, we will propose specific design implications to enhance the positive aspects of the NFT marketplace, and address challenges facing it.

\subsubsection{Intrinsic \& Extrinsic Motivations for Engaging with NFT}
In the context of traditional online innovation communities, the participation is driven by both intrinsic motivations, such as fun and challenge \cite{nov2007motivates}. In a previous study \cite{innovation}, intrinsic motivations proved to be effective for initial participation and long term engagement in online innovation communities \cite{innovation}. The majority of participants were engaged to the online innovation community for fun and activities that challenged them. Extrinsic motivations such as reward were reported as well \cite{lakhani2003hackers} 

% In most cases, participants' roles were contributors/collaborators instead of leaders.

% {Motivations for Participating in NFT Marketplace}
\zhixuan{I'm not sure whether we correctly categorize these intrinsic and extrinsic motivations}
In our participants, we also found both intrinsic and extrinsic motivations for engaging in the NFT marketplace. While some participants mentioned joining the NFT marketplace during pandemic for a living (extrinsic), their passion for the art revolution (intrinsic) motivated them to keep engaging with the marketplace. Some tried to keep up with the times (intrinsic) through interacting with cutting-edge blockchain technology, echoing well with literature which shows that learning new things and intellectual challenges are main intrinsic factors for participating in innovative activities \cite{rafaeli2008online}. Some stayed in the marketplace for a sense of belonging to the community, and building community ties (intrinsic), which was also previously reported as motivations for engaging with innovation communities \cite{franke2003communities}. Other intrinsic motivations include expressing creativity and
personal interest, searching for community support (discussed more in section \ref{comm}), etc. Other extrinsic motivations of our participants include earning money by selling NFT, receiving private/public acknowledgement, etc. 
% Given the high price and huge price fluctuation of NFT, many turn to NFT trading for speculation purposes. 
% , owning business without regulation to be their reason of interacting to this platform. 
% A few mentioned to be recognized in their respective intellectual area and enhancing reputation in community. 
% For example, P12 mentioned to build fan base in different social media. Participants also frequently mentioned to experience some community members to frequent post in their community circle to stimulate success rate of selling goods. 

% such as an empowering and encouraging community. There are responses from our participants that represent reciprocity and mutual support among NFT artists: some collect NFT solely to support the community and encourage other artists. Generally, we observe a significant optimism among NFT users, even though there are technical issues with NFT platforms, a lack of regulation in the NFT marketplace, and high gas fees along with other Ethereum-induced constraints.   

\subsubsection{Individual Practices around NFT}
% - RQ3: practices (note: pay attention to their challenges and their mitigation strategies, which become ideas for design implications)
%     -- how they discover NFT
%     -- how they create/mint NFT (for artists who are not particularly technical)
%     -- how they trade/buy/sell NFT (e.g., how they identify scams)
%     -- how they use NFT (esp. for NFT that has utilities, as a ticket)
%   
    
% \textbf{Creator-Centric Ownership Model}
% Most of the participants in our study started their interacting with NFT community during this pandemic. 
Our participants discovered the NFT marketplace from  various information sources, and had different initial experiences. Some knew NFT for the hype on social media, and record-breaking bids of NFT. Some knew NFT from people they followed on social media platforms such as Twitter and YouTube. Some learned NFT from their friends and family. Another common way they got to know NFT was online social groups, such as Clubhouse rooms and Discord channels. 

Very few of them had prior experience of blockchain and cryptocurrency. In other words, the majority of our participants were not tech savvy. Instead, they had diverse, non-technical background such as musician, tattoo artist, photographer, etc. Therefore, they encountered more or less difficulty during minting and creating their first NFTs. For example, some did not know how to set up crypto wallet accounts and deposit cryptocurrency to mint NFT. For some participants, blockchain- and NFT- related concepts were hard to understand and intimidating. When coming across difficulties, it was common for our participants to seek external support from their friends, community members, or platform representatives. Discord and Twitter served as open platforms for our participants to post questions and get answers. 
% One participant explained his experience to get help from rarible account on Twitter to successfully minted his first NFT. 
Generally, new NFT users 
% are comfortable with relying on external online social media groups outside NFT marketplace. They scrupulously 
make an effort to seek external support, and even develop their online support groups, e.g., creating Discord channels and relying on each other for information and support (detailed in \ref{comm}). 
% This also suggests that online spaces for interaction between community offered by innovative commercial platforms can measure the success of  community members.

Different roles in the NFT marketplace were found in our participants, such as creators/artists, collectors, traders, and developers. Some took more than one role, e.g., identifying themselves as both a creator and a collector. We found NFT creators to be empowered by the open marketplace.
% general engagement model in the NFT marketplace is leaning toward creator-centered since almost all participants identified themselves as creators and collectors. 
% Recent reports on the NFT marketplace highlighted that the rise of NFT has renewed the idea of developing a new ownership model to make it more creator-centric \footnote{https://www.dwt.com/insights/2021/03/what-are-non-fungible-tokens}. 
Blockchain-powered smart contracts allowed them to have a viable environment to monetize from their art without intermediaries, and provided them with lower barriers to entry and more freedom in art creation. Our participants indicated that unlike traditional art markets/auctions where artists were obligated to pay intermediaries (e.g., sponsors) during the sale, the NFT marketplace gave users full control to create and sell their NFT out of their own will. 
% However, there are some issues of scams in NFT marketplace. The common practice among NFT community group to provide alert to other members about known scams. According to participants, the reminders from other community members is the ideal way to  prevent people from falling for scams.

\subsubsection{Community Practices of NFT} 
\label{comm}

%   -- interact with others in the community
%         --- NFT promotions (grassroot)
%         --- mutual support (between creators)

Our study reflects different social interactions among community members, such as mutual support and collaboration. 
% In literature, an emerging topic in traditional art market is trust. In the process, trust is established in the community to buy and sell goods \cite{auction}. Information on provenance of goods and an open market for bidding create trustworthy and reliability which reduces the information asymmetry between different trading parties (i.e., buyers and sellers). We also found in literature that community success is measured in terms of the number of online creative collaborations completed \cite{paulini2014motivating}.

\noindent \textbf{Helpful and Reciprocal NFT Community.}
According to our participants, online communities, such as Twitter accounts and Discord channels of NFT projects, are go-to places for exchanging ideas with people who share similar interests, and promoting their NFT work. By connecting with buyers, artists are also able to understand their preferences for NFT, thus create arts that meet users' taste and sell better on the market. Even those who are not NFT creators can still benefit by participating in the community. For example, they can get first-hand information about newly-created NFT. Members of Discord channels would also kindly remind others about recent suspicious activities and spams to prevent them from financial loss. For example, one participant shared a personal experience of getting alert from a community member regarding a spam NFT, preventing him from falling for it. Later, he provided another NFT creator with potential sale opportunities. 

There exists reciprocity and mutual support in the NFT community where participants willingly assist and support each other, which was found especially common among NFT artists/creators. Some participants mentioned buying other artists' work just to show support. It was repeatedly mentioned that selling the first NFT was the hardest part, and a few participants were demotivated due to the long time period before they sold their first piece. In this regard, such support was valuable in helping new artists grow their career. Follow-back behavior was also found on NFT trading platforms such as Rarible: if an artist was followed by another one, she would follow back right away. In this way, each individual artist could better grow her social following on this platform.
% Such reciprocity was good for the development of each individual artist.

\noindent \textbf{Opportunities for Collaborative and Collective Innovation.}
Out study presented a few events of collective/collaborative NFT creation in the NFT marketplace. POAP.art\footnote{\url{https://poap.art/}} was such an example mentioned by P9, where people could collectively finish an NFT painting on the virtual canvas. P6 mentioned how the artist community collaboratively proposed new forms of NFT art. Online meetings were organized by NFT platform founders and developers to discuss how to create a better NFT
ecosystem for artists. Some participants also expressed their interest in collaboration in the near future, once they have built their own skills. However, collaboration in NFT creation was not common among our participants, since mainstream NFT platforms such as Opensea and Rarible did not support such a function.

Literature has shown that the success of an innovation community can be measured in terms of the number of completed creative collaborations \cite{luther2010works}. Collaboration can also help foster a supportive and sustainable marketplace. Thus the NFT community might want to consider collective and collaborative creation of NFT as an opportunity to enhance the ties between NFT artists, and create a sustainable community.

\subsection{Design Implications}
\review{There is some more analysis and reflection presented in the discussion, which with more refinement could be neatly interwoven in the findings section. On the whole however, many of the discussion points are familiar to prior work in use of crypto apps (see papers below!), and furthermore lack any deeper criticality, especially around more problematic issues of NFTs (e.g. energy use, fraud, shilling, lack of clear ownership rights etc.) Similarly, the design implications presented are very broad, and repeat familiar challenges  of existing crypto applications e.g. around usability, trust, cost, fraud, regulation etc. which are already well known. I think this shortcoming ultimately stems back to the broad and exploratory nature of the study, and lack of engagement with prior work.}

\yun{basically, the reviewers want to see some languages that clearly state "our findings about XXX is not discussed in prior literature or our findings about XXX is discussed previously, but we expanded the understanding with a new factor that contributed to the xxx.}
\label{design}
% \tanusree{* 2-4 main design implication}
% \tanusree{some raw ideas. need to articulate into design suggestion}
% - design implications
%     -- high gas fee, dedicated blockchain just for NFT (Flow, WAX), ETH (side chains, L2)
%     -- help creators promote their NFT (recommender system, )
%     -- help users discover high-quality NFT (reviews, also helpful for detecting scams)
%     -- support creation of new/diverse types of NFT (e.g., meebit, programmable)
%     -- support easy creation for those who are not technical or who are not artists (e.g., educational materials, usable templates so no need for programming, future work)

\subsubsection{Lower Gas Fee for NFT Creation and Transactions}
The Ethereum blockchain, on which many NFT projects are built, introduces several challenges to the NFT world. The high gas fee on Ethereum was repeatedly mentioned and complained by our participants, which set a high barrier for new artists who could not afford to mint NFT. Even for mature artists, their monetary return could be compromised to a large extent. For example, a participant indicated that the gas fee accounted for 61\% of his total NFT sell.  

Generally, the high gas fee on Ethereum makes NFT creation and trading exclusionary for artists. To make the NFT space more inclusive, one may build NFT platforms on Layer-2 blockchains \cite{layer2} such as OMG Network\footnote{\url{https://omg.network/}}, and/or dedicated blockchains for NFT such as Flow \footnote{\url{https://www.onflow.org/}} and WAX \footnote{\url{https://on.wax.io/wax-io/}}, where cheaper transactions are supported. 

\subsubsection{Fairer Recommender Systems to Support Inexperienced Creators and Users}
% There exists a power dimension and popularity based promotion in the NFT marketplace and NFT associated external online groups. 
%We find unfairness when it comes to the visibility of NFT created by artists of different popularity.
Popular artists who already have a strong fan base on social media platforms can sell more NFT at higher prices within a short period of time. NFT trading platforms also promote their work more often, probably for higher monetary return. In comparison, it is much more difficult for artists and creators who just start their career to promote their NFT. Our participants explicitly expressed this as a demotivating factor. %For example, music producer Grimes sold his NFT for almost \$6M in 20 minutes \footnote{https://www.theguardian.com/music/2021/mar/02/grimes-sells-digital-art-collection-non-fungible-tokens}, while one of our participants who was a photographer failed to sell any NFT out in the past month.

To better support less-known or inexperienced NFT creators, we advocate for fairer recommender systems that promote NFT based on more factors such as content genre and user reviews, instead of just the fame of the creators. A desirable property of such a recommender systems is diversity of recommendations, so that creators with different levels of experience and fame could be seen by others.

\begin{comment}
compared to E-commerce websites such as Amazon,
% , facebook online marketplace, 
which recommended NFT to users who might have interest in it. 
% items based on like, comments, stars provided by NFT community members.

According to our participants, NFT created by less-known artists was less likely to be promoted  and seen. 
% This will provide a space for comparatively fair chance for artist to sell their NFT goods. 
% A community based item-to-item collaborative recommendation system provide more decentralization in NFT trading platforms. 
Thus we advocate for more decentralization in recommendation algorithms. Instead of only or mostly recommending famous artists' NFT to users, less-known artists with fewer followers should also enjoy some visibility. 
\end{comment}

\subsubsection{Detecting Low-Quality NFT and Warning about Scams}

% Many of NFT's pros and cons are related to the blockchain underlying it. For example, irreversibility of blockchain appears to be a blessing among the NFT community, which could be utilized to verify digital ownership of arts. Participants also favor provable scarcity of NFT, which is achieved by hard-coding the number of copies of a certain art in smart contracts. In many cases, there is only one copy of a certain NFT art, which makes it extremely scarce and valuable. Moreover, participants like the automatic way of transactions on the blockchain ledger, which is regarded by them as a more convenient business model, and they do not need to worry about tracking receipts. 

Lack of regulation of the decentralized blockchain introduces several challenges for NFT, such as the prevalence of low-quality NFT and scams. Low-quality NFT created and spammed by those who merely pursue monetary return not only degrades general quality of the NFT marketplace, but also demotivates artists who have put a lot of effort into their work. From our study, it seems that high gas fee plays the role of a regulator, because not everybody can afford to mint. However, this is not a sustainable way of regulation, and puts a heavy burden on passionate artists in a poor financial standing. Loose, limited regulation can be found on NFT trading platforms such as Rarible, e.g., artists can opt to go through a Twitter verification process, and those who do so can enjoy more visibility for their posted NFT. However, low-quality NFT and scams are still prevalent despite all the regulatory efforts. 

To effectively and scalably solve this issue, AI algorithms can be designed and deployed by the platforms to detect scams and low-quality NFT. A key challenge facing such a system is how it can surface and promote legitimate NFT created by inexperienced creators, which may not look that fancy or high-quality. 

On-chain NFT trading data, social media data, and user reviews for NFT items can also play a role in making users aware of scams and quality issues. We can further make the warning interactive by putting negative reviews on top of suspicious NFT, which users could click on and see more related reviews regarding creativity, scarcity, and estimated effort. To encourage production of honest user reviews, rewards (e.g., earning governance tokens) and penalties (e.g., slushing \zhixuan{what does it mean?} or taking away collateralized tokens as seen in proof-of-stake consensus mechanisms) could be practiced.

% The user reviews could be multi-dimensional including factors such as . %To screen out low-quality NFTs, proxy measures such as rough estimate of the time spent on creating the NFT underlying asset can complement user reviews. 
% 

\subsubsection{Supporting Easy Creation and Purchasing for Non-Technical Users} 
The NFT space includes a diverse set of users who may have limited technology background. Our study indicated that participants especially newbies were often intimidated by the conversation around crypto and NFT, which included too many tech-heavy concepts and vocabulary. NFT collectors and creators also felt it cumbersome and time-consuming to buy and mint NFT. 

Despite the rapid development of blockchain, which leads to many cutting-edge applications \cite{wang2021non}, the usability aspect of blockchain is paid less attention to. Thus we call for more research in blockchain and NFT usability, which aims to improve user experience and accessibility of the relatively new technology, and allow more people to participate in the ongoing financial/art revolution. Specifically, educational materials, usable templates for creating NFT are example ways to make it easier for people who are not technical to create and buy NFT. 
% However, we need further research to understand the usability aspect of NFT platform.

\subsubsection{Maintaining Engagement by Ensuring Quality}
Several participants mentioned that members of the NFT community were more passionate about their participation when they were newcomers, and the passion dropped later. Also, trending topics in Discord channels and Clubhouse rooms are constantly changing. When an NFT project or piece is newly released, members would heatedly discuss it, but only for a few days. Out of thousands of NFT projects, only several of them survive and still enjoy popularity till now, such as NBA Top Shots, and Decentraland. 

Thus project owners and NFT creators might need to make an effort to improve the quality of their projects/works, so as to survive people's long-term fatigue and decreased interest. NFT trading platforms can take an active role in improving the quality of NFT, either hiring moderators to manually filter low-quality NFT out, or leverage off-the-shelf AI models to do this.

% \begin{quote}
% `` \it{In today's society of instant gratification and consumption, having to transfer monies into crypto-currency then log into different online wallets and accounts for different fees and processes is too expensive and complicated for many.''} 
% \end{quote}

\subsubsection{Regulation vs. Openness}
A tension between providing a lower barrier and ensuring NFT quality exists in the NFT marketplace. The open nature of NFT and general blockchain removes gatekeepers in the traditional art market, and provides a low barrier to entry for NFT creators to participate. However, the low entry barrier also leads to low-quality NFT and even scams, since everyone is able to mint and trade NFT in the market. 

NFT trading platforms practice different types of restrictions to prevent unexpected scams or low-quality art. For example, Foundation uses an ``invite-only" mechanism for the entry of artists: only invited artists can mint NFT on the platform. Such efforts are intrinsically two-edged swords. Despite their effectiveness in improving NFT quality, they also prevent talented yet poor artists from creating their own art, and become hurdles to creating an open-access domain for everyone, which goes against the initial vision of blockchain. Considerably more research needs to be conducted to find alternative ways of regulation, which ensures quality and decentralization at the same time.

% Individuals might re-prioritise motivating factors at different times based on how well they are satisfied. 
% In this section, we will reflect on reciprocity and mutual support in the NFT community. 
% in the current NFT landscape, and propose corresponding design implications for a more supportive and sustainable NFT community. 

% In this section, we map our results of NFT community dynamics to physical art auction and exhibition environment \cite{o2012impact}, \cite{rizzo2007fire}, \cite{vosinakis2011virtual} to highlight what are the similarities and differences between the two space. We choose these prior work of art exhibition phenomena because 1) this scenario is closely similar with NFT community,  2) there isn’t previous work of NFT to compare this platform’s characteristic and limitation. The goal of this study instead of generating an exhaustive list of similarities to first attempt to answer the question related to current  practices and community interaction of NFT and how existing social/community interaction as well as regulation present in physical art auction world can be adopted in NFT community to improve interaction among NFT users to create a sustainable marketplace. In addition, we present what are the  technological/ social design implication of NFT marketplace that causing users’ to be engaged and motivated. We also report that NFT’s features- augmented with technologies, could contribute to disseminating people's lifestyle values in public and can improve social interaction to build a empathetic and supportive community.

\subsection{Limitations and Future Work} 

There are four main limitations of our work. Firstly, the sampling size was relatively small (N=15). However, we had a diverse participant background: artists/creators, collectors, and traders. Thus we were able to collect rich data (perceptions and practices) from different stakeholders of the NFT marketplace. As a follow-up work, one may want to conduct a larger-scale survey study to obtain more quantitative findings and insights.

Secondly, although our participants were from 9 different countries (China*4, USA*4, UAE*1, Canada*1, Switzerland*1, Iran*1, Belarus*1, Germany*1, Argentina*1), we did not inspect NFT from the angle of cultural differences, which we leave as a future work.

Thirdly, our findings on community practices were mostly inferred from interview data, combined with some observations during the recruitment process. It might be interesting to do an observation-based study, and find more community values and norms. 

Lastly, most of our participants (13/15) were male. Future research could examine the demographic distribution of NFT users, and the reason why certain demographic groups are less interested in NFT, towards making it more widely adopted. 

==> section/Background_on_Blockchain_and_NFT.tex <==
\section{Background on Blockchain and NFT}

\subsection{Blockchain}
Blockchain was originally proposed by Satoshi Nakamoto where a proof of work (PoW) mechanism was used to reach a consensus on transaction data among untrusted participants in a peer-to-peer network \cite{nakamoto2019bitcoin, garay2017bitcoin}. 
% The idea of blockchain is to agreed upon in a concensus with a large network of untrusted participants \cite{garay2017bitcoin}.
A blockchain is like a public ledger containing a sequence of blocks, which hold the complete transaction records. Each block is validated by nodes in the network using cryptographic means. In addition to transaction data, each block contains a timestamp, the hash value of the previous block, and a random number for verifying the hash \cite{chuen2017handbook}. Hash values are unique, and fraud can be effectively prevented, since changes of a block would immediately change the respective hash value. Generally. the PoW mechanism ensures the integrity of the entire blockchain.


Bitcoin (BTC) \cite{bitcoin}, the first application of blockchain, is a kind of cryptocurrency. Owners have full control over bitcoin, and are able to transact it at their own discretion and without geographical constraints. It excludes involvement of any centralized authority such as governments and banks, and is free of regulation and censorship, thus protecting anonymity of users. Furthermore, mechanisms of blockchain, such as distributed consensus, reduce the risk of cyber attacks and make transactions more secure.
% People use such virtual currency/digital tokens which is cryptocurrency \cite{conti2018survey}. 

Blockchain is applied to a diverse range of settings beyond cryptocurrency \cite{conti2018survey}. The spectrum of blockchain applications ranges from financial services (e.g., decentralized exchanges, settlement of financial assets, and payment systems), risk management, Internet of Things, to public and social services \cite{zheng2018blockchain, yli2016current}. 

\subsection{Non-Fungible Tokens (NFT)}

NFT is a new type of blockchain-based digital assets, which is catching more and more attention for its uniqueness and provable scarcity. 

The most prevailing blockchain used for NFT is Ethereum \cite{wood2014ethereum}. Ethereum provides a secure environment for executing smart contracts, which are computer programs used to carry out predefined functions. There are blockchain customized for NFT though, e.g.,  Flow\footnote{\url{https://www.onflow.org/}}. Ethereum token standards guarantee that a certain asset will behave in a specific way, and specify how people can interact with basic functions of the asset. ERC-20 standard supports the creation of fungible tokens. For example, one can own and trade 0.1 and 0.01 of an ERC-20 token on the market. In contrast, NFT is non-fungible, and cannot be divided or merged. Each NFT is unique, representing the ownership of different items ranging from image and audio files to email and Twitter accounts \cite{abarbanel2019vgo}. Several Ethereum standards support the creation and trading of NFT. For instances, ERC-721 \cite{721} proposed back in 2018 is exclusively used to create NFT. It provides functionalities to transfer tokens from one account to another, get the current token balance of an account, get the owner of a specific token, and get the total supply of a token available on the network \cite{721}. ERC-1155 \cite{1155} proposed in the same year can be used to create both fungible and non-fungible tokens. 

NFT creators and buyers are two main stakeholders in the market. An NFT creator creates an NFT by signing a transaction, including the hash of NFT data, and sending the transaction to the underlying smart contract. When the smart contract receives the transaction with NFT data, the minting process begins. The minted NFT is associated with a unique identifier in the blockchain, which is an evidence of ownership for NFT owners \cite{hong2019design}. When any further trading of a certain NFT is confirmed, the NFT metadata and ownership details are added to a new block and used to preserve the ownership.

\noindent \textbf{History of NFT}
\review{the nature of what an NFT actually is, in relation to a digital asset, and what an NFT means (or does not mean) in relation to owning an asset. A short history of the development of NFTs, from Smart Contracts, through to CryptoKitties, and their recent hype, as well as an introduction to key marketplaces and concepts would also support the reader significantly. In addition, NFTs have been extensively debated in the art world, and tech press - it would have been good to see some of the key tensions surrounding NFTs introduced up front.}
\review{move forward with the project is to dig deeper into the motivation for the work.} \zhixuan{added the history of NFT ecosystem (including projects, infrastructure and marketplace)}

\cite{NFT-history} is a good summary of the history of NFT. The notion of NFT, i.e., unique digital assets, had become popular before NFT standards were established on Ethereum. Back in 2017, memes started to be traded on Ethereum. In the same year, John Watkinson and Matt Hall created unique characters, i.e., Cryptopunks, on the Ethereum blockchain. Each character was different, and the number of characters was limited to 10,000. The first project to use the ERC-721 NFT standard was the famous CryptoKitties, which was on every news station, from CoinDesk to CNN. People made crazy profits by trading the virtual cats. 

The years of 2018 and 2019 saw a massive growth within the NFT ecosystem. Hundreds of NFT projects emerged. NFT marketplaces were also thriving, led by OpenSea. Web3 wallets such as Metamask further made it easier for people to participate in the NFT space. NFT projects (e.g., games and collectibles), infrastructure (e.g., crypto wallet), and NFT marketplaces together made up the NFT ecosystem.  

% followed by the trading process. 
% The NFT trading mechanisms are basically the logic of utilized token standards. Once the transaction is confirmed by smart contract, the minting process becomes complete.

% NFTs has an inheritable Solidity smart contract standard which is ERC721, meaning that developers can easily create new ERC721-compliant contracts by importing it from their specified library OpenZeppelin library \footnote{\url{https://github.com/OpenZeppelin/openzeppelin-contracts/blob/master/contracts/token/ERC721/ERC721.sol}}. Most NFT solutions rely on smart contract based blockchain platforms to ensure their order-sensitive executions. To transfer NFTs, the owner must prove in possession of the corresponding private key and send the assets to another address with a correct digital signature. This simple operation is usually performed using a cryptocurrency wallet and is represented as sending a transaction to involve smart contracts standards like, ERC-777 \footnote{https://eips.ethereum.org/EIPS/eip-777}, ERC721 \cite{721}. ERC-1155 \cite{1155}. 

%  In the mainstream blockchain systems such as Bitcoin \cite{nakamoto2019bitcoin} and Ethereum \cite{wang2021non}, they employ hex values to encode transaction elements such as the function names, parameters and return values. This implies that the raw NFT data must follow these rules. If one claims that they owns the NFT-based intellectual property, they essentially owns the original piece of hex values signed by the creator. Others can freely copy the raw data, but they cannot claim ownership of the property. Based on that, we can observe that the NFT-related activities (e.g. buy, sell, trade, auction) have to be processed under these four phases, similar to the basic processing procedure of smart contracts.

% One form of blockchain that certifies digital asset is NFT.

% , EOS \footnote{Wax:worldwide asset exchange. Project Accessible: https://github.com/worldwide-asset-exchange/whitepaper (2021)}. 
% One pioneer is Patientory \footnote{\url{https://patientory.com/}}, which is a healthcare application. In the year of 2017, they created 100 million tokens, and 70 million of those have been sold and traded publicly in the cryptocurrency market. They implemented the tokens with their private Ethereum-based blockchain, with which patients can pay assigned doctors in an incentivized way. They can also securely access and transfer protected health information while providing actionable insights to improve health outcomes on the blockchain. 

% Another application is Privacy-preserving token management system for permissioned blockchains which support fine-grained auditing and one of the finest implications of blockchain \cite{androulaki2020privacy}. Research proposed applications in the renewable Energy Market, including a robo-advisor which suggest consumers the best selling strategy based on block generated information \cite{energy-market}. 


% \subsection{\textcolor{black}{Existing Practices/Standards for Fungible and Non-fungible Tokens}}

% Blockchain technology is a radical innovation with the potential to challenge or even replace existing financial and business models relying on third parties. In blockchain, any user is able to create and deploy programs/tokens on a shared global infrastructure with their smart contracts \cite{eth}. Initial Coin Offerings (ICOs) that re-invent crowdfunding through the use of blockchain to tokenize assets has been a public attention, enabled by the ERC-20 standard on Ethereum.

% The standards provide a unique mapping of assets to addresses/owners, and a permissioned way of transferring these assets. 

% The ERC-721 introduces a standard for NFT, in other words, this type of Token is unique and can have different value than another Token from the same Smart Contract due to its age, rarity. 

% There are also several other NFT standards emerging on other blockchains. DGoods, pioneered by the Mythical Games team, is focused on providing a feature-rich cross-chain standard starting with EOS \cite{nft1}.

%  \subsubsection{High-level Protocols of NFT} 
% Primarily NFT consisnts of two roles: NFT owner and NFT buyer. During the entire process, there are some protocol and activities for which it requires an underlying distributed ledger for keeping list of records as well as perform trading in P2P network. 

==> section/HCI-CSCW_references.tex <==
Elsden, C., Manohar, A., Briggs, J.,  Harding, M., Speed, C., & Vines, J. (2018,
	April). Making sense of  blockchain applications: A typology for HCI. In
	Proceedings of the 2018 CHI Conference on Human Factors in Computing Systems (pp.
	1-14).

	Michael Froehlich, Maurizio Raphael Wagenhaus, Albrecht Schmidt, and Florian Alt.
	2021. Don’t Stop Me Now! Exploring Challenges Of First-Time Cryptocurrency Users.
	In Designing Interactive Systems Conference 2021 (DIS '21). Association for
	Computing Machinery, New York, NY, USA, 138–148.
	DOI:https://urldefense.com/v3/__https://doi.org/10.1145/3461778.3462071__;!!DZ3fjg!rsAh7A_d2lxYWpIvjcVJkRBRd4hNU1CQOL4m_QQbhGUcUvsjpbkU3BWg4xFQ17j-yQ$

	Eaman Jahani, Peter M. Krafft, Yoshihiko Suhara, Esteban Moro, and Alex Sandy
	Pentland. 2018. ScamCoins, S*** Posters, and the Search for the Next BitcoinTM:
	Collective Sensemaking in Cryptocurrency Discussions. Proc. ACM Hum.-Comput.
	Interact. 2, CSCW, Article 79 (November 2018), 28 pages. DOI:
	https://urldefense.com/v3/__https://doi.org/10.1145/3274348__;!!DZ3fjg!rsAh7A_d2lxYWpIvjcVJkRBRd4hNU1CQOL4m_QQbhGUcUvsjpbkU3BWg4xE1p45Gjg$

	Xianyi Gao, Gradeigh D. Clark, and Janne Lindqvist.  2016. Of Two Minds, Multiple
	Addresses, and One Ledger: Characterizing Opinions, Knowledge, and Perceptions of
	Bitcoin Across Users and Non-Users. In Proceedings of the 2016 CHI Conference on
	Human Factors in Computing Systems (CHI ’16), 1656–1668.
	https://urldefense.com/v3/__https://doi.org/10.1145/2858036.2858049__;!!DZ3fjg!rsAh7A_d2lxYWpIvjcVJkRBRd4hNU1CQOL4m_QQbhGUcUvsjpbkU3BWg4xFCspQ3rA$

	Yong Ming Kow and Xianghua Ding. 2016. “Hey, I  Know What This is!”: Cultural
	Affinities and Early Stage Appropriation of the Emerging Bitcoin Technology. In
	Proceedings of the 19th International Conference on Supporting Group Work (GROUP
	’16), 213–221. https://urldefense.com/v3/__https://doi.org/10.1145/2957276.2957279__;!!DZ3fjg!rsAh7A_d2lxYWpIvjcVJkRBRd4hNU1CQOL4m_QQbhGUcUvsjpbkU3BWg4xHbwMv14w$

	Caitlin Lustig and Bonnie Nardi. 2015. Algorithmic Authority: The Case of Bitcoin.
	In 2015 48th Hawaii International Conference on System Sciences, 743–752.
	https://urldefense.com/v3/__https://doi.org/10.1109/HICSS.2015.95__;!!DZ3fjg!rsAh7A_d2lxYWpIvjcVJkRBRd4hNU1CQOL4m_QQbhGUcUvsjpbkU3BWg4xELnRx00Q$

	Caitlin Lustig. 2019. Intersecting Imaginaries: Visions of Decentralized
	Autonomous Systems. Proc. ACM Hum.-Comput. Interact. 3, CSCW, Article 210
	(November 2019), 27 pages. DOI:https://urldefense.com/v3/__https://doi.org/10.1145/3359312__;!!DZ3fjg!rsAh7A_d2lxYWpIvjcVJkRBRd4hNU1CQOL4m_QQbhGUcUvsjpbkU3BWg4xESFD4XNQ$

	Kow, Y. M., & Lustig, C. (2018). Imaginaries and crystallization processes in
	Bitcoin infrastructuring. Computer Supported Cooperative Work (CSCW), 27(2),
	209-232.

	Karim Jabbar and Pernille Bjørn. 2017. Growing the Blockchain Information
	Infrastructure. In Proceedings of the 2017 CHI Conference on Human Factors in
	Computing Systems (CHI ’17), 6487–6498. https://urldefense.com/v3/__https://doi.org/10.1145/3025453.3025959__;!!DZ3fjg!rsAh7A_d2lxYWpIvjcVJkRBRd4hNU1CQOL4m_QQbhGUcUvsjpbkU3BWg4xG3wVB2bw$

	Corina Sas and Irni Eliana Khairuddin. 2017. Design for Trust: An Exploration of
	the Challenges and Opportunities of Bitcoin Users. In Proceedings of the 2017 CHI
	Conference on Human Factors in Computing Systems (CHI ’17), 6499–6510.
	https://urldefense.com/v3/__https://doi.org/10.1145/3025453.3025886__;!!DZ3fjg!rsAh7A_d2lxYWpIvjcVJkRBRd4hNU1CQOL4m_QQbhGUcUvsjpbkU3BWg4xFCve9PGQ$
	
	
	(https://urldefense.com/v3/__https://www.theverge.com/2021/3/20/22334527/nft-scams-artists-opensea-rarible-__;!!DZ3fjg!rsAh7A_d2lxYWpIvjcVJkRBRd4hNU1CQOL4m_QQbhGUcUvsjpbkU3BWg4xGZrMOqeA$
	marble-cards-fraud-art) as well as the ecological impacts of blockchain (Jiang,
	S., Li, Y., Lu, Q. et al. Policy assessments for the carbon emission flows and
	sustainability of Bitcoin blockchain operation in China. Nat Commun 12, 1938
	(2021). https://urldefense.com/v3/__https://doi.org/10.1038/s41467-021-22256-3__;!!DZ3fjg!rsAh7A_d2lxYWpIvjcVJkRBRd4hNU1CQOL4m_QQbhGUcUvsjpbkU3BWg4xEvljayzg$ ). The lack of address for these



==> section/Placeholder.tex <==
\subsubsection{Criteria for High-quality NFT (RQ2)} \tanusree{remove and add some content in challenges sections}
% \textbf{Consideration of NFT as Aesthetic VS Utility} 
A large number of new NFTs are created like bamboo shoots after the rain. People in the NFT community are overwhelmed with the ``NFT overload.'' Our participants share various criteria they used to identify good NFTs,  such as, aesthetics, creators' reputation, effort behind the NFT, vision and/or meaning behind the NFT \yang{currently no examples of this below}, and practical utility.
% \review{Aesthetic (should look nice), Reputation of creators?, visions/meanings behind the NFT (specific context behind creation), Utility (i.e. postcard for occasions, badges for social media interaction, tickets for attending conference)}
% \vspace{3pt}
%\tanusree{how about doing an analysis of their actual NFT content. They shared their NFT profile during interview. By doing so, we can address Professor Yun's comment "what’s the ethnicity background of the participants? what’s the ethnicity or political flavors of the created content?". We can have different empression and background directly from art they create. Similar to real world "Abstract Expressionism"} 

\noindent \textbf{Aesthetic.} When the participants showed the authors their collections of NFTs, either created or collected by them, nearly all of them expressed how beautiful the NFTs were. Beauty was seen as a simple and direct standard of a good NFT for P1: \yang{quote not too useful. look nice sounds too abstract. did the participant mention what the NFT s/he was referring to? might need another quote} 
\begin{quote}
    \textit{``It just looks nice. Sometimes, even if the art does not have any meaning, you personally just think it looks nice and present a good taste of NFT.''}
\end{quote} 
% By saying that, this participant further discussed how it is important it is to have creativity element in NFT. However, he added that aesthetic value of NFT has the capacity of eliciting pleasure with positive taste.

\noindent \textbf{Reputation of Creators.} When assessing the value/quality of a certain NFT, people may fall back to simple heuristics, since NFT is a relatively new field, and there is a lack of established assessment measures. For example, P3 estimated the future value of a certain NFT based on its creator's reputation and popularity. He believed NFT created by established artists would be worth more in the future:
\begin{quote}
    \textit{``It was a piece of music that I bought, and it was created by a well known musician group. My thinking is that, they're already an established group. They have a large following in social media. So there's a demand for this item. I see he's very engaged in this space.''}
\end{quote}
% This participants was both a creator and collector. In case of buying NFTs, he considered the reputation of an artists to speculate the price in future. He also added that the legitimacy of an art depends on the reputation of the artist while there are many copycat exist in the marketplace.
\update{According to this participant, NFT created by reputable artists could better serve speculation purposes, due to popularity of the artists, and people's high demand for their work. In many cases, including this participant, social media (especially Twitter) followers are one of the main indications for our participants to assess the reputation of an artist.} 

People would buy NFT created by well-known artists they perceived as talented, even without giving much thought to the real quality of the NFT. P5 mentioned a reputed figure in the NFT marketplace, who was known as Beeple and sold NFT in record-breaking amount of $63$ million dollars. \update{According to this participant, Beeple was talented and successful in delivering trending content in 3D art, and people would buy his work no matter how good it is. In addition to it, he has already a numbers of followers in twitter which is a way to discover his artwork and even gain more popularity}: 
\begin{quote}
    \textit{``His name is spelled BEEPLE. He's the biggest artist in 3D art. It's 3D animation, the most popular form of content. And people see value in it. [...] So I think people tend to like/buy things [...] created by someone talented, regardless of whether it's good or not.''}
\end{quote}

\update{Another participant, P4, who is a tattoo artist, shared her experienced how her NFTs got popularity within a very short period of time. She never had a real life art presentation in gallery. Within three months of joining NFT marketplace, she started to connect with the community and got 3k followers in her twitter account. Before that, she even never had a twitter. As the followers increase, her art piece in NFT got more popularity. \yang{do we have more info about how she got popular or how she got 3k followers? the current quote is still pretty abstract. in general, more specific quotes are better}
\begin{quote}
    \textit{``I'm not an artist itself with, I didn’t draw a picture to sell it in the Gallery in real life. I entered this space three months ago and no one ever know me or saw me. I didn't have a Twitter profile before that. Now I have 3k followers. If you're open to be a part of the community and grow with the others, and you get a lot of followers in twitter and your NFTs get noticed.''}
\end{quote}
}


\noindent \textbf{Efforts behind NFT.} The amount of time and effort devoted to making an NFT was yet another simple heuristic in addition to reputation of creators: the more effort, the more value. P5 used the example of 3D animation, a time-consuming form of NFT art, to illustrate his opinions: 
\begin{quote}
    \textit{``3D animation basically is kind of the most popular form of content. People see value in it, probably because it takes a lot of time and effort to model things. So I think people tend to [buy/like it] when they see something that has taken a lot of time.''}
\end{quote}
% According to this participant, good NFT should represent the effort f

% In this similar context, P1 preferred a NFT to present a certain meaning that creator want to convey and creativeity as two main criteria of good NFT. \textit{``So I'd say the main criteria when I look at NFT arts [...] whether it's a good piece of art is originality, creativity and peacefulness. Sometimes a piece of art can be extremely abstract. But if it's done in a tasteful way and have meaning even though it doesn't contain that much imagery.''}. 

% This participant's preference of good NFT has a similarity with the conventional abstract painting which is a opposition to Renaissance model and figurative art \cite{leder2006entitling}. It contains the valuation of shapes, colors and textures which is subjective to and tangled with artists' emotion that prob audience to understand the meaning behind the work. 

% \noindent \textbf{Practical Utility or Not?}
% \yang{Having actual utility (e.g., NFT as tickets) was considered another criterion, find anther quote}. 

\noindent \textbf{Practical Utility} \yang{separate utility and meaning/vision.} Having actual utility (e.g., NFT as tickets, postcard) was considered another criterion for a good quality NFT among our participants. 

A heated debate about whether NFT should have utility or practical value behind it was noticed by P12. He personally liked the idea of having utility behind NFT, which gave NFT more possibilities:
\begin{quote}
    \textit{``Does NFT need to have utility behind it? Or can it just be digital art? Some people say an NFT is worth more if it has utility behind it. I know there's NFT like, if you buy it, you're able to get into a conference with it. There's a lot of debate happening there, but I personally like the idea of having utility behind NFT, cause there's a lot of exploration you can do there that hasn't been done yet.''}
\end{quote}

Many participants indicated how they used NFT as a self identity in the digital space. P7 thought NFT could be used as personal identities when making friends online, especially in the Metaverse \footnote{https://studio.gometa.io/landing}, which was a virtual shared space:
\begin{quote}
    \textit{''I believe in the future, people will spend more time on the Internet, in the virtual world, in the Metaverse. And in that world, people don't meet each other physically. People use their digital identities to make friends with each other.''}
\end{quote}



% Similarly, Bored Apes, which werev popular NFT avatars, were used as personal identities by members of some Clubhouse rooms. P7 told us that members of a Chinese-speaking NFT-related Clubhouse room used Bored Apes as their Avatars, which was seen by them as a sign of membership. This participant also mentioned an NFT-themed ``attack,'' in which they randomly entered other non-NFT rooms, and shouted like apes. The main motivation behind this ``attack'' was to ``let the non-NFT people know about NFT.'' P11 thought one day, a Bored Ape may be used as the digital identity to attend parties held by the community. 

% Similarly, P3 indicated the about this growing community with diverse people. He added that how he made friends within this short period and gained a large network. He felt that this community provided him the ability to reach out many people.
























\subsection{Design Implications}
\review{There is some more analysis and reflection presented in the discussion, which with more refinement could be neatly interwoven in the findings section. On the whole however, many of the discussion points are familiar to prior work in use of crypto apps (see papers below!), and furthermore lack any deeper criticality, especially around more problematic issues of NFTs (e.g. energy use, fraud, shilling, lack of clear ownership rights etc.) Similarly, the design implications presented are very broad, and repeat familiar challenges  of existing crypto applications e.g. around usability, trust, cost, fraud, regulation etc. which are already well known. I think this shortcoming ultimately stems back to the broad and exploratory nature of the study, and lack of engagement with prior work.}

\yun{basically, the reviewers want to see some languages that clearly state "our findings about XXX is not discussed in prior literature or our findings about XXX is discussed previously, but we expanded the understanding with a new factor that contributed to the xxx.}
\label{design}
% \tanusree{* 2-4 main design implication}
% \tanusree{some raw ideas. need to articulate into design suggestion}
% - design implications
%     -- high gas fee, dedicated blockchain just for NFT (Flow, WAX), ETH (side chains, L2)
%     -- help creators promote their NFT (recommender system, )
%     -- help users discover high-quality NFT (reviews, also helpful for detecting scams)
%     -- support creation of new/diverse types of NFT (e.g., meebit, programmable)
%     -- support easy creation for those who are not technical or who are not artists (e.g., educational materials, usable templates so no need for programming, future work)

\subsubsection{Lower Gas Fee for NFT Creation and Transactions}
The Ethereum blockchain, on which many NFT projects are built, introduces several challenges to the NFT world. The high gas fee on Ethereum was repeatedly mentioned and complained by our participants, which set a high barrier for new artists who could not afford to mint NFT. Even for mature artists, their monetary return could be compromised to a large extent. For example, a participant indicated that the gas fee accounted for 61\% of his total NFT sell.  

Generally, the high gas fee on Ethereum makes NFT creation and trading exclusionary for artists. To make the NFT space more inclusive, one may build NFT platforms on Layer-2 blockchains \cite{layer2} such as OMG Network\footnote{\url{https://omg.network/}}, and/or dedicated blockchains for NFT such as Flow \footnote{\url{https://www.onflow.org/}} and WAX \footnote{\url{https://on.wax.io/wax-io/}}, where cheaper transactions are supported. 
\begin{comment}
\subsubsection{Fairer Recommender Systems to Support Inexperienced Creators and Users}
% There exists a power dimension and popularity based promotion in the NFT marketplace and NFT associated external online groups. 
%We find unfairness when it comes to the visibility of NFT created by artists of different popularity.
Popular artists who already have a strong fan base on social media platforms can sell more NFT at higher prices within a short period of time. NFT trading platforms also promote their work more often, probably for higher monetary return. In comparison, it is much more difficult for artists and creators who just start their career to promote their NFT. Our participants explicitly expressed this as a demotivating factor. %For example, music producer Grimes sold his NFT for almost \$6M in 20 minutes \footnote{https://www.theguardian.com/music/2021/mar/02/grimes-sells-digital-art-collection-non-fungible-tokens}, while one of our participants who was a photographer failed to sell any NFT out in the past month.

To better support less-known or inexperienced NFT creators, we advocate for fairer recommender systems that promote NFT based on more factors such as content genre and user reviews, instead of just the fame of the creators. A desirable property of such a recommender systems is diversity of recommendations, so that creators with different levels of experience and fame could be seen by others.


compared to E-commerce websites such as Amazon,
% , facebook online marketplace, 
which recommended NFT to users who might have interest in it. 
% items based on like, comments, stars provided by NFT community members.

According to our participants, NFT created by less-known artists was less likely to be promoted  and seen. 
% This will provide a space for comparatively fair chance for artist to sell their NFT goods. 
% A community based item-to-item collaborative recommendation system provide more decentralization in NFT trading platforms. 
Thus we advocate for more decentralization in recommendation algorithms. Instead of only or mostly recommending famous artists' NFT to users, less-known artists with fewer followers should also enjoy some visibility. 
\end{comment}

\subsubsection{Detecting Low-Quality NFT and Warning about Scams}

% Many of NFT's pros and cons are related to the blockchain underlying it. For example, irreversibility of blockchain appears to be a blessing among the NFT community, which could be utilized to verify digital ownership of arts. Participants also favor provable scarcity of NFT, which is achieved by hard-coding the number of copies of a certain art in smart contracts. In many cases, there is only one copy of a certain NFT art, which makes it extremely scarce and valuable. Moreover, participants like the automatic way of transactions on the blockchain ledger, which is regarded by them as a more convenient business model, and they do not need to worry about tracking receipts. 

Lack of regulation of the decentralized blockchain introduces several challenges for NFT, such as the prevalence of low-quality NFT and scams. Low-quality NFT created and spammed by those who merely pursue monetary return not only degrades general quality of the NFT marketplace, but also demotivates artists who have put a lot of effort into their work. From our study, it seems that high gas fee plays the role of a regulator, because not everybody can afford to mint. However, this is not a sustainable way of regulation, and puts a heavy burden on passionate artists in a poor financial standing. Loose, limited regulation can be found on NFT trading platforms such as Rarible, e.g., artists can opt to go through a Twitter verification process, and those who do so can enjoy more visibility for their posted NFT. However, low-quality NFT and scams are still prevalent despite all the regulatory efforts. 

To effectively and scalably solve this issue, AI algorithms can be designed and deployed by the platforms to detect scams and low-quality NFT. A key challenge facing such a system is how it can surface and promote legitimate NFT created by inexperienced creators, which may not look that fancy or high-quality. 

On-chain NFT trading data, social media data, and user reviews for NFT items can also play a role in making users aware of scams and quality issues. We can further make the warning interactive by putting negative reviews on top of suspicious NFT, which users could click on and see more related reviews regarding creativity, scarcity, and estimated effort. To encourage production of honest user reviews, rewards (e.g., earning governance tokens) and penalties (e.g., slushing \zhixuan{what does it mean?} or taking away collateralized tokens as seen in proof-of-stake consensus mechanisms) could be practiced.

% The user reviews could be multi-dimensional including factors such as . %To screen out low-quality NFTs, proxy measures such as rough estimate of the time spent on creating the NFT underlying asset can complement user reviews. 
% 

\subsubsection{Supporting Easy Creation and Purchasing for Non-Technical Users} 
The NFT space includes a diverse set of users who may have limited technology background. Our study indicated that participants especially newbies were often intimidated by the conversation around crypto and NFT, which included too many tech-heavy concepts and vocabulary. NFT collectors and creators also felt it cumbersome and time-consuming to buy and mint NFT. 

Despite the rapid development of blockchain, which leads to many cutting-edge applications \cite{wang2021non}, the usability aspect of blockchain is paid less attention to. Thus we call for more research in blockchain and NFT usability, which aims to improve user experience and accessibility of the relatively new technology, and allow more people to participate in the ongoing financial/art revolution. Specifically, educational materials, usable templates for creating NFT are example ways to make it easier for people who are not technical to create and buy NFT. 
% However, we need further research to understand the usability aspect of NFT platform.

\subsubsection{Maintaining Engagement by Ensuring Quality}
Several participants mentioned that members of the NFT community were more passionate about their participation when they were newcomers, and the passion dropped later. Also, trending topics in Discord channels and Clubhouse rooms are constantly changing. When an NFT project or piece is newly released, members would heatedly discuss it, but only for a few days. Out of thousands of NFT projects, only several of them survive and still enjoy popularity till now, such as NBA Top Shots, and Decentraland. 

Thus project owners and NFT creators might need to make an effort to improve the quality of their projects/works, so as to survive people's long-term fatigue and decreased interest. NFT trading platforms can take an active role in improving the quality of NFT, either hiring moderators to manually filter low-quality NFT out, or leverage off-the-shelf AI models to do this.

% \begin{quote}
% `` \it{In today's society of instant gratification and consumption, having to transfer monies into crypto-currency then log into different online wallets and accounts for different fees and processes is too expensive and complicated for many.''} 
% \end{quote}

\subsubsection{Regulation vs. Openness}
A tension between providing a lower barrier and ensuring NFT quality exists in the NFT marketplace. The open nature of NFT and general blockchain removes gatekeepers in the traditional art market, and provides a low barrier to entry for NFT creators to participate. However, the low entry barrier also leads to low-quality NFT and even scams, since everyone is able to mint and trade NFT in the market. 

NFT trading platforms practice different types of restrictions to prevent unexpected scams or low-quality art. For example, Foundation uses an ``invite-only" mechanism for the entry of artists: only invited artists can mint NFT on the platform. Such efforts are intrinsically two-edged swords. Despite their effectiveness in improving NFT quality, they also prevent talented yet poor artists from creating their own art, and become hurdles to creating an open-access domain for everyone, which goes against the initial vision of blockchain. Considerably more research needs to be conducted to find alternative ways of regulation, which ensures quality and decentralization at the same time.

% Individuals might re-prioritise motivating factors at different times based on how well they are satisfied. 
% In this section, we will reflect on reciprocity and mutual support in the NFT community. 
% in the current NFT landscape, and propose corresponding design implications for a more supportive and sustainable NFT community. 

% In this section, we map our results of NFT community dynamics to physical art auction and exhibition environment \cite{o2012impact}, \cite{rizzo2007fire}, \cite{vosinakis2011virtual} to highlight what are the similarities and differences between the two space. We choose these prior work of art exhibition phenomena because 1) this scenario is closely similar with NFT community,  2) there isn’t previous work of NFT to compare this platform’s characteristic and limitation. The goal of this study instead of generating an exhaustive list of similarities to first attempt to answer the question related to current  practices and community interaction of NFT and how existing social/community interaction as well as regulation present in physical art auction world can be adopted in NFT community to improve interaction among NFT users to create a sustainable marketplace. In addition, we present what are the  technological/ social design implication of NFT marketplace that causing users’ to be engaged and motivated. We also report that NFT’s features- augmented with technologies, could contribute to disseminating people's lifestyle values in public and can improve social interaction to build a empathetic and supportive community.








































\tanusree{here are some discussion point we can elaborate in this section}

\textbf{Opportunities for NFT creators}
\begin{itemize}
    \item \textbf{Having Unique ownership and self regulated business model}: thrive to be more creative, keep track of the items and have royalty (not sharing it with any gatekeeper anymore). Will discuss how this differentiate NFT market from other similar online/physical marketplace. will connect with some literature.
    
    \item \textbf{New Assessment Mechanisms Enabled by NFTs \yun{this section can be put separately as a big design implication section. }}: a) will disucss this community as an opportunity to meet other NFT creators, create long term relationship by collaborating and helping each other during the process of creating and promoting work. b) will also discuss the assessment heuristic of fellow NFT creators if they are authentic and share same interest. As a community, participants mentioned that they are able to detect shady people (NFT creators) who try to trick the system to earn money within short period of time and not being authentic and don't have long term vision to stay in this market. Finally, will discuss, the view of the community and NFT creators to have an opportunity to engage people of similar vision with long term goal in this market.
    
    \item \textbf{Incentive Mechanisms: Being a part of this new internet/art revolution}: will discuss the vision of NFT creators about the near and long-term future of NFT art and blockchain technology revolutions. 
    
    \item \textbf{Constantly Learning to use new tools to improve artwork}: a) will discuss about the tools used by different creators and how they evolved since their tooling usage since they joined this marketplace. b) Will discuss some difficulty of using existing tools and limitations. As the implication, this will help new artist to learn about tools to create and promote NFTs since the early stage is the most challenging time when one can feel demotivated due to lack of strategies to promote, sell and create NFTs. This will also help the design implication for future tool design for NFT upcoming designers.
    
\end{itemize}


\textbf{Challenges for NFT creators and as a community}
\begin{itemize}
    \item \textbf{Metrics to discover/assess good artists and artworks}: will discuss about the poor quality of NFT and many malicious NFT creators copying others' work and creating NFT. Will discuss different ways our participants normally discover good artist or artwork. One main thing mentioned frequently is reputation. so, How do they assess reputation? (according to our participants, its twitter followers). Will discuss it briefly and will call for future research opportunity to explore more.
    
    \item \textbf{Trust issues in fellow NFT creators/ community when anonymity is a built in feature}: a) Will discuss the good things of community collaboration, supporting each in promoting, creating and solving bugs in different scenario. b) will also discuss some experience that participants had with fellow NFT creators who acted suspicious behind avator. Its not always comfortable to help fellow NFT creators with resources when they always hide behind the avator and their interaction in the community group is not satisfactory. 
    
    
    \item \textbf{ tech/blockchain/regulation related challenges} \yun{Instead of regulation, you could mention something like "Blur Moderation of NFTs." Basically, content moderation needs human-AI collaboration, there has been works defining the stages of training human moderators, e.g., Seering 2019 paper on moderator engagement, and  there are many moderation rules (e.g.,  Casey's paper on Reddit Rules!), but I wonder if it is clear for NFT communities? you may look at the blocks for general online communities' moderation, then point out that new building blocks may need to be added.}This point is more intuitive. I will discuss a summary of other terminology, concepts related challenges for creators; platform regulation. 
\end{itemize}



--- minting, bidding, canceling, sales and transfer of ownership
Interesting point to explain under different social THEORY:
revolution:
\begin{quote}
    \textit{``It's the new art revolution... I'm better in online marketing than in the real world. I guess it's a cool new thing because you know, I have pretty much followers on Instagram and Facebook. On Instagram I have around 180,000, and on Facebook I have 110,000. So I know I'm better in online stuff, and it's excited to be part of this revolution.''}
\end{quote} 

P3 noticed:
\begin{quote}
    \textit{``I think almost everyone that I've interacted with believes this [NFT] to be one of the most important technologies and advancements in our lifetime. I think a lot of people are calling it the new Renaissance for artists[...]. A lot of new inspiration and new art is coming out, and people are very willing to collaborate in network, across countries, across the world. So I think the overall perception I've received is, people are very excited and very optimistic, and they want to do more and more with this space and develop it.''}
\end{quote} 


-------Many participants indicated how they used NFT as a self identity in digital space. P7 thought NFT could be used as personal identities when making friends online, especially in the Metaverse \footnote{https://studio.gometa.io/landing}, which was a virtual shared space:
\textit{''I believe in the future, people will spend more time on the Internet, in the virtual world, in the Metaverse. And in that world, people don't meet each other physically. People use their digital identities to make friends with each other.''} 

He added that how he made friends within this short period and gained a large network. He felt that this community provided him the ability to reach out many people.


------Some mentioned the supportive community as a motivation of being in the NFT space. For example, P4's motivation for staying in the NFT marketplace after the pandemic had much to do with community ties, such as mutual support and understanding among the artist community:


-----\begin{quote}
    \textit{``His name is spelled BEEPLE. He's the biggest artist in 3D art. It's 3D animation, the most popular form of content. And people see value in it. [...] So I think people tend to like things [...] created by someone talented, regardless of whether it's good or not. They tend to buy it more.''}
\end{quote}


\subsubsection{Differences of NFT from Other Cryptos (RQ1)}
Given NFT is a recent phenomenon, participants viewed NFT as different concept. Some of these includes, unique trait of artist, a way of verifying ownership of items and representing digital identity, scope for self created business model for empowerment. 

% \noindent \textbf{NFT is Unique.} 
% NFT tokens are non-fungible, which means each NFT has some special traits, while fungible tokens (e.g., Bitcoin) are all the same. The primary difference between cryptocurrency and NFTs that NFT cannot be traded for each other as they are unique representations of assets. Four participants (P1, P5, P7, P8) mentioned NFTs are one-of-a-kind digital assets that represent real-world items and are not interchangeable in contrast to fungible tokens.P1 pointed out that every Bitcoin was the same, while NFTs were created by different creators: 
% \textit{``Every single Bitcoin is exactly the same. The only thing that's different is the code. When it comes to NFT, first, it has different creators and someone made it by intention. It has customization built-into words, and it has digital files attached to it to give it value.''}. This participants put off \textit{different intention} as a basis of the uniqueness of NFT. 

% P7 viewed fungible tokens as a way for speculation, and NFT as art with special traits, for which people may have emotions associated to it \textit{``Fungible tokens are more for speculation, and people trade them like stocks. But non-fungible tokens, most of them are kind of art. [...]This token has some special traits, very different from each other. If you own one of them, you have some personal emotion for it. Maybe you use it as an Avatar and sometimes, you don't want to resell it.''}. As we noticed in most of the participants having some types of emotion related to the NFT they creates. P11 explained his NFT creation for his child who was ready to be born in December and he viewed the NFT as a way to keep memories for his son. P4 explained her stress during pandemic and how she overcome by creating NFT duckies. She explained - \textit{``I have a stressful job during COVID. I needed the thing which is able to create in different ways and the duckies are always in our world everywhere, all over the world.''} It has been very common among participants that they don't appreciate NFT which were simple copies of successful ones-doesn't present special traits and creativity: P1 said-\textit{``There're thousands of copy cats that are trying to replicate what CryptoKitties have accomplished. And the unfortunate thing is, it's actually working, people are buying the copy cats. When it comes to art, you have to be creative. ''}


%\end{quote} 
%P2 complemented another difference. According to him, Bitcoin had a fixed supply, but there was not a supply limit for NFT: 
%\begin{quote}
 %   \textit{``I'm familiar with Bitcoin, and have basic knowledge of smaller tokens. Bitcoin is like digital gold. The supply remains the same. Ethereum (where NFTs are created) does not seem to have a supply limit. Unlimited number of NFTs can be created.''}
%\end{quote}
%\textbf{Characteristics of NFT.}
%Typical features of NFT include uniqueness, provable scarcity, inter-operability, and indivisibility. The participants were able to identify some of the features.
%\textit{Irreversibility} of NFT ownership was mentioned by some participants. For instance,  P2 said, 
%\begin{quote}
%    \textit{``It's stored on the blockchain, which is secure. You can't copy or remove it. You can only add, no taking away.''} 
%\end{quote}
%Irreversibility of NFT was supported by the underlying blockchain, which prevented third parties from maliciously tampering ownership of digital collectibles. P11 also mentioned the irreversible and transparent feature of NFT, which made it hard to copy original, valuable items, such as a postcard from a famous person. 
% NFT is also free of physical damage, according to him:
% \begin{quote}
%     \textit{``If I receive a physical postcard, I have to make an effort to protect it from water or fire. There's some risk in storage.''}
% \end{quote}




% \noindent \textbf{NFT Means Ownership.}
% In conventional art markets, the process of verifying copyright for intangible goods was cumbersome. Often times, there was not a way to validate the provenance \cite{van2002art}. P1 illustrated a scenario where it was difficult to verify the authenticity and ownership of art:
% \textit{Before NFT was a thing, I would post the painting on Instagram, and then offer it for sale. 99.9\% of people would just say, why should I buy it? I can just copy the image and download it to myself. There's no real way to prove that you created it or that you've bought it.} On the contrary, NFT is a cryptographic ownership of a unique item which is encoded into the underlying blockchain \cite{wang2021non}. Each NFT can be traced back to its owner. P1, P3 and P14 mentioned about the ownership aspect of NFT. For instance, P1 considered NFT as a way to verify ownership of digital files \textit{`` NFT is buying the coin of someone, and that coin has its value because a digital file is attached to it, whether that be a video, a song, a painting, or just a picture. It's very much just a way to verify ownership of digital files, which previously was very difficult to do.''}. This participant also advocated the advantage of blockcahin and its' irreversibility in which prevented third parties from maliciously tampering ownership of digital collectibles hard to copy original, valuable items, such as a postcard from a famous person. Even after reselling a NFT several times, ownership can be traced back within transaction recorded on the blockchain. At the same time, their full history is publicly available. Anyone can see it and confirm an NFT’s authenticity   



\noindent \textbf{NFT Empowers Users.} 
As a business person owning an NFT company, P3 highlighted convenience of the business model of NFT. He thought NFT allowed freelancers to automate their workflow, with all transactions recorded by the blockchain and easily exportable, which made people's work more convenient and efficient: \textit{`` It empowers individuals to create their own business model. Your business transactions would all be recorded. I think it's something that will benefit freelancers, and allow people to automate their workflow more easily. You don't have to worry about tracking receipts and things like that anymore, because it's all stored on the blockchain.''}. Similarly, many participants indicated the decentralization in ethereum blockchain as a self-governance mechanism where individuals don' require to trust or grant custodianship to a third party who can impose their own rules. In the traditional art market, artists often relied on event organizer and sponsors to exhibit their work \cite{spence2020bob}. The decentralization feature of NFT given by the underlying blockchain freed the NFT marketplace from those gatekeepers. Such an autonomous platform empowered artists, who could exhibit, sell and promote their work freely now, according to P13: \textit{``One of the benefits (of the NFT marketplace) is there are no gatekeepers like in the traditional art market. In the NFT world, you're a self promoter. You just need to come on the platform and do your promotion and sell it without the gatekeepers. This one of the biggest benefits.''} Similarly, P9 indicated the notion of low barriers in NFT for artists to present their digital work, with the help of painting tools and software. Even unknown artists could grow their career in the NFT marketplace. P11 liked to collect NFT created by unknown artists, and would recommend his friends who were artists to create NFT: \textit{``Some artists are unknown, and it's hard for them to make money. But their art may sell well if a market is built to support their career. I know some artists in Taiwan who are of some renown but not that famous. They make extra money by creating NFT of their artwork. So if I have friends who are painters, I would recommend them to create NFT on the platforms.''} NFT marketplace gives an opportunity to numerous digital artists to pounce upon and use their skills to earn living.


\noindent \textbf{NFT is a Place for Collaboration and Connection.} 
Among our participants, we didn't observed as many collaboration in regards to create NFT together. In most cases, NFT creation was reflection of their unique emotion and skill sets. However, there is a drift of willingness to collaborate. P3 expressed the optimism and will to collaborate in the NFT community: \textit{``A lot of new inspiration and new work is coming out and people are very willing to collaborate. In network, across countries, across the world. So I think the overall perception I've received is, people are very excited and very optimistic and they are wanting to do more and more with this space and develop it.''} On a practical level, P6 told us how the artist community collaboratively tried to propose new forms of NFT art:
\textit{``We're really collaborative. And we're always trying to make valuable pieces of art, you know, not trying to make products just for sale. We're always thinking about proposing something new in the art market.''} As the founder of an NFT platform, P10 would attend online meetings organized by other platform founders and developers, and discuss product functions, as well as how to create a better NFT ecosystem for artists.

% \noindent \textbf{NFT Represents Digital Identity}. 

% Many participants indicated how they used NFT as a self identity in digital space. P7 thought NFT could be used as personal identities when making friends online, especially in the Metaverse \footnote{https://studio.gometa.io/landing}, which was a virtual shared space:
% \textit{''I believe in the future, people will spend more time on the Internet, in the virtual world, in the Metaverse. And in that world, people don't meet each other physically. People use their digital identities to make friends with each other.''} Similarly, Bored ape was a popular NFT project recently. P7 told us that members of a Chinese-speaking NFT-related Clubhouse room used bored apes as their Avatars, which showed their membership. This participants also explained an idea discussed in their NFT group of creating a ape NFT themed attack for a non NFT group. The main idea is to let the non NFT people to know about NFT. P11 thought one day, a bored ape may be used as the digital identity to attend parties held by the community. Similarly, P3 indicated the about this growing community with diverse people. He added that how he made friends within this short period and gained a large network. He felt that this community provided him the ability to reach out many people.


==> section/outline.tex <==
Results

- RQ1: perceptions of NFT
 + positive perceptions
    -- people's understanding of NFT
        --- ownership
        --- uniqueness 
        --- empower arts*
        --- collaboration*
        --- digital identity*
    -- Criteria for good NFT
        --- aesthetic considerations
        --- creators' reputation/how much effort* (heuristics that people use; a new field/phenomenon, lack of established assessment measures, so people fall back to simple heuristics)
        --- utility*
 - negative/limitations
    -- Challenges of NFT
        --- technical/bugs
        --- security risks (scams)*
        --- lack of regulations (hard to track/enforce copyright, new trace quote)*
        --- low-quality NFT (long tail, help people discover high-quality NFT/design implication, e.g., reviews/likes, etc)* 
        --- blockchain-related
            ---- irreversibility*
            ---- gas fee
            
- RQ2: motivations
    -- monetary gain
        --- artists create NFT
            ---- making a living during pandemic*
        --- new business model
        --- trading / speculating
    -- express oneself* (identity performance)
    -- community support*
    -- be part of an innovative movement*
    
- RQ3: practices (note: pay attention to their challenges and their mitigation strategies, which become ideas for design implications)
    -- how they discover NFT
    -- how they create/mint NFT (for artists who are not particularly technical)
    -- how they trade/buy/sell NFT (e.g., how they identify scams)
    -- how they use NFT (esp. for NFT that has utilities, as a ticket)
    -- interact with others in the community
        --- NFT promotions (grassroot)
        --- mutual support (between creators)
        
Discussion

- discuss/position main findings in the lit
    -- revisit/summarize RQ1, RQ2, RQ3
    -- highlight the community aspect

- design implications
    -- high gas fee, dedicated blockchain just for NFT (Flow, WAX), ETH (side chains, L2)
    -- help creators promote their NFT (recommender system, )
    -- help users discover high-quality NFT (reviews, also helpful for detecting scams)
    -- support creation of new/diverse types of NFT (e.g., meebit, programmable)
    -- support easy creation for those who are not technical or who are not artists (e.g., educational materials, usable templates so no need for programming, future work)
    
- limitations
    -- sample size (we have diverse participant background, rich data)
    -- we have participants from different countries, but we cannot conclude on country/cultural differences. 
    -- mostly male participants. future research examine if most NFT users are male and why women don't adopt NFT. 
    -- self-reported qualitative data but with some observations. 
    
    
\noindent \textbf{Authenticity and Cryptographic Digital Ownership.}
The basic conceptions and key characteristics of NFT are its authenticity and cryptographic ownership, which allows owners to trace their NFT even after it has been resold several times. In the conventional art market, the process of verifying copyright of intangible commodities is cumbersome. Often times, there is not a way to validate their provenance \cite{van2002art}. On the contrary, NFT collectibles including art/design and game items are valued for their authenticity, rarity and cryptographic ownership. Each minted\footnote{``Minting" refers to the process of tokenizing an item, and uploading it to an NFT platform such as Foundation.} item is encoded into the underlying blockchain \cite{wang2021non}, which can be traced back to its owner. P1 illustrated a scenario before the NFT market bloomed. He explained why it was difficult to verify the authenticity and ownership of art in conventional social networks: \textit{``Before NFT was a thing, I would post the painting on Instagram, and then offer it for sale. 99.9\% of people would just say, why should I buy it? I can just copy the image and download it to myself. There's no real way to prove that you created it or that you've bought it.''}  P1, P3 and P14 mentioned the ownership aspect of NFT. For instance, P1 considered NFT as a way to verify ownership of digital files: \textit{``NFT is buying the coin of someone, and that coin has its value, because a digital file is attached to it which can be a video, song, painting, or picture. It's a way to verify ownership of digital files with the irreversibility nature of blockcahin, which previously was very difficult to do.''} This participant advocated the advantage of blockcahin underlying NFT and its irreversible property, which prevented third parties from maliciously tampering ownership of or copying digital collectibles,  enabled secure storage of the transaction record, and ensured transparency by making the record/ledger publicly available.     

